The model checking fingerprints of CTL operators

The aim of this study is to understand the inherent expressive power of CTL operators. We investigate the complexity of model checking for all CTL fragments with one CTL operator and arbitrary Boolean operators. This gives us a fingerprint of each CTL operator. The comparison between the fingerprints yields a hierarchy of the operators that mirrors their strength with respect to model checking.

==> Bilder-CTL.tex <==
% Declare layers
\pgfdeclarelayer{background}
\pgfsetlayers{background,main}

\definecolor{darkgrey}{gray}{0.6}

\tikzstyle{vertex split}=[circle split,draw=black,minimum size=20pt,inner sep=0pt]
\tikzstyle{selected vertex} = [vertex, fill=black!24]
\tikzstyle{weight} = [font=\small]
\tikzstyle{selected edge} = [draw,line width=2pt,niceArrows]
\tikzstyle{dashed edge} = [draw,densely dashed,line width=1.5pt,niceArrows,black!40]
\tikzstyle{selecteddashed edge} = [draw,densely dashed,line width=1.2pt,niceArrows,black!70]
\tikzstyle{dotted edge} = [draw,densely dotted,line width=1.5pt,niceArrows,black!40]
\tikzstyle{selecteddotted edge} = [draw,densely dotted,line width=1.6pt,niceArrows,black!70]


\tikzstyle{edge} = [draw,thick]
\tikzstyle{revedge} = [draw,thick,<-]
\tikzstyle{mmandgate2} = [and gate,thick,point down,logic gate inputs={nn},info=center:{$\wedge$}] 
\tikzstyle{goodandgate2} = [mmandgate2,fill=black!20]
\tikzstyle{mmandgate3} = [and gate,thick,point down,logic gate inputs={nnn},info=center:{$\wedge$}] 
\tikzstyle{mmorgate2} = [and gate,thick,point down,logic gate inputs={nn},info=center:{$\vee$}] 
\tikzstyle{goodorgate2} = [mmorgate2,fill=black!20] 
\tikzstyle{mmorgate3} = [and gate,thick,point down,logic gate inputs={nnn},info=center:{$\vee$}] 
\tikzstyle{goodorgate3} = [mmorgate3,fill=black!20] 

\tikzstyle{dkante} = [draw,line width=2mm]
\tikzstyle{ckante} = [dkante,black!30]
\tikzstyle{loopcover} = [dkante,in=-10,out=10,min distance=5mm,looseness=8]
\tikzstyle{red vertex} = [vertex, fill=red!24]
\tikzstyle{green vertex} = [vertex, fill=green!44]

\tikzset{
vertex/.style={thick,draw=black,fill=white,ellipse,minimum size=4mm,inner sep=.5mm}
}

%---------------------------------------------------------------------------------------------------


% Ein Schaltkreis-Beispiel
\newcommand{\layeredcircuit}{%
\begin{tikzpicture}[circuit logic US,baseline=(CCC.base)]
\tikzstyle{edge} = [draw,thick,niceArrows]

    \matrix[column sep=7mm,row sep=9mm,ampersand replacement=\&,matrix anchor=south] at (0,0) 
    {
     \node {layer $0$} ; \& \node (l01) {$1$} ; \& \node(l02) {$1$} ;\& \node(l03) {$0$} ; \\ % Knoten l01, l02, l03 in Layer 0
     \node {layer $1$} ; \& \node[mmandgate2] (l11) {} ; \& \node[mmandgate2] (l12) {} ; \& \node[mmandgate2] (l13) {} ; \\
     \node {layer $2$} ; \& \node[mmorgate2] (l21) {} ; \& \node[mmorgate2] (l22) {} ; \& \node[mmorgate2] (l23) {} ; \\
     \node {layer $3$} ; \& \node[mmandgate2] (l31) {} ; \& \node[mmandgate2] (l32) {} ; \& \node[mmandgate3] (l33) {} ; \\
     \node {layer $4$} ; \&  \& \node[mmorgate3] (l41) {} ; \& \\
    } ;


    % die Kanten aus den Eingangsgattern
    \foreach \von/\nach/\in in {l01/l11/2, l02/l11/1, l01/l12/2, l02/l12/1, l03/l13/1, l02/l13/2}
       \draw[edge] (\von) -- (\nach.input \in) ; 
    
    % die Kanten aus den übrigen Gattern des Schaltkreises
    \foreach \von/\nach/\in in {l11/l21/2, l11/l22/2, l12/l21/1, l12/l22/1, l13/l23/1,
                                l21/l32/2, l21/l33/3, l22/l31/2, l22/l33/2, l23/l31/1, l23/l32/1, l23/l33/1,
                                l31/l41/3, l32/l41/2, l33/l41/1}                                
       \draw[edge] (\von.output) -- (\nach.input \in) ; 
     
%    \draw[edge,thick] (l41.output) -- ++(down:3mm) ;    % die Kante aus dem Ausgangsgatter (gehört nicht zum Graph)
    
    \node (CCC) at (1.2,-0.7) {layered monotone circuit $C$} ;
    
    
\end{tikzpicture}
}

% Ein Schaltkreis-Beispiel, das aus \layeredcircuit entsteht,
%  bei dem die Oder-Gatter kopiert werden, so dass jedes Oder-Gatter Ausgangsgrad 1 hat
\newcommand{\layeredcircuitveeone}{%
\begin{tikzpicture}[circuit logic US,baseline=(CCC.base)]
\tikzstyle{edge} = [draw,thick,niceArrows]

    \matrix[column sep=7mm,row sep=9mm,ampersand replacement=\&,matrix anchor=south] at (0,0) 
    {
%     \node {layer $0$} ; \& 
       \node (l01) {} ;  \node[xshift=-2mm] (l011) at (l01) {$1$} ;  \node[xshift=2mm] (l012) at (l01) {$1$} ;  \& 
       \node (l02) {} ;  \node[xshift=-4mm] (l021) at (l02) {$1$} ;  \node (l022) at (l02) {$1$} ; \node[xshift=4mm] (l023) at (l02) {$1$} ; \& 
       \node(l031) {$0$} ; \\ % Knoten in Layer 0
%     \node {layer $1$} ; \& 
       \node[mmandgate2] (l11) {} ; \& \node[mmandgate2] (l12) {} ; \& \node[mmandgate2] (l13) {} ; \\
%     \node {layer $2$} ; \& 
       \node[mmorgate2,yshift=-3mm] (l211) {} ;  \node[mmorgate2,yshift=8mm] (l212) at (l211) {} ; \& 
       \node[mmorgate2,yshift=-3mm] (l221) {} ;  \node[mmorgate2,yshift=8mm] (l222) at (l221) {} ; \& 
       \node[mmorgate2] (l232) {} ; \node[mmorgate2,yshift=-8mm] (l231) at (l232) {} ; \node[mmorgate2,yshift=8mm] (l233) at (l232) {} ; \\
%     \node {layer $3$} ; \& 
       \node[mmandgate2] (l31) {} ; \& \node[mmandgate2] (l32) {} ; \& \node[mmandgate3] (l33) {} ; \\
%     \node {layer $4$} ; \&  
       \& \node[mmorgate3] (l41) {} ; \& \\
    } ;


    % die Kanten aus den Eingangsgattern
    \foreach \von/\nach/\in in {l011/l11/2, l012/l12/2, l021/l11/1, l022/l12/1, l023/l13/2, l031/l13/1}
       \draw[edge] (\von) -- (\nach.input \in) ; 
    
    % die Kanten aus den übrigen Gattern des Schaltkreises
    \foreach \von/\nach/\in in {l11/l211/2, l11/l212/2, l11/l221/2, l11/l222/2, l12/l211/1, l12/l212/1,  l12/l221/1,l12/l222/1, l13/l231/1,l13/l232/1,l13/l233/1,
                                l211/l32/2, l212/l33/3, l221/l31/2, l222/l33/1, l231/l31/1, l232/l32/1, l233/l33/3,
                                l31/l41/3, l32/l41/2, l33/l41/1}                                
       \draw[edge] (\von.output) -- (\nach.input \in) ; 
     
%    \draw[edge,thick] (l41.output) -- ++(down:3mm) ;    % die Kante aus dem Ausgangsgatter (gehört nicht zum Graph)
    
    \node (CCC) at (0,-0.7) {mon. circuit $C$} ;
    
    
\end{tikzpicture}
}

% Ein Schaltkreis-Beispiel, das aus \layeredcircuit entsteht,
%  bei dem die Oder-Gatter kopiert werden, so dass jedes Oder-Gatter Ausgangsgrad 1 hat --
% nun sind auch noch die Oder-Gatter so arrangiert, dass sie "in Reihe" geschaltet werden können
\newcommand{\layeredcircuitveeonere}{%
\begin{tikzpicture}[circuit logic US,baseline=(CCC.base)]
\tikzstyle{edge} = [draw,thick,niceArrows]

    \matrix[column sep=7mm,row sep=8mm,ampersand replacement=\&,matrix anchor=south] at (0,0) 
    {
%     \node {layer $0$} ; \& 
       \node (l01) {} ;  \node[xshift=-4mm] (l011) at (l01) {$1$} ;  \node[xshift=4mm] (l021) at (l01) {$1$} ;  \& 
       \node (l02) {} ;  \node[xshift=-4mm] (l012) at (l02) {$1$} ;  \node[xshift=4mm] (l022) at (l02) {$1$} ;  \& 
       \node (l03) {} ;  \node[xshift=-4mm] (l031) at (l03) {$0$} ;  \node[xshift=4mm] (l023) at (l03) {$1$} ; \\ % Knoten in Layer 0
%     \node {layer $1$} ; \& 
       \node[mmandgate2] (l11) {} ; \& \node[mmandgate2] (l12) {} ; \& \node[mmandgate2] (l13) {} ; \\
%     \node {layer $2$} ; \& 
       \node[mmorgate2,yshift=-3mm] (l221) {} ;  \node[mmorgate2,yshift=8mm] (l231) at (l221) {} ; \& 
       \node[mmorgate2,yshift=-3mm] (l211) {} ;  \node[mmorgate2,yshift=8mm] (l232) at (l211) {} ; \& 
       \node[mmorgate2] (l222) {} ; \node[mmorgate2,yshift=-8mm] (l212) at (l222) {} ; \node[mmorgate2,yshift=8mm] (l233) at (l222) {} ; \\
%     \node {layer $3$} ; \& 
       \node[mmandgate2] (l31) {} ; \& \node[mmandgate2] (l32) {} ; \& \node[mmandgate3] (l33) {} ; \\
%     \node {layer $4$} ; \&  
       \& \node[mmorgate3] (l41) {} ; \& \\
    } ;


    % die Kanten aus den Eingangsgattern
    \foreach \von/\nach/\in in {l011/l11/2, l012/l12/2, l021/l11/1, l022/l12/1, l023/l13/1, l031/l13/2}
       \draw[edge] (\von) -- (\nach.input \in) ; 
    
    % die Kanten aus den übrigen Gattern des Schaltkreises
    \foreach \von/\nach/\in in {l11/l211/2, l11/l212/2, l11/l221/2, l11/l222/2, l12/l211/1, l12/l212/1,  l12/l221/1,l12/l222/1, l13/l231/1,l13/l232/1,l13/l233/1,
                                l211/l32/2, l212/l33/3, l221/l31/2, l222/l33/2, l231/l31/1, l232/l32/1, l233/l33/1,
                                l31/l41/3, l32/l41/2, l33/l41/1}                                
       \draw[edge] (\von.output) -- (\nach.input \in) ; 
     
%    \draw[edge,thick] (l41.output) -- ++(down:3mm) ;    % die Kante aus dem Ausgangsgatter (gehört nicht zum Graph)
    
    \node (CCC) at (0,-0.7) {layered monotone $\lor_1$-circuit $C_1$} ;
    
    
\end{tikzpicture}
}

% Ein Kripke-Modell, das aus \layeredcircuitveeone entsteht,
% wenn die oder-Gatter in Serie geschaltet werden -- Vorversion
\newcommand{\layeredKmodelveeone}{%
\begin{tikzpicture}[circuit logic US,baseline=(l41.base)]
\tikzstyle{edge} = [draw,thick,niceArrows]

    \matrix[column sep=7mm,row sep=9mm,ampersand replacement=\&,matrix anchor=south] at (0,0) 
    {
     \node {layer $0$} ; \& 
       \node (l01) {} ;  \node[vertex,xshift=-5mm] (l011) at (l01) {$1$} ;  \node[vertex,xshift=5mm] (l021) at (l01) {$1$} ;  \& 
       \node (l02) {} ;  \node[vertex,xshift=-5mm] (l012) at (l02) {$1$} ;  \node[vertex,xshift=5mm] (l022) at (l02) {$1$} ;  \& 
       \node (l03) {} ;  \node[vertex,xshift=-5mm] (l023) at (l03) {$1$} ;  \node[vertex,xshift=5mm] (l031) {$0$} ; \\ % Knoten in Layer 0
     \node {layer $1$} ; \& \node[vertex] (l11) {$\wedge$} ; \& \node[vertex] (l12) {$\wedge$} ; \& \node[vertex] (l13) {$\wedge$} ; \\
     \node {layer $2$} ; \& 
       \node (l21) {} ; \node[vertex,xshift=-5mm] (l221) at (l21) {$\vee$} ;  \node[vertex,xshift=5mm] (l231) at (l21) {$\vee$} ; \& 
       \node (l22) {} ; \node[vertex,xshift=-5mm] (l211) at (l22) {$\vee$} ;  \node[vertex,xshift=5mm] (l232) at (l22) {$\vee$} ; \& 
       \node (l23) {} ; \node[vertex] (l222) at (l23) {$\vee$} ; \node[vertex,xshift=-9mm] (l212) at (l23) {$\vee$} ; \node[vertex,xshift=9mm] (l233) at (l23) {$\vee$} ; \\
     \node {layer $3$} ; \& \node[vertex] (l31) {$\wedge$} ; \& \node[vertex] (l32) {$\wedge$} ; \& \node[vertex] (l33) {$\wedge$} ; \\
     \node {layer $4$} ; \&  \& \node[vertex] (l41) {$\vee$} ; \& \\
    } ;

    % die Kanten zwischen den Eingangsgattern
    \foreach \von/\nach in {l011/l021,l012/l022,l023/l031}
       \draw[edge] (\von) -- (\nach) ; 
 
    % die Kanten aus den Eingangsgattern
    \foreach \nach/\von in {l011/l11, l012/l12, l023/l13}
       \draw[edge] (\von) -- (\nach) ; 
    
    % die Kanten zwischen den Gattern in Layer 2
    \foreach \von/\nach in {l221/l231, l211/l232, l212/l222, l222/l233}
       \draw[edge] (\von) -- (\nach) ; 

    % die Kanten aus den übrigen Gattern des Schaltkreises
    \foreach \nach/\von in {l11/l211, l11/l212, l11/l221, l11/l222, l12/l211, l12/l212,  l12/l221, l12/l222, l13/l231, l13/l232, l13/l233,
                                l211/l32, l212/l33, l221/l31, 
                                l31/l41, l32/l41, l33/l41}                                
       \draw[edge] (\von) -- (\nach) ; 
     
\end{tikzpicture}
}

% Eine Instanz von ASAGAP\veeonein
% wenn die oder-Gatter in Serie geschaltet werden -- Vorversion
\newcommand{\ASAGAPveeonein}{%
\begin{tikzpicture}[circuit logic US,baseline=(l41.base)]
\tikzstyle{edge} = [draw,thick,niceArrows]

    \matrix[column sep=0.5mm,row sep=2.5mm,ampersand replacement=\&,matrix anchor=south] at (0,0) 
    {
     \node {slice $V_4\subseteq V_{\exists}$: } ; \& 
       \node (l01) {} ;  \node[vertex,xshift=-3mm] (l011) at (l01) {$T$} ;  \node[vertex,xshift=3mm] (l021) at (l01) {$T$} ;  \& 
       \node (l02) {} ;  \node[vertex,xshift=-3mm] (l012) at (l02) {$T$} ;  \node[vertex,xshift=3mm] (l022) at (l02) {$T$} ;  \& 
       \node (l03) {} ;  \node[vertex,xshift=-3mm] (l023) at (l03) {$T$} ;  \node[vertex,xshift=3mm] (l031) {} ; \\ % Knoten in Layer 0
     \node {slice $V_3\subseteq V_{\forall}$:} ; \& 
       \node[vertex] (l11) { } ; \& \node[vertex] (l12) { } ; \& \node[vertex] (l13) { } ; \\
     \node {slice $V_2\subseteq V_{\exists}$:} ; \& 
       \node (l21) {} ; \node[vertex,xshift=-3mm] (l221) at (l21) { } ;  \node[vertex,xshift=3mm] (l231) at (l21) { } ; \& 
       \node (l22) {} ; \node[vertex,xshift=-3mm] (l211) at (l22) { } ;  \node[vertex,xshift=3mm] (l232) at (l22) { } ; \& 
       \node (l23) {} ; 
       \node[vertex,xshift=-3mm] (l212) at (l23) { } ; \node[vertex,xshift=3mm] (l233) at (l23) { } ; 
     \\
     \node {slice $V_1\subseteq V_{\forall}$:} ; \& \node[vertex] (l31) { } ; \& \node[vertex] (l32) { } ; \& \node[vertex] (l33) { } ; \\
     \node {slice $V_0\subseteq V_{\exists}$:} ; \&  \& \node[vertex,label=below:{$s$}] (l41) { } ; \& \\
    } ;

    % die Kanten von slice 3 nach slice 4
    \foreach \von/\nach in {l11/l011, l11/l021, l12/l012, l12/l022, l13/l023, l13/l031}
       \draw[edge] (\von) -- (\nach) ; 
 
    % die Kanten von slice 1 nach slice 2
    \foreach \von/\nach in {l31/l221, l31/l231, l32/l211, l32/l232, l33/l212, l33/l233}
       \draw[edge] (\von) -- (\nach) ; 

    % die Kanten aus den übrigen Gattern des Schaltkreises
    \foreach \nach/\von in {l11/l211, l11/l212, l11/l221, l12/l211, l12/l212,  l12/l221, l13/l231, l12/l232, l13/l232, l13/l233,
                                l31/l41, l32/l41, l33/l41}                                
       \draw[edge] (\von) -- (\nach) ; 
     
    \begin{pgfonlayer}{background}
      \draw[ckante,draw=gray!30] (l41) -- (l32) ;   
      \draw[ckante,draw=black!50] (l32) -- (l211) ;   
      \draw[ckante,draw=black!50] (l32) -- (l232) ;   
      \draw[ckante,draw=gray!30] (l211) -- (l11) ;   
      \draw[ckante,draw=gray!30] (l232) -- (l12) ;   
      \draw[ckante,draw=black!50] (l11) -- (l011) ;   
      \draw[ckante,draw=black!50] (l11) -- (l021) ;   
      \draw[ckante,draw=black!50] (l12) -- (l012) ;   
      \draw[ckante,draw=black!50] (l12) -- (l022) ;   
    \end{pgfonlayer}
\end{tikzpicture}
}

% Ein Kripke-Modell, das aus \layeredcircuitveeone entsteht,
% wenn die oder-Gatter in Serie geschaltet werden -- endgültig Version
\newcommand{\layeredKmodelveeonefinal}{%
\begin{tikzpicture}[circuit logic US,baseline=(l41.base)]
\tikzstyle{vertex}=[circle,draw=black,thick,minimum size=12pt,inner sep=2pt]
\tikzstyle{edge} = [draw,thick,niceArrows]
\tikzstyle{tinyloopabove} = [draw,thick,in=-15,out=15,min distance=3mm,looseness=8]

    \matrix[column sep=7mm,row sep=9mm,ampersand replacement=\&,matrix anchor=south] at (0,0) 
    {
%     \node {layer $0$} ; \& 
       \node (l01) {} ;  \node[vertex,xshift=-12mm] (l011) at (l01) {$1$} ; \node[vertex,xshift=-4mm] (l011r) at (l01) {} ;  
                         \node[vertex,xshift=4mm] (l021) at (l01) {$1$} ;  \node[vertex,xshift=12mm] (l021r) at (l01) {} ;  \& 
       \node (l02) {} ;  \node[vertex,xshift=-12mm] (l012) at (l02) {$1$} ;  \node[vertex,xshift=-4mm] (l012r) at (l02) {} ;  
                         \node[vertex,xshift=4mm] (l022) at (l02) {$1$} ;  \node[vertex,xshift=12mm] (l022r) at (l02) {} ;  \& 
       \node (l03) {} ;  \node[vertex,xshift=-12mm] (l023) at (l03) {$1$} ;  \node[vertex,xshift=-4mm] (l023r) at (l03) {} ;  
                         \node[vertex,xshift=4mm] (l031) {$0$} ; \node[vertex,xshift=12mm] (l031r) {} ; \\ % Knoten in Layer 0
%     \node {layer $1$} ; \& 
       \node[vertex] (l11) {$\wedge$} ; \& \node[vertex] (l12) {$\wedge$} ; \& \node[vertex] (l13) {$\wedge$} ; \\
%     \node {layer $2$} ; \& 
       \node (l21) {} ; \node[vertex,xshift=-12mm] (l221) at (l21) {$\vee$} ;  \node[vertex,xshift=-4mm] (l221r) at (l21) {} ;  
                        \node[vertex,xshift=4mm] (l231) at (l21) {$\vee$} ; \node[vertex,xshift=12mm] (l231r) at (l21) {} ; \& 
       \node (l22) {} ; \node[vertex,xshift=-12mm] (l211) at (l22) {$\vee$} ;  \node[vertex,xshift=-4mm] (l211r) at (l22) {} ;  
                        \node[vertex,xshift=4mm] (l232) at (l22) {$\vee$} ;  \node[vertex,xshift=12mm] (l232r) at (l22) {} ; \& 
       \node (l23) {} ; \node[vertex,xshift=-4mm] (l222) at (l23) {$\vee$} ; \node[vertex,xshift=4mm] (l222r) at (l23) {} ; 
                        \node[vertex,xshift=-20mm] (l212) at (l23) {$\vee$} ; \node[vertex,xshift=-12mm] (l212r) at (l23) {} ; 
                        \node[vertex,xshift=12mm] (l233) at (l23) {$\vee$} ; \node[vertex,xshift=20mm] (l233r) at (l23) {} ; \\
%     \node {layer $3$} ; \& 
       \node[vertex] (l31) {$\wedge$} ; \& \node[vertex] (l32) {$\wedge$} ; \& \node[vertex] (l33) {$\wedge$} ; \\
%     \node {layer $4$} ; \&  
      \& \node[vertex] (l41) {$\vee$} ; \node[vertex,xshift=8mm] (l41r) at (l41) {} ; \& \\
    } ;

    \foreach \zz in {l021r,l022r,l031r,l231r,l232r,l233r,l41r}
      \draw (\zz) edge[tinyloopabove] (\zz) ;

    % die Kanten zwischen den Eingangsgattern
    \foreach \von/\nach in {l011/l011r, l011r/l021, l021/l021r, l012/l012r/, l012r/l022, l022/l022r, l023/l023r, l023r/l031, l031/l031r}
       \draw[edge] (\von) -- (\nach) ; 
 
    % die Kanten aus den Eingangsgattern
    \foreach \nach/\von in {l011/l11, l012/l12, l023/l13}
       \draw[edge] (\von) -- (\nach) ; 
    
    % die Kanten zwischen den Gattern in Layer 2
    \foreach \von/\nach in {l221/l221r, l221r/l231, l231/l231r, l211/l211r, l211r/l232, l232/l232r,
                            l212/l212r, l212r/l222, l222/l222r, l222r/l233, l233/l233r}
       \draw[edge] (\von) -- (\nach) ; 

    % die Kanten aus den übrigen Gattern des Schaltkreises
    \foreach \nach/\von in {l11/l211, l11/l212, l11/l221, l11/l222, l12/l211, l12/l212,  l12/l221, l12/l222, l13/l231, l13/l232, l13/l233,
                                l211/l32, l212/l33, l221/l31, 
                                l31/l41, l32/l41, l33/l41, l41r/l41}                                
       \draw[edge] (\von) -- (\nach) ; 
     
\end{tikzpicture}
}




% Ein Kripke-Modell, das aus \layeredcircuitveeone entsteht,
% wenn die oder-Gatter in Serie geschaltet werden -- endgültig Version
\newcommand{\transformedGl}{%
\begin{tikzpicture}[circuit logic US,baseline=(l41.base)]
\tikzstyle{vertex}=[ellipse,draw=black,thick,minimum size=12pt,inner sep=0mm]
\tikzstyle{edge} = [draw,thick,niceArrows]
\tikzstyle{tinyloopabove} = [draw,thick,niceArrows,in=-15,out=15,min distance=3mm,looseness=8]

    \matrix[column sep=4.5mm,row sep=4mm,ampersand replacement=\&,matrix anchor=south] at (0,0) 
    {
     \node {slice $V^{\flat}_4$} ; \& 
       \node (l01) {} ;  \node[vertex,xshift=-12mm] (l011) at (l01) {$V_{\exists}$} ; 
       					 \node[vertex,xshift=-4mm] (l011r) at (l01) {$\hat{V}_{\exists}$} ;  
                         \node[vertex,xshift=4mm] (l021) at (l01) {$V_{\exists}$} ;  
                         \node[vertex,xshift=12mm] (l021r) at (l01) {$\hat{V}_{\exists}$} ;  \& 
       \node (l02) {} ;  \node[vertex,xshift=-12mm] (l012) at (l02) {$V_{\exists}$} ;  
       					 \node[vertex,xshift=-4mm] (l012r) at (l02) {$\hat{V}_{\exists}$} ;  
                         \node[vertex,xshift=4mm] (l022) at (l02) {$V_{\exists}$} ;  
                         \node[vertex,xshift=12mm] (l022r) at (l02) {$\hat{V}_{\exists}$} ;  \& 
       \node (l03) {} ;  \node[vertex,xshift=-12mm] (l023) at (l03) {$V_{\exists}$} ;  
       					 \node[vertex,xshift=-4mm] (l023r) at (l03) {$\hat{V}_{\exists}$} ;  
                         \node[vertex,xshift=4mm] (l031) {$V_{\exists}$} ; 
                         \node[vertex,xshift=12mm] (l031r) {$\hat{V}_{\exists}$} ; \\ % Knoten in Layer 0
     \node {slice $V^{\flat}_3$} ; \& 
       \node[vertex] (l11) {$V_{\forall}$} ; 
       \node[vertex,xshift=12mm] (l11r) at (l11) {$\hat{V}_{\forall}$} ; \& 
       \node[vertex] (l12) {$V_{\forall}$} ; 
       \node[vertex,xshift=12mm] (l12r) at (l12) {$\hat{V}_{\forall}$} ; \& 
       \node[vertex] (l13) {$V_{\forall}$} ; 
       \node[vertex,xshift=12mm] (l13r) at (l13) {$\hat{V}_{\forall}$} ;\\
     \node {slice $V^{\flat}_2$} ; \& 
       \node (l21) {} ; 
       		\node[vertex,xshift=-12mm] (l221) at (l21) {$V_{\exists}$} ;  
					\node[vertex,xshift=-4mm] (l221r) at (l21) {$\hat{V}_{\exists}$} ;  
					\node[vertex,xshift=4mm] (l231) at (l21) {$V_{\exists}$} ; 
					\node[vertex,xshift=12mm] (l231r) at (l21) {$\hat{V}_{\exists}$} ; \& 
       \node (l22) {} ; 
       		\node[vertex,xshift=-12mm] (l211) at (l22) {$V_{\exists}$} ;  
					\node[vertex,xshift=-4mm] (l211r) at (l22) {$\hat{V}_{\exists}$} ;  
					\node[vertex,xshift=4mm] (l232) at (l22) {$V_{\exists}$} ;  
					\node[vertex,xshift=12mm] (l232r) at (l22) {$\hat{V}_{\exists}$} ; \& 
       \node (l23) {} ; 
           \node[vertex,xshift=-12mm] (l212) at (l23) {$V_{\exists}$} ; 
           \node[vertex,xshift=-4mm] (l212r) at (l23) {$\hat{V}_{\exists}$} ; 
           \node[vertex,xshift=4mm] (l233) at (l23) {$V_{\exists}$} ; 
           \node[vertex,xshift=12mm] (l233r) at (l23) {$\hat{V}_{\exists}$} ; \\
     \node {slice $V^{\flat}_1$} ; \& 
       \node[vertex] (l31) {$V_{\forall}$} ; 
       \node[vertex,xshift=12mm] (l31r) at (l31) {$\hat{V}_{\forall}$} ;\& 
       \node[vertex] (l32) {$V_{\forall}$} ; 
       \node[vertex,xshift=12mm] (l32r) at (l32) {$\hat{V}_{\forall}$} ;\& 
       \node[vertex] (l33) {$V_{\forall}$} ; 
       \node[vertex,xshift=12mm] (l33r) at (l33) {$\hat{V}_{\forall}$} ;\\
     \node {slice $V^{\flat}_0$} ; \&  
      \& \node[vertex] (l41) {$V_{\exists}$} ; 
         \node[vertex,xshift=8mm] (l41r) at (l41) {$\hat{V}_{\exists}$} ; \& \\
    } ;

    \foreach \zz in {l021r,l022r,l031r,l231r,l232r,l233r,l41r,l11r,l12r,l13r,l31r,l32r,l33r}
      \draw (\zz) edge[tinyloopabove] (\zz) ;

    % die Kanten zwischen den Eingangsgattern
    \foreach \von/\nach in {l011/l011r, l011r/l021, l021/l021r, l012/l012r/, l012r/l022, l022/l022r, l023/l023r, l023r/l031, l031/l031r}
       \draw[edge] (\von) -- (\nach) ; 
 
    % die Kanten aus den Eingangsgattern
    \foreach \nach/\von in {l011/l11, l012/l12, l023/l13}
       \draw[edge] (\von) -- (\nach) ; 
    
    % die Kanten zwischen den Gattern in Layer 3
    \foreach \von/\nach in {l11/l11r, l12/l12r, l13/l13r}
       \draw[edge] (\von) -- (\nach) ; 

    % die Kanten zwischen den Gattern in Layer 2
    \foreach \von/\nach in {l221/l221r, l221r/l231, l231/l231r, l211/l211r, l211r/l232, l232/l232r,
                            l212/l212r, l212r/l233, l233/l233r}
       \draw[edge] (\von) -- (\nach) ; 

    % die Kanten zwischen den Gattern in Layer 1
    \foreach \von/\nach in {l31/l31r, l32/l32r, l33/l33r}
       \draw[edge] (\von) -- (\nach) ; 

    % die Kanten aus den übrigen Gattern des Schaltkreises
    \foreach \nach/\von in {l11/l211, l11/l221, l12/l211, l12/l212, l12/l232, l13/l232, l13/l233,l211/l32, l212/l33, l221/l31, l31/l41, l32/l41, l41r/l41}                                
       \draw[edge] (\von) -- (\nach) ; 

    % gebogene Kanten
    \path[edge] (l221) edge [out=35,in=-155] node {} (l12);
    \path[edge] (l231) edge [out=25,in=200] node {} (l13);
    \path[edge] (l212) edge [out=155,in=-35] node {} (l11); 
    \path[edge] (l41) edge [out=45,in=225] node {} (l33); 

    \begin{pgfonlayer}{background}
      \draw[ckante,draw=gray!30] (l41) -- (l32) -- (l32r) ; 
      \draw[ckante,draw=black!50] (l32) -- (l211) -- (l211r) -- (l232) -- (l232r); 
      \foreach \ee in {l232r,l021r,l022r} 
         \draw (\ee) edge[tinyloopabove,ckante,draw=black!50,-] (\ee) ;
      \foreach \ee in {l32r,l11r,l12r} 
         \draw (\ee) edge[tinyloopabove,ckante,draw=gray!30,-] (\ee) ;
   
      \draw[ckante,draw=gray!30] (l211) -- (l11) -- (l11r) ;   
      \draw[ckante,draw=gray!30] (l232) -- (l12) -- (l12r) ;   
      \draw[ckante,draw=black!50] (l11) -- (l011) -- (l011r) -- (l021) -- (l021r) ;   
      \draw[ckante,draw=black!50] (l12) -- (l012) -- (l012r) -- (l022) -- (l022r) ;   
    \end{pgfonlayer}
\end{tikzpicture}
}


% Ein Kripke-Modell, das aus \layeredcircuitveeone entsteht,
% wenn die oder-Gatter in Serie geschaltet werden -- endgültig Version
\newcommand{\ERveefromGl}{%
\begin{tikzpicture}[circuit logic US,baseline=(l41.base)]
\tikzstyle{edge} = [draw,thick,niceArrows]
\tikzstyle{tinyloopabove} = [draw,niceArrows,thick,in=-15,out=15,min distance=3mm,looseness=8]
\tikzstyle{vertex}=[rectangle,rounded corners,draw=black,thick,minimum size=13pt,minimum height=20pt,inner sep=.5mm,fill=white]

    \matrix[column sep=5mm,row sep=3mm,ampersand replacement=\&,matrix anchor=south] at (0,0) 
    {
     \node {$V_4\cup\hat{V}_4$:} ; \& 
       \node (l01) {} ;  \node[vertex,xshift=-12mm] (l011) at (l01) {\knoteninhalt{$s_4$\\$s_3$\\$t$}} ; \node[vertex,xshift=-4mm] (l011r) at (l01) {\knoteninhalt{$\hat{s}_3$}} ;  
                         \node[vertex,xshift=4mm] (l021) at (l01) {\knoteninhalt{$s_4$\\$s_3$\\$t_3$\\$t$}} ;  \node[vertex,xshift=12mm] (l021r) at (l01) { } ;  \& 
       \node (l02) {} ;  \node[vertex,xshift=-12mm] (l012) at (l02) {\knoteninhalt{$s_4$\\$s_3$\\$t$}} ;  \node[vertex,xshift=-4mm] (l012r) at (l02) {\knoteninhalt{$\hat{s}_3$}} ;  
                         \node[vertex,xshift=4mm] (l022) at (l02) {\knoteninhalt{$s_4$\\$s_3$\\$t_3$\\$t$}} ;  \node[vertex,xshift=12mm] (l022r) at (l02) { } ;  \& 
       \node (l03) {} ;  \node[vertex,xshift=-12mm] (l023) at (l03) {\knoteninhalt{$s_4$\\$s_3$\\$t$}} ;  \node[vertex,xshift=-4mm] (l023r) at (l03) {\knoteninhalt{$\hat{s}_3$}} ;  
                         \node[vertex,xshift=4mm] (l031) {\knoteninhalt{$s_4$\\$s_3$\\$t_3$}} ; \node[vertex,xshift=12mm] (l031r) { } ; \\ % Knoten in Layer 0
                         
     \node {$V_3\cup\hat{V}_3$:} ; \& 
       \node[vertex] (l11) {\knoteninhalt{$s_3$\\$s_2$}} ; \node[vertex,xshift=12mm] (l11r) at (l11) {} ; \& 
       \node[vertex] (l12) {\knoteninhalt{$s_3$\\$s_2$}} ; \node[vertex,xshift=12mm] (l12r) at (l12) {} ; \& 
       \node[vertex] (l13) {\knoteninhalt{$s_3$\\$s_2$}} ; \node[vertex,xshift=12mm] (l13r) at (l13) {} ; \\
     \node {$V_2\cup\hat{V}_2$:} ; \& 
       \node (l21) {} ; \node[vertex,xshift=-12mm] (l221) at (l21) {\knoteninhalt{$s_2$\\$s_1$}} ;  \node[vertex,xshift=-4mm] (l221r) at (l21) {\knoteninhalt{$\hat{s}_1$}} ;  
                        \node[vertex,xshift=4mm] (l231) at (l21) {\knoteninhalt{$s_2$\\$s_1$\\$t_1$}} ; \node[vertex,xshift=12mm] (l231r) at (l21) { } ; \& 
       \node (l22) {} ; \node[vertex,xshift=-12mm] (l211) at (l22) {\knoteninhalt{$s_2$\\$s_1$}} ;  \node[vertex,xshift=-4mm] (l211r) at (l22) {\knoteninhalt{$\hat{s}_1$}} ;  
                        \node[vertex,xshift=4mm] (l232) at (l22) {\knoteninhalt{$s_2$\\$s_1$\\$t_1$}} ;  \node[vertex,xshift=12mm] (l232r) at (l22) { } ; \& 
       \node (l23) {} ; %\node[vertex,xshift=-4mm] (l222) at (l23) {\knoteninhalt{$s_2$\\$s_1$}} ; \node[vertex,xshift=4mm] (l222r) at (l23) {\knoteninhalt{$\hat{s}_1$}} ; 
                        \node[vertex,xshift=-12mm] (l212) at (l23) {\knoteninhalt{$s_2$\\$s_1$}} ; \node[vertex,xshift=-4mm] (l212r) at (l23) {\knoteninhalt{$\hat{s}_1$}} ; 
                        \node[vertex,xshift=4mm] (l233) at (l23) {\knoteninhalt{$s_2$\\$s_1$\\$t_1$}} ; \node[vertex,xshift=12mm] (l233r) at (l23) { } ; \\
     \node {$V_1\cup\hat{V}_1$:} ; \& 
       \node[vertex] (l31) {\knoteninhalt{$s_1$\\$s_0$}} ; \node[vertex,xshift=12mm] (l31r) at (l31) {} ; \& 
       \node[vertex] (l32) {\knoteninhalt{$s_1$\\$s_0$}} ; \node[vertex,xshift=12mm] (l32r) at (l32) {} ; \& 
       \node[vertex] (l33) {\knoteninhalt{$s_1$\\$s_0$}} ; \node[vertex,xshift=12mm] (l33r) at (l33) {} ;\\
     \node {$V_0\cup\hat{V}_0$:} ; \&  
      \& \node[vertex] (l41) {\knoteninhalt{$s_0$}} ; \node[vertex,xshift=8mm] (l41r) at (l41) { } ; \& \\
    } ;

    \foreach \zz in {l021r,l022r,l031r,l231r,l232r,l233r,l41r,l11r,l12r,l13r,l31r,l32r,l33r}
      \draw (\zz) edge[tinyloopabove] (\zz) ;

    % die Kanten zwischen den Eingangsgattern
    \foreach \von/\nach in {l011/l011r, l011r/l021, l021/l021r, l012/l012r/, l012r/l022, l022/l022r, l023/l023r, l023r/l031, l031/l031r}
       \draw[edge] (\von) -- (\nach) ; 
 
    % die Kanten von slice 3 zu slice 4
    \foreach \von/\nach in {l11/l011, l12/l012, l13/l023}
       \draw[edge] (\von.north) -- (\nach.south) ; 

    % die Kanten von slice 3 zu slice 3
    \foreach \von/\nach in {l11/l11r, l12/l12r, l13/l13r}
       \draw[edge] (\von) -- (\nach) ; 
     
    % die Kanten von slice 2 zu slice 3
    \foreach \von/\nach in {l211/l11, l221/l11, 
                            l211/l12, l212/l12, l221/l12, 
                            l231/l13, l232/l12, l232/l13, l233/l13}
       \draw[edge] (\von.north) -- (\nach.south) ; 

    % die Kanten von slice 1 zu slice 2
    \foreach \von/\nach in {l31/l221, l32/l211, l33/l212}
       \draw[edge] (\von.north) -- (\nach.south) ; 

    % die Kanten von slice 1 zu slice 1
    \foreach \von/\nach in {l31/l31r, l32/l32r, l33/l33r}
       \draw[edge] (\von) -- (\nach) ; 
       
    % die Kanten von slice 0 zu slice 1
    \foreach \von/\nach in {l41/l31, l41/l32, l41/l33}
       \draw[edge] (\von.north) -- (\nach.south) ; 

    % die Kanten zwischen den Gattern in Layer 2
    \foreach \von/\nach in {l221/l221r, l221r/l231, l231/l231r, l211/l211r, l211r/l232, l232/l232r,
                            l212/l212r, l212r/l233, l233/l233r}
       \draw[edge] (\von) -- (\nach) ; 

    % die Kanten aus den übrigen Gattern des Schaltkreises
    \foreach \nach/\von in {l41r/l41}                                
       \draw[edge] (\von) -- (\nach) ; 
       
    \begin{pgfonlayer}{background}
      \draw[ckante,draw=gray!30] (l41) -- (l32) -- (l32r) ; 
      \draw[ckante,draw=black!50] (l32.north) -- (l211.south);
           \draw[ckante,draw=black!50] (l211.east) -- (l211r) -- (l232) -- (l232r); 
      \foreach \ee in {l232r,l021r,l022r} 
         \draw (\ee) edge[tinyloopabove,ckante,draw=black!50,-] (\ee) ;
      \foreach \ee in {l32r,l11r,l12r} 
         \draw (\ee) edge[tinyloopabove,ckante,draw=gray!30,-] (\ee) ;
   
      \draw[ckante,draw=gray!30] (l211.north) -- (l11.south);  \draw[ckante,draw=gray!30] (l11.east)-- (l11r) ;   
      \draw[ckante,draw=gray!30] (l232.north) -- (l12.south);  \draw[ckante,draw=gray!30] (l12.east)-- (l12r) ;   
      \draw[ckante,draw=black!50] (l11.north) -- (l011.south);
            \draw[ckante,draw=black!50] (l011.east) -- (l011r) -- (l021) -- (l021r) ;   
      \draw[ckante,draw=black!50] (l12.north) -- (l012.south);
            \draw[ckante,draw=black!50] (l012.east)-- (l012r) -- (l022) -- (l022r) ;   
    \end{pgfonlayer}
     
\end{tikzpicture}
}


% Ein Kripke-Modell, das aus \layeredcircuitveeone entsteht,
% wenn die oder-Gatter in Serie geschaltet werden -- endgültig Version
\newcommand{\EGoplusfromGl}{%
\begin{tikzpicture}[circuit logic US,baseline=(l41.base)]
%\tikzstyle{vertex}=[circle,draw=black,thick,minimum size=12pt,inner sep=0pt]
\tikzstyle{edge} = [draw,thick,niceArrows]
\tikzstyle{tinyloopabove} = [draw,niceArrows,thick,in=-15,out=15,min distance=3mm,looseness=8]
\tikzstyle{vertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=32pt,inner sep=2pt,fill=white]

    \matrix[column sep=4mm,row sep=5mm,ampersand replacement=\&,matrix anchor=south] at (0,0) 
    {
     \node {$V_4\cup\hat{V}_4$:} ; \& 
       \node (l01) {} ;  \node[vertex,xshift=-12mm] (l011) at (l01) {\knoteninhalt{$s_4$\\$t$}} ; \node[vertex,xshift=-4mm] (l011r) at (l01) {\knoteninhalt{$s_4$\\$\hat{s}_4$}} ;  
                         \node[vertex,xshift=4mm] (l021) at (l01) {\knoteninhalt{$s_4$\\$t$}} ;  \node[vertex,xshift=12mm] (l021r) at (l01) {\knoteninhalt{$s_4$\\$\hat{s}_4$}} ;  \& 
       \node (l02) {} ;  \node[vertex,xshift=-12mm] (l012) at (l02) {\knoteninhalt{$s_4$\\$t$}} ;  \node[vertex,xshift=-4mm] (l012r) at (l02) {\knoteninhalt{$s_4$\\$\hat{s}_4$}} ;  
                         \node[vertex,xshift=4mm] (l022) at (l02) {\knoteninhalt{$s_4$\\$t$}} ;  \node[vertex,xshift=12mm] (l022r) at (l02) {\knoteninhalt{$s_4$\\$\hat{s}_4$}} ;  \& 
       \node (l03) {} ;  \node[vertex,xshift=-12mm] (l023) at (l03) {\knoteninhalt{$s_4$\\$t$}} ;  \node[vertex,xshift=-4mm] (l023r) at (l03) {\knoteninhalt{$s_4$\\$\hat{s}_4$}} ;  
                         \node[vertex,xshift=4mm] (l031) {\knoteninhalt{$s_4$}} ; \node[vertex,xshift=12mm] (l031r) {\knoteninhalt{$s_4$\\$\hat{s}_4$}} ; \\ 
                         
     \node {$V_3\cup\hat{V}_3$:} ; \& 
       \node[vertex] (l11) {\knoteninhalt{$s_3$}} ; \node[vertex,xshift=12mm] (l11r) at (l11) {\knoteninhalt{$s_3$\\$\hat{s_3}$}} ; \& 
       \node[vertex] (l12) {\knoteninhalt{$s_3$}} ; \node[vertex,xshift=12mm] (l12r) at (l12) {\knoteninhalt{$s_3$\\$\hat{s_3}$}} ; \& 
       \node[vertex] (l13) {\knoteninhalt{$s_3$}} ; \node[vertex,xshift=12mm] (l13r) at (l13) {\knoteninhalt{$s_3$\\$\hat{s_3}$}} ;\\
     
     \node {$V_2\cup\hat{V}_2$:} ; \& 
       \node (l21) {} ; \node[vertex,xshift=-12mm] (l221) at (l21) {\knoteninhalt{$s_2$}} ;  \node[vertex,xshift=-4mm] (l221r) at (l21) {\knoteninhalt{$s_2$\\$\hat{s}_2$}} ;  
                        \node[vertex,xshift=4mm] (l231) at (l21) {\knoteninhalt{$s_2$}} ; \node[vertex,xshift=12mm] (l231r) at (l21) {\knoteninhalt{$s_2$\\$\hat{s}_2$}} ; \& 
       \node (l22) {} ; \node[vertex,xshift=-12mm] (l211) at (l22) {\knoteninhalt{$s_2$}} ;  \node[vertex,xshift=-4mm] (l211r) at (l22) {\knoteninhalt{$s_2$\\$\hat{s}_2$}} ;  
                        \node[vertex,xshift=4mm] (l232) at (l22) {\knoteninhalt{$s_2$}} ;  \node[vertex,xshift=12mm] (l232r) at (l22) {\knoteninhalt{$s_2$\\$\hat{s}_2$}} ; \& 
       \node (l23) {} ; %\node[vertex,xshift=-4mm] (l222) at (l23) {\knoteninhalt{$s_2$}} ; \node[vertex,xshift=4mm] (l222r) at (l23) {\knoteninhalt{$s_2$\\$\hat{s}_2$}} ; 
                        \node[vertex,xshift=-12mm] (l212) at (l23) {\knoteninhalt{$s_2$}} ; \node[vertex,xshift=-4mm] (l212r) at (l23) {\knoteninhalt{$s_2$\\$\hat{s}_2$}} ; 
                        \node[vertex,xshift=4mm] (l233) at (l23) {\knoteninhalt{$s_2$}} ; \node[vertex,xshift=12mm] (l233r) at (l23) {\knoteninhalt{$s_2$\\$\hat{s}_2$}} ; \\
     \node {$V_1\cup \hat{V}_1$:} ; \& 
       \node[vertex] (l31) {\knoteninhalt{$s_1$}} ; \node[vertex,xshift=12mm] (l31r) at (l31) {\knoteninhalt{$s_1$\\$\hat{s_1}$}} ; \& 
       \node[vertex] (l32) {\knoteninhalt{$s_1$}} ; \node[vertex,xshift=12mm] (l32r) at (l32) {\knoteninhalt{$s_1$\\$\hat{s_1}$}} ; \& 
       \node[vertex] (l33) {\knoteninhalt{$s_1$}} ; \node[vertex,xshift=12mm] (l33r) at (l33) {\knoteninhalt{$s_1$\\$\hat{s_1}$}} ; \\
       
     \node {$V_0\cup\hat{V}_0$:} ; \&  
      \& \node[vertex] (l41) {\knoteninhalt{$s_0$}} ; \node[vertex,xshift=8mm] (l41r) at (l41) {\knoteninhalt{$s_0$\\$\hat{s}_0$}} ; \& \\
    } ;

    \foreach \zz in {l021r,l022r,l031r,l231r,l232r,l233r,l41r,l11r,l12r,l13r,l31r,l32r,l33r}
      \draw (\zz) edge[tinyloopabove] (\zz) ;

    % die Kanten zwischen den Eingangsgattern
    \foreach \von/\nach in {l011/l011r, l011r/l021, l021/l021r, l012/l012r, l012r/l022, l022/l022r, l023/l023r, l023r/l031, l031/l031r}
       \draw[edge] (\von) -- (\nach) ; 
 
    % die Kanten von slice 3 zu slice 4
    \foreach \von/\nach in {l11/l011, l12/l012, l13/l023}
       \draw[edge] (\von.north) -- (\nach.south) ; 
    
    % die Kanten von slice 3 zu slice 3
    \foreach \von/\nach in {l11/l11r, l12/l12r, l13/l13r}
       \draw[edge] (\von) -- (\nach) ; 
    
    % die Kanten von slice 2 zu slice 3
    \foreach \von/\nach in {l211/l11, l221/l11,
                            l211/l12, l212/l12, l221/l12,
                            l231/l13, l232/l12, l232/l13, l233/l13}
       \draw[edge] (\von.north) -- (\nach.south) ; 

    % die Kanten von slice 1 zu slice 2
    \foreach \von/\nach in {l31/l221, l32/l211, l33/l212}
       \draw[edge] (\von.north) -- (\nach.south) ; 

    % die Kanten von slice 1 zu slice 1
    \foreach \von/\nach in {l31/l31r, l32/l32r, l33/l33r}
       \draw[edge] (\von) -- (\nach) ; 
 
     % die Kanten von slice 0 zu slice 1
    \foreach \von/\nach in {l41/l31, l41/l32, l41/l33}
       \draw[edge] (\von.north) -- (\nach.south) ; 

    % die Kanten zwischen den Gattern in slice 2
    \foreach \von/\nach in {l221/l221r, l221r/l231, l231/l231r, l211/l211r, l211r/l232, l232/l232r,
                            l212/l212r, l212r/l233, l233/l233r}
       \draw[edge] (\von) -- (\nach) ; 

    % die Kanten aus den übrigen Gattern des Schaltkreises
    \foreach \nach/\von in {l41r/l41}                                
       \draw[edge] (\von) -- (\nach) ; 
       
    \begin{pgfonlayer}{background}
      \draw[ckante,draw=gray!30] (l41) -- (l32) -- (l32r) ; 
      \draw[ckante,draw=black!50] (l32.north) -- (l211.south);
           \draw[ckante,draw=black!50] (l211.east) -- (l211r) -- (l232) -- (l232r); 
      \foreach \ee in {l232r,l021r,l022r} 
         \draw (\ee) edge[tinyloopabove,ckante,draw=black!50,-] (\ee) ;
      \foreach \ee in {l32r,l11r,l12r} 
         \draw (\ee) edge[tinyloopabove,ckante,draw=gray!30,-] (\ee) ;
   
      \draw[ckante,draw=gray!30] (l211.north) -- (l11.south);  \draw[ckante,draw=gray!30] (l11.east)-- (l11r) ;   
      \draw[ckante,draw=gray!30] (l232.north) -- (l12.south);  \draw[ckante,draw=gray!30] (l12.east)-- (l12r) ;   
      \draw[ckante,draw=black!50] (l11.north) -- (l011.south);
            \draw[ckante,draw=black!50] (l011.east) -- (l011r) -- (l021) -- (l021r) ;   
      \draw[ckante,draw=black!50] (l12.north) -- (l012.south);
            \draw[ckante,draw=black!50] (l012.east)-- (l012r) -- (l022) -- (l022r) ;   
    \end{pgfonlayer}
     
\end{tikzpicture}
}


% Ein Kripke-Modell, das aus \layeredcircuitveeone entsteht,
% wenn die oder-Gatter in Serie geschaltet werden -- endgültig Version
\newcommand{\EUfromGl}{%
\begin{tikzpicture}[circuit logic US,baseline=(l41.base)]
%\tikzstyle{vertex}=[circle,draw=black,thick,minimum size=12pt,inner sep=0pt]
\tikzstyle{edge} = [draw,thick,niceArrows]
\tikzstyle{tinyloopabove} = [draw,niceArrows,thick,in=-15,out=15,min distance=3mm,looseness=8]
\tikzstyle{vertex}=[rectangle,rounded corners,draw=black,thick,minimum size=13pt,minimum height=20pt,inner sep=0mm,fill=white]

    \matrix[column sep=5mm,row sep=3mm,ampersand replacement=\&,matrix anchor=south] at (0,0) 
    {
     \node {$V_4\cup\hat{V}_4$:} ; \& 
       \node (l01) {} ;  \node[vertex,xshift=-12mm] (l011) at (l01) {\knoteninhalt{$s_4$\\$t$}} ; \node[vertex,xshift=-4mm] (l011r) at (l01) {\knoteninhalt{$\hat{s}_4$}} ;  
                         \node[vertex,xshift=4mm] (l021) at (l01) {\knoteninhalt{$s_4$\\$t$}} ;  \node[vertex,xshift=12mm] (l021r) at (l01) {\knoteninhalt{$\hat{e}_4$}} ;  \& 
       \node (l02) {} ;  \node[vertex,xshift=-12mm] (l012) at (l02) {\knoteninhalt{$s_4$\\$t$}} ;  \node[vertex,xshift=-4mm] (l012r) at (l02) {\knoteninhalt{$\hat{s}_4$}} ;  
                         \node[vertex,xshift=4mm] (l022) at (l02) {\knoteninhalt{$s_4$\\$t$}} ;  \node[vertex,xshift=12mm] (l022r) at (l02) {\knoteninhalt{$\hat{e}_4$}} ;  \& 
       \node (l03) {} ;  \node[vertex,xshift=-12mm] (l023) at (l03) {\knoteninhalt{$s_4$\\$t$}} ;  \node[vertex,xshift=-4mm] (l023r) at (l03) {\knoteninhalt{$\hat{s}_4$}} ;  
                         \node[vertex,xshift=4mm] (l031) {\knoteninhalt{$s_4$}} ; \node[vertex,xshift=12mm] (l031r) {\knoteninhalt{$\hat{e}_4$}} ; \\ 
                         
     \node {$V_3\cup\hat{V}_3$:} ; \& 
       \node[vertex] (l11) {\knoteninhalt{$s_3$}} ; \node[vertex,xshift=12mm] (l11r) at (l11) {\knoteninhalt{$\hat{e}_3$}} ; \& 
       \node[vertex] (l12) {\knoteninhalt{$s_3$}} ; \node[vertex,xshift=12mm] (l12r) at (l12) {\knoteninhalt{$\hat{e}_3$}} ; \& 
       \node[vertex] (l13) {\knoteninhalt{$s_3$}} ; \node[vertex,xshift=12mm] (l13r) at (l13) {\knoteninhalt{$\hat{e}_3$}} ;\\
     
     \node {$V_2\cup\hat{V}_2$:} ; \& 
       \node (l21) {} ; \node[vertex,xshift=-12mm] (l221) at (l21) {\knoteninhalt{$s_2$}} ;  \node[vertex,xshift=-4mm] (l221r) at (l21) {\knoteninhalt{$\hat{s}_2$}} ;  
                        \node[vertex,xshift=4mm] (l231) at (l21) {\knoteninhalt{$s_2$}} ; \node[vertex,xshift=12mm] (l231r) at (l21) {\knoteninhalt{$\hat{e}_2$}} ; \& 
       \node (l22) {} ; \node[vertex,xshift=-12mm] (l211) at (l22) {\knoteninhalt{$s_2$}} ;  \node[vertex,xshift=-4mm] (l211r) at (l22) {\knoteninhalt{$\hat{s}_2$}} ;  
                        \node[vertex,xshift=4mm] (l232) at (l22) {\knoteninhalt{$s_2$}} ;  \node[vertex,xshift=12mm] (l232r) at (l22) {\knoteninhalt{$\hat{e}_2$}} ; \& 
       \node (l23) {} ; % \node[vertex,xshift=-4mm] (l222) at (l23) {\knoteninhalt{$s_2$}} ; \node[vertex,xshift=4mm] (l222r) at (l23) {\knoteninhalt{$\hat{s}_2$}} ; 
                        \node[vertex,xshift=-12mm] (l212) at (l23) {\knoteninhalt{$s_2$}} ; \node[vertex,xshift=-4mm] (l212r) at (l23) {\knoteninhalt{$\hat{s}_2$}} ; 
                        \node[vertex,xshift=4mm] (l233) at (l23) {\knoteninhalt{$s_2$}} ; \node[vertex,xshift=12mm] (l233r) at (l23) {\knoteninhalt{$\hat{e}_2$}} ; \\
     \node {$V_1\cup \hat{V}_1$:} ; \& 
       \node[vertex] (l31) {\knoteninhalt{$s_1$}} ; \node[vertex,xshift=12mm] (l31r) at (l31) {\knoteninhalt{$\hat{e}_1$}} ; \& 
       \node[vertex] (l32) {\knoteninhalt{$s_1$}} ; \node[vertex,xshift=12mm] (l32r) at (l32) {\knoteninhalt{$\hat{e}_1$}} ; \& 
       \node[vertex] (l33) {\knoteninhalt{$s_1$}} ; \node[vertex,xshift=12mm] (l33r) at (l33) {\knoteninhalt{$\hat{e}_1$}} ; \\
       
     \node {$V_0\cup\hat{V}_0$:} ; \&  
      \& \node[vertex] (l41) {\knoteninhalt{$s_0$}} ; \node[vertex,xshift=8mm] (l41r) at (l41) {\knoteninhalt{$\hat{e}_0$}} ; \& \\
    } ;

    \foreach \zz in {l021r,l022r,l031r,l231r,l232r,l233r,l41r,l11r,l12r,l13r,l31r,l32r,l33r}
      \draw (\zz) edge[tinyloopabove] (\zz) ;

    % die Kanten zwischen den Eingangsgattern
    \foreach \von/\nach in {l011/l011r, l011r/l021, l021/l021r, l012/l012r/, l012r/l022, l022/l022r, l023/l023r, l023r/l031, l031/l031r}
       \draw[edge] (\von) -- (\nach) ; 
 
    % die Kanten von slice 3 zu slice 4
    \foreach \von/\nach in {l11/l011, l12/l012, l13/l023}
       \draw[edge] (\von.north) -- (\nach.south) ; 
    
    % die Kanten von slice 3 zu slice 3
    \foreach \von/\nach in {l11/l11r, l12/l12r, l13/l13r}
       \draw[edge] (\von) -- (\nach) ; 
    
    % die Kanten von slice 2 zu slice 3
    \foreach \von/\nach in {l211/l11, l221/l11, 
                            l211/l12, l212/l12, l221/l12, 
                            l231/l13, l232/l12, l232/l13, l233/l13}
       \draw[edge] (\von.north) -- (\nach.south) ; 

    % die Kanten von slice 1 zu slice 2
    \foreach \von/\nach in {l31/l221, l32/l211, l33/l212}
       \draw[edge] (\von.north) -- (\nach.south) ; 

    % die Kanten von slice 1 zu slice 1
    \foreach \von/\nach in {l31/l31r, l32/l32r, l33/l33r}
       \draw[edge] (\von) -- (\nach) ; 
 
     % die Kanten von slice 0 zu slice 1
    \foreach \von/\nach in {l41/l31, l41/l32, l41/l33}
       \draw[edge] (\von.north) -- (\nach.south) ; 

    % die Kanten zwischen den Gattern in slice 2
    \foreach \von/\nach in {l221/l221r, l221r/l231, l231/l231r, l211/l211r, l211r/l232, l232/l232r,
                            l212/l212r, l212r/l233, l233/l233r}
       \draw[edge] (\von) -- (\nach) ; 

    % die Kanten aus den übrigen Gattern des Schaltkreises
    \foreach \nach/\von in {l41r/l41}                                
       \draw[edge] (\von) -- (\nach) ; 
       
    \begin{pgfonlayer}{background}
      \draw[ckante,draw=gray!30] (l41) -- (l32) -- (l32r) ; 
      \draw[ckante,draw=black!50] (l32.north) -- (l211.south);
           \draw[ckante,draw=black!50] (l211.east) -- (l211r) -- (l232) -- (l232r); 
      \foreach \ee in {l232r,l021r,l022r} 
         \draw (\ee) edge[tinyloopabove,ckante,draw=black!50,-] (\ee) ;
      \foreach \ee in {l32r,l11r,l12r} 
         \draw (\ee) edge[tinyloopabove,ckante,draw=gray!30,-] (\ee) ;
   
      \draw[ckante,draw=gray!30] (l211.north) -- (l11.south);  \draw[ckante,draw=gray!30] (l11.east)-- (l11r) ;   
      \draw[ckante,draw=gray!30] (l232.north) -- (l12.south);  \draw[ckante,draw=gray!30] (l12.east)-- (l12r) ;   
      \draw[ckante,draw=black!50] (l11.north) -- (l011.south);
            \draw[ckante,draw=black!50] (l011.east) -- (l011r) -- (l021) -- (l021r) ;   
      \draw[ckante,draw=black!50] (l12.north) -- (l012.south);
            \draw[ckante,draw=black!50] (l012.east)-- (l012r) -- (l022) -- (l022r) ;   
    \end{pgfonlayer}
     
\end{tikzpicture}
}




%% Das Kripke-Modell, das aus dem \layeredcircuit durch Umdrehen der Kanten ensteht
\newcommand{\layeredKmodel}{%
\begin{tikzpicture}[baseline=(KKK.base),niceArrows]
\tikzstyle{tinyloopabove} = [draw,niceArrows,thick,in=75,out=105,min distance=3mm,looseness=8]

    \matrix(m)[column sep=7mm,row sep=9mm,ampersand replacement=\&,matrix anchor=south] at (0,0)
    {
     \node[vertex] (l01) {} ; \& \node[vertex] (l02) {} ; \& \node[vertex] (l03) {} ;  \\
     \node[vertex] (l11) {}    ; \& \node[vertex] (l12) {} ; \& \node[vertex] (l13) {} ;  \\
     \node[vertex] (l21) {}    ; \& \node[vertex] (l22) {} ; \& \node[vertex] (l23) {} ; \\
     \node[vertex] (l31) {}    ; \& \node[vertex] (l32) {} ; \& \node[vertex] (l33) {} ; \\
      \& \node[vertex,label=below:{$out$}] (l41) {} ; \& \\
    } ;

    \foreach \zz in {l01,l02,l03}
      \draw (\zz) edge[tinyloopabove] (\zz) ;
    
    % die Tripel (z.B.  l01/l11/2) sind aus \layeredcircuit kopiert
    % die Kanten aus den Eingangsgattern
    \foreach \von/\nach/\in in {l01/l11/2, l02/l11/1, l01/l12/2, l02/l12/1, l03/l13/1, l02/l13/2}
       \draw[revedge] (\von) -- (\nach) ; 
    
    % die Kanten aus den übrigen Gattern des Schaltkreises
    \foreach \von/\nach/\in in {l11/l21/2, l11/l22/2, l12/l21/1, l12/l22/1, l13/l23/1,
                                l21/l32/2, l21/l33/3, l22/l31/2, l22/l33/1, l23/l31/1, l23/l32/1, l23/l33/3,
                                l31/l41/3, l32/l41/2, l33/l41/1}                                
       \draw[revedge] (\von) -- (\nach) ; 
    
    \node (KKK) at (0,-1) {Graph $G_s(C)$} ;
 
\end{tikzpicture}
}



% Ein Schaltkreis-Beispiel mit Markierungen für die Gatter mit Ausgabe 1
\newcommand{\schaltkreisbsp}{%
\begin{tikzpicture}[circuit logic US,baseline=(CCC.base)]
\tikzstyle{edge} = [draw,thick,niceArrows]

    \matrix[column sep=7mm,row sep=7mm,ampersand replacement=\&,matrix anchor=south] at (0,0) 
    {
     \node (e1) {$1$} ; \& \node(e2) {$1$} ;\& \node(e3) {$0$} ; \\
     \node[goodandgate2] (d1) {} ; \& \node[goodandgate2] (d2) {} ; \& \node[mmandgate2] (d3) {} ; \\
     \node[goodorgate2] (c1) {} ; \& \node[goodorgate2] (c2) {} ; \& \node[mmorgate2] (c3) {} ; \\
     \node[mmandgate2] (b1) {} ; \& \node[mmandgate2] (b2) {} ; \& \node[goodandgate2] (b3) {} ; \\
      \& \node[goodorgate3] (a1) {} ; \& \\
    } ;


    \draw[edge] (e1) -- (d1.input 2) ;
    \draw[edge] (e2) -- (d1.input 1) ;
    \draw[edge] (e1) -- (d2.input 2) ;
    \draw[edge] (e2) -- (d2.input 1) ;
    \draw[edge] (e3) -- (d3.input 1) ;
    \draw[edge] (e2) -- (d3.input 2) ;
    
    \draw[edge] (d1.output) -- (c1.input 2) ; 
    \draw[edge] (d1.output) -- (c2.input 2) ; 
    \draw[edge] (d2.output) -- (c1.input 1) ; 
    \draw[edge] (d2.output) -- (c2.input 1) ; 
%    \draw[edge] (d3.output) -- (c2.input 1) ; 
    \draw[edge] (d3.output) -- (c3.input 1) ; 

    \draw[edge] (c1.output) -- (b2.input 2) ; 
    \draw[edge] (c1.output) -- (b3.input 2) ;
    \draw[edge] (c2.output) -- (b1.input 2) ; 
    \draw[edge] (c2.output) -- (b3.input 1) ; 
    \draw[edge] (c3.output) -- (b1.input 1) ; 
    \draw[edge] (c3.output) -- (b2.input 1) ; 
     
    \draw[edge] (b1.output) -- (a1.input 3) ; 
    \draw[edge] (b2.output) -- (a1.input 2) ; 
    \draw[edge] (b3.output) -- (a1.input 1) ; 
    
    \draw[edge,thick] (a1.output) -- ++(down:3mm) ;
    
    \node (CCC) at (0,-0.7) {mon. circuit $C$} ;
    
    \begin{pgfonlayer}{background}
      \draw[ckante] (e1) -- (d1.input 2) ;
      \draw[ckante] (e2) -- (d1.input 1) ;
      \draw[ckante] (e1) -- (d2.input 2) ;
      \draw[ckante] (e2) -- (d2.input 1) ;
      
      \draw[ckante] (d1.output) -- (c2.input 2) ; \draw[ckante] (c2.output) -- (b3.input 2) ;
      \draw[ckante] (d2.output) -- (c1.input 1) ; \draw[ckante] (c1.output) -- (b3.input 1) ;

      \draw[ckante] (b3.output) -- (a1.input 1) ;
   
    \end{pgfonlayer}
    
\end{tikzpicture}
}


%% Das Kripke-Modell, das aus dem Schaltkreis entsteht
\newcommand{\kripkemodelbsp}{%
\begin{tikzpicture}[baseline=(KKK.base),niceArrows]

    \matrix(m)[column sep=7mm,row sep=9mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node[vertex] (e1) {$t$} ; \& \node[vertex] (e2) {$t$} ; \& \node[vertex] (e3) { } ; \\[-3mm]
     \node[vertex] (d1) {}    ; \& \node[vertex] (d2) {} ; \& \node[vertex] (d3) {} ; \\
     \node[vertex] (c1) {}    ; \& \node[vertex] (c2) {} ; \& \node[vertex] (c3) {} ; \\
     \node[vertex] (b1) {}    ; \& \node[vertex] (b2) {} ; \& \node[vertex] (b3) {} ; \\
      \& \node[vertex,label=below:{$out$}] (a1) {} ; \& \\
    } ;

    \draw[revedge] (e1) -- (d1) ;
    \draw[revedge] (e2) -- (d1) ;
    \draw[revedge] (e1) -- (d2) ;
    \draw[revedge] (e2) -- (d2) ;
    \draw[revedge] (e3) -- (d3) ;
    \draw[revedge] (e2) -- (d3) ;
    
    \draw[revedge] (d1) -- (c1) ; 
    \draw[revedge] (d1) -- (c2) ; 
    \draw[revedge] (d2) -- (c1) ; 
%    \draw[revedge] (d2) -- (c3) ; 
    \draw[revedge] (d2) -- (c2) ; 
    \draw[revedge] (d3) -- (c3) ; 

    \draw[revedge] (c1) -- (b2) ; 
    \draw[revedge] (c1) -- (b3) ;
    \draw[revedge] (c2) -- (b1) ; 
    \draw[revedge] (c2) -- (b3) ; 
    \draw[revedge] (c3) -- (b1) ; 
    \draw[revedge] (c3) -- (b2) ; 
     
    \draw[revedge] (b1) -- (a1) ; 
    \draw[revedge] (b2) -- (a1) ; 
    \draw[revedge] (b3) -- (a1) ; 
    
    \node (KKK) at (0,-1) {Kripke model $K_C$} ;
 
\end{tikzpicture}
}

%% Das Kripke-Modell fuer die AC1-Haerte von CTL-MC(EF,\oplus), das aus dem Schaltkreis entsteht
\newcommand{\EFoplusACeinshart}{%
\begin{tikzpicture}[niceArrows]
\tikzstyle{tinyloopabove} = [draw,niceArrows,thick,in=75,out=105,min distance=3mm,looseness=8]

    \matrix(m)[column sep=9mm,row sep=3mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node {$W_0$:} ; \&
     \node[vertex] (e1) {$z_0,t$} ; \& \node[vertex] (e2) {$z_0,t$} ; \& \node[vertex] (e3) {$z_0$} ; 
               \&[8mm] \node[vertex,label=east:{$a_0$}] (a_0) {$z_0$} ; \& \node[vertex,label=east:{$b_0$}] (b_0) {$z_0,t$} ;   \\
     \node {$W_1$:} ; \&
     \node[vertex] (d1) {$z_1$}    ; \& \node[vertex] (d2) {$z_1$} ; \& \node[vertex] (d3) {$z_1$} ; 
               \&  \node[vertex,label=east:{$a_1$}] (a_1) {$z_1$} ; \& \node[vertex,label=east:{$b_1$}] (b_1) {$z_1$} ;   \\
     \node {$W_2$:} ; \&
     \node[vertex] (c1) {$z_2$}    ; \& \node[vertex] (c2) {$z_2$} ; \& \node[vertex] (c3) {$z_2$} ; 
               \&  \node[vertex,label=east:{$a_2$}] (a_2) {$z_2$} ; \& \node[vertex,label=east:{$b_2$}] (b_2) {$z_2$} ; \\
     \node {$W_3$:} ; \&
     \node[vertex] (b1) {$z_3$}    ; \& \node[vertex] (b2) {$z_3$} ; \& \node[vertex] (b3) {$z_3$} ; 
               \&  \node[vertex,draw=gray,label=east:{$a_3$}] (a_3) {$z_3$} ; \& \node[vertex,label=east:{$b_3$}] (b_3) {$z_3$} ; \\
     \node {$W_4$:} ; \&
      \& \node[vertex,label=below:{$s$}] (a1) {$z_4$} ; \&  
               \&  \node[vertex,draw=gray,label=east:{$a_4$}] (a_4) {$z_4$} ; \& \node[vertex,draw=gray,label=east:{$b_4$}] (b_4) {$z_4$} ; \\
    } ;

    \foreach \zz in {e1,e2,e3,a_0,b_0}
      \draw (\zz) edge[tinyloopabove] (\zz) ;
      
    \draw[edge,draw=gray] (a_4) -- (a_3) ;  \draw[edge,draw=gray] (a_3) -- (a_2) ;  \draw[edge] (a_2) -- (a_1) ;  \draw[edge] (a_1) -- (a_0) ;  
    \draw[edge,draw=gray] (b_4) -- (b_3) ; \draw[edge] (b_3) -- (b_2) ;  \draw[edge] (b_2) -- (b_1) ;  \draw[edge] (b_1) -- (b_0) ;  
    \draw[edge,draw=gray] (a_4) -- (b_3) ;
    
    \foreach \zz in {d1,d2,d3,b_1}
      \draw[edge] (\zz) --  (a_0) ;
    \foreach \zz in {c1,c2,c3,a_2}
      \draw[edge] (\zz) --  (b_1) ;
    \foreach \zz in {b1,b2,b3,b_3}
      \draw[edge] (\zz) --  (a_2) ;

    \draw[edge] (a1) -- (b_3) ;   

    \draw[revedge] (e1) -- (d1) ;
    \draw[revedge] (e2) -- (d1) ;
    \draw[revedge] (e1) -- (d2) ;
    \draw[revedge] (e2) -- (d2) ;
    \draw[revedge] (e3) -- (d3) ;
    \draw[revedge] (e2) -- (d3) ;
    
    \draw[revedge] (d1) -- (c1) ; 
    \draw[revedge] (d1) -- (c2) ; 
    \draw[revedge] (d2) -- (c1) ; 
%    \draw[revedge] (d2) -- (c3) ; 
    \draw[revedge] (d2) -- (c2) ; 
    \draw[revedge] (d3) -- (c3) ; 

    \draw[revedge] (c1) -- (b2) ; 
    \draw[revedge] (c1) -- (b3) ;
    \draw[revedge] (c2) -- (b1) ; 
    \draw[revedge] (c2) -- (b3) ; 
    \draw[revedge] (c3) -- (b1) ; 
    \draw[revedge] (c3) -- (b2) ; 
     
    \draw[revedge] (b1) -- (a1) ; 
    \draw[revedge] (b2) -- (a1) ; 
    \draw[revedge] (b3) -- (a1) ; 
    
%    \node (KKK) at (0,-1) {Kripke model $K_C$} ;
 
\end{tikzpicture}
}


%% Das intuitionistische Kripke-Modell, das aus dem Schaltkreis entsteht
\newcommand{\kripkemodelint}{%
\begin{tikzpicture}[baseline=(KKK.base),niceArrows]
\tikzstyle{vertex}=[rectangle,draw=black,thick,minimum size=16pt,inner sep=2pt]
\tikzstyle{goodvertex}=[rectangle,draw=black,fill=black!20,thick,minimum size=16pt,inner sep=2pt]
\tikzstyle{fvertex}=[rectangle,thick,minimum width=40mm,inner sep=2pt]

\tikzstyle{tinyloopabove} = [draw,niceArrows,thick,in=75,out=105,min distance=3mm,looseness=8]
\tikzstyle{tinyloopright} = [draw,niceArrows,thick,in=-7,out=7,min distance=5mm,looseness=8]

    \matrix(m)[column sep=2mm,row sep=7mm,ampersand replacement=\&,matrix anchor=south,column 5/.style={anchor=base west}] at (0,-0.4)
    {
        \node {$4$} ; \& \node[goodvertex] (e1) {$a_1,a_2,a_3,a_4$} ; \& \node[goodvertex] (e2) {$a_1,a_2,a_3,a_4$} ; \& 
             \node[vertex] (e3) { $t,a_1,a_2,a_3,a_4$} ; 
            \&[2mm] \node {$t\iimpl a_5$} ; \\[-3mm]
        \node {$3$} ; \& \node[vertex] (d1) {$a_1,a_2,a_3$}    ; \& \node[vertex] (d2) {$a_1,a_2,a_3$} ; \& \node[goodvertex] (d3) {$a_1,a_2,a_3$} ; 
       \& \node {$(t\iimpl a_5)\iimpl a_4$} ; \\
        \node {$2$} ;\& \node[goodvertex] (c1) {$a_1,a_2$}    ; \& \node[goodvertex] (c2) {$a_1,a_2$} ; \& \node[vertex] (c3) {$a_1,a_2$} ; 
       \& \node {$((t\iimpl a_5)\iimpl a_4)\iimpl a_3$} ;\\
       \node {$1$} ; \& \node[goodvertex] (b1) {$a_1$}    ; \& \node[goodvertex] (b2) {$a_1$} ; \& \node[vertex] (b3) {$a_1$} ;
       \& \node {$(((t\iimpl a_5)\iimpl a_4)\iimpl a_3)\iimpl a_2$} ;\\
       \node {$0$} ; \& \& \node[goodvertex,label=below:{$out$}] (a1) {} ; \&        \&  \node (a) { } ;\\
    } ;
 
    \node[xshift=19mm] at (a) {$((((t\iimpl a_5)\iimpl a_4)\iimpl a_3)\iimpl a_2)\iimpl a_1$} ;
    
    \draw (e1) edge[tinyloopabove] (e1) ;
    \draw (e2) edge[tinyloopabove] (e2) ;
    \draw (e3) edge[tinyloopabove] (e3) ;
    
    \foreach \vv in {d1,d2,d3,c1,c2,c3,b1,b2,b3,a1}
      \draw (\vv) edge[tinyloopright] (\vv) ;

    \draw[revedge] (e1) -- (d1) ;
    \draw[revedge] (e2) -- (d1) ;
    \draw[revedge] (e1) -- (d2) ;
    \draw[revedge] (e2) -- (d2) ;
    \draw[revedge] (e3) -- (d3) ;
    \draw[revedge] (e2) -- (d3) ;
    
    \draw[revedge] (d1) -- (c1) ; 
    \draw[revedge] (d1) -- (c2) ; 
    \draw[revedge] (d2) -- (c1) ; 
%    \draw[revedge] (d2) -- (c3) ; 
    \draw[revedge] (d2) -- (c2) ; 
    \draw[revedge] (d3) -- (c3) ; 

    \draw[revedge] (c1) -- (b2) ; 
    \draw[revedge] (c1) -- (b3) ;
    \draw[revedge] (c2) -- (b1) ; 
    \draw[revedge] (c2) -- (b3) ; 
    \draw[revedge] (c3) -- (b1) ; 
    \draw[revedge] (c3) -- (b2) ; 
     
    \draw[revedge] (b1) -- (a1) ; 
    \draw[revedge] (b2) -- (a1) ; 
    \draw[revedge] (b3) -- (a1) ; 
    
    \node (KKK) at (0,-1) {Intuitionistic Kripke model $I_C$} ;
 
\end{tikzpicture}
}

%% Das andere Kripke-Modell, das aus dem SAC1-Schaltkreis entsteht
\newcommand{\kripkemodelbspzwei}{%
\begin{tikzpicture}[baseline=(KKK.base),niceArrows]

    \matrix[column sep=2mm,row sep=9mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node (e1) {} ;
     \node[vertex,xshift=-4mm] (d1l) at (e1) {$t,l$} ; \node[vertex,xshift=4mm] (d1r) at (e1) {$t,r$} ;  \&
     \node (e2) {} ;
     \node[vertex,xshift=-4mm] (d2l) at (e2) {$t,l$} ; \node[vertex,xshift=4mm] (d2r) at (e2) {$t,r$} ;  \&
     \node (e3) {} ;
     \node[vertex,xshift=-4mm] (d3l) at (e3) {$l$} ; \node[vertex,xshift=4mm] (d3r) at (e3) {$r$} ;  \\
     
     \node[vertex] (d1) {}    ; \& \node[vertex] (d2) {} ; \& \node[vertex] (d3) {} ; \\
     \node (c1) {} ;
     \node[vertex,xshift=-4mm] (b1l) at (c1) {$l$} ; \node[vertex,xshift=4mm] (b1r) at (c1) {$r$} ;  \&
     \node (c2) {} ;
     \node[vertex,xshift=-4mm] (b2l) at (c2) {$l$} ; \node[vertex,xshift=4mm] (b2r) at (c2) {$r$} ;  \&
     \node (c3) {} ;
     \node[vertex,xshift=-4mm] (b3l) at (c3) {$l$} ; \node[vertex,xshift=4mm] (b3r) at (c3) {$r$} ;  \\
     \node[vertex] (b1) {}    ; \& \node[vertex] (b2) {} ; \& \node[vertex] (b3) {} ; \\
      \& \node[vertex,label=below:{$out$}] (a1) {} ; \& \\
    } ;

    \draw[revedge] (d1l) -- (d1) ;
    \draw[revedge] (d1r) -- (d1) ;
    \draw[revedge] (d2l) -- (d2) ;
    \draw[revedge] (d2r) -- (d2) ;
    \draw[revedge] (d3l) -- (d3) ;
    \draw[revedge] (d3r) -- (d3) ;
    
    \draw[revedge] (d1) -- (b2l) ; 
    \draw[revedge] (d2) -- (b2l) ; 
    \draw[revedge] (d1) -- (b3l) ; 
    \draw[revedge] (d1) -- (b1l) ; 
    \draw[revedge] (d1) -- (b3r) ; 
    \draw[revedge] (d2) -- (b3r) ; 
    \draw[revedge] (d2) -- (b3l) ; 
%    \draw[revedge] (d2) -- (b1r) ; 
%    \draw[revedge] (d2) -- (b2r) ; 
    \draw[revedge] (d2) -- (b1l) ; 
    \draw[revedge] (d3) -- (b1r) ; 
    \draw[revedge] (d3) -- (b2r) ; 

    \draw[revedge] (b2l) -- (b2) ; 
    \draw[revedge] (b3l) -- (b3) ;
    \draw[revedge] (b1r) -- (b1) ; 
    \draw[revedge] (b3r) -- (b3) ; 
    \draw[revedge] (b1l) -- (b1) ; 
    \draw[revedge] (b2r) -- (b2) ; 
     
    \draw[revedge] (b1) -- (a1) ; 
    \draw[revedge] (b2) -- (a1) ; 
    \draw[revedge] (b3) -- (a1) ; 

    \node (KKK) at (0,-1) {Kripke model $\hat{K}_C$} ;
    
\end{tikzpicture}
}

%% Das andere Kripke-Modell, das aus dem SAC1-Schaltkreis entsteht
\newcommand{\EGistPhart}{%
\begin{tikzpicture}[baseline=(KKK.base),vertex/.style={draw=black,circle,inner sep=.7mm,fill=white}]

    \matrix[column sep=2mm,row sep=6mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node (e1) {} ;
     \node[vertex,xshift=-6mm] (d1l) at (e1) {$s_4,t$} ; \node[vertex,xshift=6mm] (d1r) at (e1) {$s_4,t$} ;  \&
     \node (e2) {} ;
     \node[vertex,xshift=-5mm] (d2l) at (e2) {$s_4,t$} ; \node[vertex,xshift=6mm] (d2r) at (e2) {$s_4,t$} ;  \&
     \node (e3) {} ;
     \node[vertex,xshift=-4mm] (d3l) at (e3) {$s_4$} ; \node[vertex,xshift=4mm] (d3r) at (e3) {$s_4$} ;  \&[12mm] \node[vertex] (t4) {$t_4$} ;\\
     
     \node[vertex] (d1) {$s_3$}    ; \& \node[vertex] (d2) {$s_3$} ; \& \node[vertex] (d3) {$s_3$} ; \& \node[vertex] (t3) {$t_3$} ;\\[2mm]
     \node (c1) {} ;
     \node[vertex,xshift=-5mm] (b1l) at (c1) {$s_2$} ; \node[vertex,xshift=5mm] (b1r) at (c1) {$s_2$} ;  \&
     \node (c2) {} ;
     \node[vertex,xshift=-5mm] (b2l) at (c2) {$s_2$} ; \node[vertex,xshift=5mm] (b2r) at (c2) {$s_2$} ;  \&
     \node (c3) {} ;
     \node[vertex,xshift=-5mm] (b3l) at (c3) {$s_2$} ; \node[vertex,xshift=5mm] (b3r) at (c3) {$s_2$} ;  \& \node[vertex] (t2) {$t_2$} ; \\
     \node[vertex] (b1) {$s_1$}    ; \& \node[vertex] (b2) {$s_1$} ; \& \node[vertex] (b3) {$s_1$} ; \& \node[vertex] (t1) {$t_1$} ; \\
      \& \node[vertex,label=below:{$out$}] (a1) {$s_0$} ; \& \\
    } ;

    % die horizontalen Kanten für die Und-Gatter-Simulation
    \foreach \von/\zu in {{d1l/d1r}, {d2l/d2r}, {d3l/d3r},
                          {b1l/b1r}, {b2l/b2r}, {b3l/b3r}}
       \draw[edge,niceArrows] (\von) -- (\zu) ;
       
    % die loops
    \foreach \knoten in {t1,t2,t3,t4}
       \draw[edge,niceArrows] (\knoten) edge[loop right] (\knoten) ;
       
    % die nach unten geschwungenen Kanten zu den t-Knoten
    \foreach \von/\zu/\wie in {{b1/t1/21}, {b2/t1/18}, {b3/t1/15},
                               {b1r/t2/25}, {b2r/t2/23}, {b3r/t2/20}}
       \draw[edge,niceArrows] (\von) edge[bend right=\wie] (\zu) ;

    % die nach oben geschwungenen Kanten zu den t-Knoten
    \foreach \von/\zu/\wie in {{d1/t3/21}, {d2/t3/18}, {d3/t3/15},
                               {d1r/t4/25}, {d2r/t4/23}, {d3r/t4/20}}
       \draw[edge,niceArrows] (\von) edge[bend left=\wie] (\zu) ;
       
    \draw[revedge] (d1l) -- (d1) ;
%    \draw[revedge] (d1r) -- (d1) ;
    \draw[revedge] (d2l) -- (d2) ;
%    \draw[revedge] (d2r) -- (d2) ;
    \draw[revedge] (d3l) -- (d3) ;
%    \draw[revedge] (d3r) -- (d3) ;
    
    \draw[revedge] (d1) -- (b2l) ; 
    \draw[revedge] (d2) -- (b2l) ; 
    \draw[revedge] (d1) -- (b3l) ; 
    \draw[revedge] (d1) -- (b1l) ; 
    \draw[revedge] (d1) -- (b3r) ; 
    \draw[revedge] (d3) -- (b3r) ; 
    \draw[revedge] (d2) -- (b3l) ; 
    \draw[revedge] (d2) -- (b1r) ; 
    \draw[revedge] (d2) -- (b2r) ; 
    \draw[revedge] (d3) -- (b1l) ; 
    \draw[revedge] (d3) -- (b1r) ; 
    \draw[revedge] (d3) -- (b2r) ; 

    \draw[revedge] (b2l) -- (b2) ; 
    \draw[revedge] (b3l) -- (b3) ;
%    \draw[revedge] (b1r) -- (b1) ; 
%    \draw[revedge] (b3r) -- (b3) ; 
    \draw[revedge] (b1l) -- (b1) ; 
%    \draw[revedge] (b2r) -- (b2) ; 
     
    \draw[revedge] (b1) -- (a1) ; 
    \draw[revedge] (b2) -- (a1) ; 
    \draw[revedge] (b3) -- (a1) ; 

    \node (KKK) at (0,-1) {Kripke model $\hat{C}_{\EG}$} ;
    
    \begin{pgfonlayer}{background}
      \draw[dkante,black!23,densely dashed] (a1) -- (b3) edge[bend right=15] (t1) ;
      \draw[dkante,black!23,densely dashed] (t1) edge[loopcover] (t1) ;
      
      \draw[dkante,black!35] (b3) -- (b3l) -- (b3r) edge[bend right=18] (t2) (t2) edge[loopcover] (t2) ;

      \draw[dkante,black!23,dashed] (b3r) -- (d1) edge[bend left=21] (t3) ;
      \draw[dkante,black!23,dotted] (b3l) -- (d2) edge[bend left=18] (t3) ;
      \draw[dkante,black!23,densely dotted] (t3) edge[loopcover] (t3) ;
      
      \draw[dkante,black!23] (d1) -- (d1l) -- (d1r) edge[bend left=25] (t4) ;
      \draw[dkante,black!35] (t4) edge[loopcover] (t4) ;

      \draw[dkante,black!23] (d2) -- (d2l) -- (d2r) edge[bend left=21] (t4) ;
      \draw[dkante,black!35] (t4) edge[loopcover] (t4) ;  
    \end{pgfonlayer}  
    
\end{tikzpicture}
}

%% Das andere Kripke-Modell, das aus dem SAC1-Schaltkreis entsteht, die neueste Version
\newcommand{\EGistPhartneu}{%
\begin{tikzpicture}[baseline=(KKK.base),vertex/.style={draw=black,ellipse,inner sep=.7mm,fill=white},x=1.5cm]

    \matrix[column sep=4mm,row sep=6mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node (e1) {} ;
     \node[vertex,xshift=-10mm] (d1l) at (e1) {$s_4,t$} ; \node[vertex,xshift=10mm] (d1r) at (e1) {$s_4,t$} ;  \&
     \node (e2) {} ;
     \node[vertex,xshift=-10mm] (d2l) at (e2) {$s_4,t$} ; \node[vertex,xshift=10mm] (d2r) at (e2) {$s_4,t$} ;  \&
     \node (e3) {} ;
     \node[vertex,xshift=-10mm] (d3l) at (e3) {$s_4$} ; \node[vertex,xshift=10mm] (d3r) at (e3) {$s_4$} ;  \&[12mm] \node[vertex] (t4) {$t_4$} ;\\
     
     \node[vertex] (d1) {$s_3$}    ; \& \node[vertex] (d2) {$s_3$} ; \& \node[vertex] (d3) {$s_3$} ; \& \node[vertex] (t3) {$t_3$} ;\\[2mm]
     \node[vertex] (c1) {$t_2$} ;
     \node[vertex,xshift=-9mm] (b1l) at (c1) {$s_2$} ; \node[vertex,xshift=9mm] (b1r) at (c1) {$s_2$} ;  \&
     \node[vertex] (c2) {$t_2$} ;
     \node[vertex,xshift=-9mm] (b2l) at (c2) {$s_2$} ; \node[vertex,xshift=9mm] (b2r) at (c2) {$s_2$} ;  \&
     \node[vertex] (c3) {$t_2$} ;
     \node[vertex,xshift=-9mm] (b3l) at (c3) {$s_2$} ; \node[vertex,xshift=9mm] (b3r) at (c3) {$s_2$} ;  \& \node[vertex] (t2) {$t_2$} ; \\
     \node[vertex] (b1) {$s_1$}    ; \& \node[vertex] (b2) {$s_1$} ; \& \node[vertex] (b3) {$s_1$} ; \& \node[vertex] (t1) {$t_1$} ; \\
      \& \node[vertex,label=below:{$out$}] (a1) {$s_0$} ; \& \\
    } ;

    % die horizontalen Kanten für die Und-Gatter-Simulation
    \foreach \von/\zu in {{d1l/d1r}, {d2l/d2r}, {d3l/d3r}}
       \draw[edge,niceArrows] (\von) -- (\zu) ;

    \foreach \von/\ueber/\zu in {{b1l/c1/b1r}, {b2l/c2/b2r}, {b3l/c3/b3r}}{
       \draw[edge,niceArrows] (\von)   -- (\ueber) ;
       \draw[edge,niceArrows] (\ueber) -- (\zu) ;
     }  
    % die loops
    \foreach \knoten in {t1,t2,t3,t4}
       \draw[edge,niceArrows] (\knoten) edge[loop right] (\knoten) ;
       
    % die nach unten geschwungenen Kanten zu den t-Knoten
    \foreach \von/\zu/\wie in {{b1/t1/15}, {b2/t1/15}, {b3/t1/15},
                               {b1r/t2/15}, {b2r/t2/15}, {b3r/t2/15}}
       \draw[edge,niceArrows] (\von) edge[bend right=\wie] (\zu) ;

    % die nach oben geschwungenen Kanten zu den t-Knoten
    \foreach \von/\zu/\wie in {{d1/t3/15}, {d2/t3/15}, {d3/t3/15},
                               {d1r/t4/23}, {d2r/t4/23}, {d3r/t4/20}}
       \draw[edge,niceArrows] (\von) edge[bend left=\wie] (\zu) ;
       
    \draw[revedge,niceArrows] (d1l) -- (d1) ;
%    \draw[revedge] (d1r) -- (d1) ;
    \draw[revedge,niceArrows] (d2l) -- (d2) ;
%    \draw[revedge] (d2r) -- (d2) ;
    \draw[revedge,niceArrows] (d3l) -- (d3) ;
%    \draw[revedge] (d3r) -- (d3) ;
    
   {\tikzset{niceArrows}
	    \draw[revedge] (d1) -- (b2l) ; 
	    \draw[revedge] (d2) -- (b2l) ; 
	    \draw[revedge] (d1) -- (b3l) ; 
	    \draw[revedge] (d1) -- (b1l) ; 
	    \draw[revedge] (d1) edge[out=-20, in=150] (b3r) ; 
	    \draw[revedge] (d3) -- (b3r) ; 
	    \draw[revedge] (d2) -- (b3l) ; 
%	    \draw[revedge] (d2) -- (b1r) ; 
%	    \draw[revedge] (d2) -- (b2r) ; 
	    \draw[revedge] (d3) edge[out=-150, in=30] (b1l) ; 
	    \draw[revedge] (d3) -- (b1r) ; 
	    \draw[revedge] (d3) -- (b2r) ; 
	
	    \draw[revedge] (b2l) -- (b2) ; 
	    \draw[revedge] (b3l) -- (b3) ;
	%    \draw[revedge] (b1r) -- (b1) ; 
	%    \draw[revedge] (b3r) -- (b3) ; 
	    \draw[revedge] (b1l) -- (b1) ; 
	%    \draw[revedge] (b2r) -- (b2) ; 
	     
	    \draw[revedge] (b1) -- (a1) ; 
	    \draw[revedge] (b2) -- (a1) ; 
	    \draw[revedge] (b3) -- (a1) ; 
    }

    \node (KKK) at (0,-1) {Kripke model $\hat{C}_{\EG}$} ;
    
    \begin{pgfonlayer}{background}
      \draw[dkante,black!23,densely dashed] (a1) -- (b3) edge[bend right=15] (t1) ;
      \draw[dkante,black!23,densely dashed] (t1) edge[loopcover] (t1) ;
      
      \draw[dkante,black!35] (b3) -- (b3l) -- (b3r) edge[bend right=18] (t2) (t2) edge[loopcover] (t2) ;

      \draw[dkante,black!23,densely dashed] (b3r) edge[out=150, in=-20] (d1) (d1) edge[bend left=15] (t3) ;
      \draw[dkante,black!23,densely dashed] (b3l) -- (d2) edge[bend left=15] (t3) ;
      \draw[dkante,black!23,densely dashed] (t3) edge[loopcover] (t3) ;
      
      \draw[dkante,black!23] (d1) -- (d1l) -- (d1r) edge[bend left=23] (t4) ;
      \draw[dkante,black!23] (t4) edge[loopcover] (t4) ;

      \draw[dkante,black!23] (d2) -- (d2l) -- (d2r) edge[bend left=23] (t4) ;
      \draw[dkante,black!23] (t4) edge[loopcover] (t4) ;  
    \end{pgfonlayer}  
    
\end{tikzpicture}
}



%% Das andere Kripke-Modell, das aus dem SAC1-Schaltkreis entsteht, die neueste Version
\newcommand{\EGoplusistPhart}{%
\begin{tikzpicture}[baseline=(KKK.base),vertex/.style={draw=black,ellipse,inner sep=0.4mm,fill=white}]
\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=40pt,inner sep=2pt]
    \matrix[column sep=4mm,row sep=6mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node (e1)[vertex] {$s_4,t_4$} ;
     \node[vertex,xshift=-11mm] (d1l) at (e1) {$s_4,t$} ; \node[vertex,xshift=11mm] (d1r) at (e1) {$s_4,t$} ;  \&
     \node (e2)[vertex] {$s_4,t_4$} ;
     \node[vertex,xshift=-11mm] (d2l) at (e2) {$s_4,t$} ; \node[vertex,xshift=11mm] (d2r) at (e2) {$s_4,t$} ;  \&
     \node (e3)[vertex] {$s_4,t_4$} ;
     \node[vertex,xshift=-11mm] (d3l) at (e3) {$s_4$} ; \node[vertex,xshift=11mm] (d3r) at (e3) {$s_4$} ;  \&[12mm] \node[vertex] (t4) {$s_4,t_4$} ;\\
     
     \node[vertex] (d1) {$s_3$}    ; \& \node[vertex] (d2) {$s_3$} ; \& \node[vertex] (d3) {$s_3$} ; \& \node[vertex] (t3) {$s_3,t_3$} ;\\[2mm]
     \node[vertex] (c1) {$s_2,t_2$} ;
     \node[vertex,xshift=-11mm] (b1l) at (c1) {$s_2$} ; \node[vertex,xshift=11mm] (b1r) at (c1) {$s_2$} ;  \&
     \node[vertex] (c2) {$s_2,t_2$} ;
     \node[vertex,xshift=-11mm] (b2l) at (c2) {$s_2$} ; \node[vertex,xshift=11mm] (b2r) at (c2) {$s_2$} ;  \&
     \node[vertex] (c3) {$s_2,t_2$} ;
     \node[vertex,xshift=-11mm] (b3l) at (c3) {$s_2$} ; \node[vertex,xshift=11mm] (b3r) at (c3) {$s_2$} ;  \& \node[vertex] (t2) {$s_2,t_2$} ; \\
     \node[vertex] (b1) {$s_1$}    ; \& \node[vertex] (b2) {$s_1$} ; \& \node[vertex] (b3) {$s_1$} ; \& \node[vertex] (t1) {$s_1,t_1$} ; \\
      \& \node[vertex,label=below:{$out$}] (a1) {$s_0$} ; \& \& \node[vertex] (t0) {$s_0,t_0$} ; \\
    } ;

    % die horizontalen Kanten für die Und-Gatter-Simulation
    \foreach \von/\ueber/\zu in {{d1l/e1/d1r}, {d2l/e2/d2r}, {d3l/e3/d3r}}{
       \draw[edge,niceArrows] (\von) -- (\ueber) ;
       \draw[edge,niceArrows] (\ueber) -- (\zu) ;
     }


    \foreach \von/\ueber/\zu in {{b1l/c1/b1r}, {b2l/c2/b2r}, {b3l/c3/b3r}}{
       \draw[edge,niceArrows] (\von)   -- (\ueber) ;
       \draw[edge,niceArrows] (\ueber) -- (\zu) ;
     }  
     
    % die loops
    \foreach \knoten in {t0,t1,t2,t3,t4}
       \draw[edge,niceArrows] (\knoten) edge[loop right] (\knoten) ;
       
    % die nach unten geschwungenen Kanten zu den t-Knoten
    \foreach \von/\zu/\wie in {{b1/t1/21}, {b2/t1/18}, {b3/t1/15},
                               {b1r/t2/25}, {b2r/t2/23}, {b3r/t2/20}}
       \draw[edge,niceArrows] (\von) edge[bend right=\wie] (\zu) ;

    % die nach oben geschwungenen Kanten zu den t-Knoten
    \foreach \von/\zu/\wie in {{d1/t3/21}, {d2/t3/18}, {d3/t3/15},
                               {d1r/t4/25}, {d2r/t4/23}, {d3r/t4/20}}
       \draw[edge,niceArrows] (\von) edge[bend left=\wie] (\zu) ;
       
    \draw[revedge] (d1l) -- (d1) ;
%    \draw[revedge] (d1r) -- (d1) ;
    \draw[revedge] (d2l) -- (d2) ;
%    \draw[revedge] (d2r) -- (d2) ;
    \draw[revedge] (d3l) -- (d3) ;
%    \draw[revedge] (d3r) -- (d3) ;
    
    \draw[revedge] (d1) -- (b2l) ; 
    \draw[revedge] (d2) -- (b2l) ; 
    \draw[revedge] (d1) -- (b3l) ; 
    \draw[revedge] (d1) -- (b1l) ; 
    \draw[revedge] (d1) -- (b3r) ; 
    \draw[revedge] (d3) -- (b3r) ; 
    \draw[revedge] (d2) -- (b3l) ; 
%    \draw[revedge] (d2) -- (b1r) ; 
%    \draw[revedge] (d2) -- (b2r) ; 
    \draw[revedge] (d3) -- (b1l) ; 
    \draw[revedge] (d3) -- (b1r) ; 
    \draw[revedge] (d3) -- (b2r) ; 

    \draw[revedge] (b2l) -- (b2) ; 
    \draw[revedge] (b3l) -- (b3) ;
%    \draw[revedge] (b1r) -- (b1) ; 
%    \draw[revedge] (b3r) -- (b3) ; 
    \draw[revedge] (b1l) -- (b1) ; 
%    \draw[revedge] (b2r) -- (b2) ; 
     
    \draw[revedge] (b1) -- (a1) ; 
    \draw[revedge] (b2) -- (a1) ; 
    \draw[revedge] (b3) -- (a1) ; 

    \draw[edge,niceArrows,thick] (a1) -- (t0) ;

    \node (KKK) at (0,-1) {Kripke model $\hat{C}_{\EG}$} ;
    
    \begin{pgfonlayer}{background}
      \draw[dkante,black!23,densely dashed] (a1) -- (b3) edge[bend right=15] (t1) ;
      \draw[dkante,black!23,densely dashed] (t1) edge[loopcover] (t1) ;
      
      \draw[dkante,black!35] (b3) -- (b3l) -- (b3r) edge[bend right=18] (t2) (t2) edge[loopcover] (t2) ;

      \draw[dkante,black!23,dashed] (b3r) -- (d1) edge[bend left=21] (t3) ;
      \draw[dkante,black!23,dotted] (b3l) -- (d2) edge[bend left=18] (t3) ;
      \draw[dkante,black!23,densely dotted] (t3) edge[loopcover] (t3) ;
      
      \draw[dkante,black!23] (d1) -- (d1l) -- (d1r) edge[bend left=25] (t4) ;
      \draw[dkante,black!35] (t4) edge[loopcover] (t4) ;

      \draw[dkante,black!23] (d2) -- (d2l) -- (d2r) edge[bend left=23] (t4) ;
      \draw[dkante,black!23] (t4) edge[loopcover] (t4) ;  
    \end{pgfonlayer}  
    
\end{tikzpicture}
}


%% Das andere Kripke-Modell, das aus dem SAC1-Schaltkreis entsteht, die neueste Version
\newcommand{\ERveeACihart}{%
\begin{tikzpicture}[vertex/.style={draw=black,ellipse,inner sep=0.4mm,fill=white}]
\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=38pt,inner sep=2pt,fill=white]

    \matrix[column sep=6mm,row sep=12mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node (e1)[evertex] {\knoteninhalt{$s'_1$}} ;
       \node[evertex,xshift=-11mm] (d1l) at (e1) {\knoteninhalt{$s_0$\\$s_1$\\$t$}} ; 
       \node[evertex,minimum size=22pt,xshift=11mm] (d1r) at (e1) {\knoteninhalt{$s_0$\\$s'_1$\\$t,t_0$}} ;  \&
     \node (e2)[evertex] {\knoteninhalt{$s'_1$}} ;
       \node[evertex,xshift=-11mm] (d2l) at (e2) {\knoteninhalt{$s_0$\\$s_1$\\$t$}} ; 
       \node[evertex,minimum size=22pt,xshift=11mm] (d2r) at (e2) {\knoteninhalt{$s_0$\\$s'_1$\\$t,t_0$}} ;  \&
     \node (e3)[evertex] {\knoteninhalt{$s'_1$}} ;
       \node[evertex,xshift=-11mm] (d3l) at (e3) {\knoteninhalt{$s_0$\\$s_1$}} ; 
       \node[evertex,xshift=11mm] (d3r) at (e3) {\knoteninhalt{$s_0$\\$s'_1$\\$t_0$}} ;  
     \& \node[evertex] (t4) { } ;\\
     
     \node[evertex] (d1) {\knoteninhalt{$s_1$\\$s_2$\\$t_1$}}    ; \& 
     \node[evertex] (d2) {\knoteninhalt{$s_1$\\$s_2$\\$t_1$}} ;    \& 
     \node[evertex] (d3) {\knoteninhalt{$s_1$\\$s_2$\\$t_1$}} ; \& \\[2mm]
     
     \node[evertex] (c1) {\knoteninhalt{$s'_3$}} ;
       \node[evertex,xshift=-11mm] (b1l) at (c1) {\knoteninhalt{$s_2$\\$s_3$}} ; 
       \node[evertex,xshift=11mm] (b1r) at (c1) {\knoteninhalt{$s_2$\\$s'_3$\\$t_2$}} ;  \&
     \node[evertex] (c2) {\knoteninhalt{$s'_3$}} ;
       \node[evertex,xshift=-11mm] (b2l) at (c2) {\knoteninhalt{$s_2$\\$s'_3$}} ; 
       \node[evertex,xshift=11mm] (b2r) at (c2) {\knoteninhalt{$s_2$\\$s'_3$\\$t_2$}} ;  \&
     \node[evertex] (c3) {\knoteninhalt{$s'_3$}} ;
       \node[evertex,xshift=-11mm] (b3l) at (c3) {\knoteninhalt{$s_2$\\$s_3$}} ; 
       \node[evertex,xshift=11mm] (b3r) at (c3) {\knoteninhalt{$s_2$\\$s'_3$}} ;  
       \node[evertex,xshift=11mm] (b3rr) at (b3r) {\knoteninhalt{$s_3$}} ;  
       \node[evertex,xshift=11mm] (b3rrr) at (b3rr) {\knoteninhalt{$s_2$\\$s_3$\\$t_2$}} ;      
       \&  \\
     \node[evertex] (b1) {\knoteninhalt{$s_3$\\$s_4$\\$t_3$}} ; \& 
     \node[evertex] (b2) {\knoteninhalt{$s_3$\\$s_4$\\$t_3$}} ; \& 
     \node[evertex] (b3) {\knoteninhalt{$s_3$\\$s_4$\\$t_3$}} ; \&  \\
      \& \node[evertex,label=below:{$out$}] (a1) {\knoteninhalt{$s_4$\\$s_5$\\$t_4$}} ; \& \& \\
    } ;

    % die horizontalen Kanten für die Und-Gatter-Simulation
    \foreach \von/\ueber/\zu in {{d1l/e1/d1r}, {d2l/e2/d2r}, {d3l/e3/d3r}}{
       \draw[edge,niceArrows] (\von) -- (\ueber) ;
       \draw[edge,niceArrows] (\ueber) -- (\zu) ;
     }


    \foreach \von/\ueber/\zu in {{b1l/c1/b1r}, {b2l/c2/b2r}, {b3l/c3/b3r}, {b3r/b3rr/b3rrr}}{
       \draw[edge,niceArrows] (\von)   -- (\ueber) ;
       \draw[edge,niceArrows] (\ueber) -- (\zu) ;
     }  
     
    % die loops
    \foreach \knoten in {t4}
       \draw[edge,niceArrows] (\knoten) edge[loop right] (\knoten) ;
       
%    % die nach unten geschwungenen Kanten zu den t-Knoten
%    \foreach \von/\zu/\wie in {{b1/t1/21}, {b2/t1/18}, {b3/t1/15},
%                               {b1r/t2/25}, {b2r/t2/23}, {b3r/t2/20}}
%       \draw[edge,niceArrows] (\von) edge[bend right=\wie] (\zu) ;

    % die nach oben geschwungenen Kanten zu den t-Knoten
    \foreach \von/\zu/\wie in {{d1r/t4/25}, {d2r/t4/23}, {d3r/t4/20}}
       \draw[edge] (\von.north) edge[bend left=\wie,niceArrows] (\zu) ;
       
    \draw[revedge] (d1l) -- (d1) ;
%    \draw[revedge] (d1r) -- (d1) ;
    \draw[revedge] (d2l) -- (d2) ;
%    \draw[revedge] (d2r) -- (d2) ;
    \draw[revedge] (d3l) -- (d3) ;
%    \draw[revedge] (d3r) -- (d3) ;
    
    \draw[revedge] (d1) -- (b2l.north) ; 
    \draw[revedge] (d2) -- (b2l.north) ; 
    \draw[revedge] (d1) -- (b3l.north) ; 
    \draw[revedge] (d1) -- (b1l.north) ; 
    \draw[revedge] (d1) -- (b3r.north) ; 
    \draw[revedge] (d3) -- (b3r.north) ; 
    \draw[revedge] (d2) -- (b3l.north) ; 
%    \draw[revedge] (d2) -- (b1r) ; 
%    \draw[revedge] (d2) -- (b2r) ; 
    \draw[revedge] (d3) -- (b1l.north) ; 
    \draw[revedge] (d3) -- (b1r.north) ; 
    \draw[revedge] (d3) -- (b2r.north) ; 
    
    \draw[niceArrows,thick] (b3rrr.north) -- (d2) ;
    \draw[niceArrows,thick] (b3rrr.north) -- (d3) ;

    \draw[revedge] (b2l) -- (b2) ; 
    \draw[revedge] (b3l) -- (b3) ;
%    \draw[revedge] (b1r) -- (b1) ; 
%    \draw[revedge] (b3r) -- (b3) ; 
    \draw[revedge] (b1l) -- (b1) ; 
%    \draw[revedge] (b2r) -- (b2) ; 

     
     
    \draw[revedge] (b1) -- (a1) ; 
    \draw[revedge] (b2) -- (a1) ; 
    \draw[revedge] (b3) -- (a1) ; 


%    \node (KKK) at (0,-1) {Kripke model ${K}_{\ER,\lor}$} ;
    
    \begin{pgfonlayer}{background}
      \draw[dkante,black!23,densely dashed] (a1) -- (b3) ; 
%      \draw[dkante,black!23,densely dashed] (t1) edge[loopcover] (t1) ;
      
      \draw[dkante,black!35] (b3) -- (b3l) -- (b3r) -- (b3rr) -- (b3rrr) ; 

      \draw[dkante,black!23,dashed] (b3r.north) -- (d1) ;
      \draw[dkante,black!23,dotted] (b3l.north) -- (d2) ; 
      \draw[dkante,black!23,dotted] (b3rrr.north) -- (d2) ; 
      
      \draw[dkante,black!23] (d1) -- (d1l) -- (d1r) ;

      \draw[dkante,black!23] (d2) -- (d2l) -- (d2r) ; 
    \end{pgfonlayer}  
    
\end{tikzpicture}
}


%% Das andere Kripke-Modell, das aus dem SAC1-Schaltkreis entsteht, die neueste Version
\newcommand{\ERveeistPhart}{%
\begin{tikzpicture}[vertex/.style={draw=black,ellipse,inner sep=0.4mm,fill=white}]
\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=38pt,inner sep=2pt,fill=white]

    \matrix[column sep=6mm,row sep=12mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node {layer $0$} ; \&
     \node (e1)[evertex] {\knoteninhalt{$s'_1$}} ;
       \node[evertex,xshift=-11mm] (d1l) at (e1) {\knoteninhalt{$s_0$\\$s_1$\\$t$}} ; 
       \node[evertex,minimum size=22pt,xshift=11mm] (d1r) at (e1) {\knoteninhalt{$s_0$\\$s_1$\\$t,t_0$}} ;  \&
     \node (e2)[evertex] {\knoteninhalt{$s'_1$}} ;
       \node[evertex,xshift=-11mm] (d2l) at (e2) {\knoteninhalt{$s_0$\\$s_1$\\$t$}} ; 
       \node[evertex,minimum size=22pt,xshift=11mm] (d2r) at (e2) {\knoteninhalt{$s_0$\\$s_1$\\$t,t_0$}} ;  \&
     \node (e3)[evertex] {\knoteninhalt{$s'_1$}} ;
       \node[evertex,xshift=-11mm] (d3l) at (e3) {\knoteninhalt{$s_0$\\$s_1$}} ; 
       \node[evertex,xshift=11mm] (d3r) at (e3) {\knoteninhalt{$s_0$\\$s_1$\\$t_0$}} ;  
     \& \node[evertex] (t4) { } ;\\

     \node {layer $1$} ; \&
     \node[evertex] (d1) {\knoteninhalt{$s_1$\\$s_2$\\$t_1$}}    ; \& 
     \node[evertex] (d2) {\knoteninhalt{$s_1$\\$s_2$\\$t_1$}} ;    \& 
     \node[evertex] (d3) {\knoteninhalt{$s_1$\\$s_2$\\$t_1$}} ; \& \\[2mm]
     
     \node {layer $2$} ; \&
     \node[evertex] (c1) {\knoteninhalt{$s'_3$}} ;
       \node[evertex,xshift=-11mm] (b1l) at (c1) {\knoteninhalt{$s_2$\\$s_3$}} ; 
       \node[evertex,xshift=11mm] (b1r) at (c1) {\knoteninhalt{$s_2$\\$s_3$\\$t_2$}} ;  \&
     \node[evertex] (c2) {\knoteninhalt{$s'_3$}} ;
       \node[evertex,xshift=-11mm] (b2l) at (c2) {\knoteninhalt{$s_2$\\$s_3$}} ; 
       \node[evertex,xshift=11mm] (b2r) at (c2) {\knoteninhalt{$s_2$\\$s_3$\\$t_2$}} ;  \&
     \node[evertex] (c3) {\knoteninhalt{$s'_3$}} ;
       \node[evertex,xshift=-11mm] (b3l) at (c3) {\knoteninhalt{$s_2$\\$s_3$}} ; 
       \node[evertex,xshift=11mm] (b3r) at (c3) {\knoteninhalt{$s_2$\\$s_3$}} ;  
       \node[evertex,xshift=11mm] (b3rr) at (b3r) {\knoteninhalt{$s'_3$}} ;  
       \node[evertex,xshift=11mm] (b3rrr) at (b3rr) {\knoteninhalt{$s_2$\\$s_3$\\$t_2$}} ;      
       \&  \\
     
     \node {layer $3$} ; \&
     \node[evertex] (b1) {\knoteninhalt{$s_3$\\$s_4$\\$t_3$}} ; \& 
     \node[evertex] (b2) {\knoteninhalt{$s_3$\\$s_4$\\$t_3$}} ; \& 
     \node[evertex] (b3) {\knoteninhalt{$s_3$\\$s_4$\\$t_3$}} ; \&  \\

     \node {layer $4$} ; \&   \& \node[evertex,label=below:{$out$}] (a1) {\knoteninhalt{$s_4$\\$s_5$\\$t_4$}} ; \& \& \\
    } ;

    % die horizontalen Kanten für die Und-Gatter-Simulation
    \foreach \von/\ueber/\zu in {{d1l/e1/d1r}, {d2l/e2/d2r}, {d3l/e3/d3r}}{
       \draw[edge,niceArrows] (\von) -- (\ueber) ;
       \draw[edge,niceArrows] (\ueber) -- (\zu) ;
     }


    \foreach \von/\ueber/\zu in {{b1l/c1/b1r}, {b2l/c2/b2r}, {b3l/c3/b3r}, {b3r/b3rr/b3rrr}}{
       \draw[edge,niceArrows] (\von)   -- (\ueber) ;
       \draw[edge,niceArrows] (\ueber) -- (\zu) ;
     }  
     
    % die loops
    \foreach \knoten in {t4}
       \draw[edge,niceArrows] (\knoten) edge[loop right] (\knoten) ;
       
%    % die nach unten geschwungenen Kanten zu den t-Knoten
%    \foreach \von/\zu/\wie in {{b1/t1/21}, {b2/t1/18}, {b3/t1/15},
%                               {b1r/t2/25}, {b2r/t2/23}, {b3r/t2/20}}
%       \draw[edge,->] (\von) edge[bend right=\wie] (\zu) ;

    % die nach oben geschwungenen Kanten zu den t-Knoten
    \foreach \von/\zu/\wie in {{d1r/t4/25}, {d2r/t4/23}, {d3r/t4/20}}
       \draw[edge] (\von.north) edge[bend left=\wie,niceArrows] (\zu) ;
       
    \draw[revedge] (d1l) -- (d1) ;
%    \draw[revedge] (d1r) -- (d1) ;
    \draw[revedge] (d2l) -- (d2) ;
%    \draw[revedge] (d2r) -- (d2) ;
    \draw[revedge] (d3l) -- (d3) ;
%    \draw[revedge] (d3r) -- (d3) ;
    
    \draw[revedge] (d1) -- (b2l.north) ; 
    \draw[revedge] (d2) -- (b2l.north) ; 
    \draw[revedge] (d1) -- (b3l.north) ; 
    \draw[revedge] (d1) -- (b1l.north) ; 
    \draw[revedge] (d1) -- (b3r.north) ; 
    \draw[revedge] (d3) -- (b3r.north) ; 
    \draw[revedge] (d2) -- (b3l.north) ; 
%    \draw[revedge] (d2) -- (b1r) ; 
%    \draw[revedge] (d2) -- (b2r) ; 
    \draw[revedge] (d3) -- (b1l.north) ; 
    \draw[revedge] (d3) -- (b1r.north) ; 
    \draw[revedge] (d3) -- (b2r.north) ; 
    
    \draw[niceArrows,thick] (b3rrr.north) -- (d2) ;
    \draw[niceArrows,thick] (b3rrr.north) -- (d3) ;

    \draw[revedge] (b2l) -- (b2) ; 
    \draw[revedge] (b3l) -- (b3) ;
%    \draw[revedge] (b1r) -- (b1) ; 
%    \draw[revedge] (b3r) -- (b3) ; 
    \draw[revedge] (b1l) -- (b1) ; 
%    \draw[revedge] (b2r) -- (b2) ; 

     
     
    \draw[revedge] (b1) -- (a1) ; 
    \draw[revedge] (b2) -- (a1) ; 
    \draw[revedge] (b3) -- (a1) ; 


%    \node (KKK) at (0,-1) {Kripke model ${K}_{\ER,\lor}$} ;
    
    \begin{pgfonlayer}{background}
      \draw[dkante,black!23,densely dashed] (a1) -- (b3) ; 
%      \draw[dkante,black!23,densely dashed] (t1) edge[loopcover] (t1) ;
      
      \draw[dkante,black!35] (b3) -- (b3l) -- (b3r) -- (b3rr) -- (b3rrr) ; 

      \draw[dkante,black!23,dashed] (b3r.north) -- (d1) ;
      \draw[dkante,black!23,dotted] (b3l.north) -- (d2) ; 
      \draw[dkante,black!23,dotted] (b3rrr.north) -- (d2) ; 
      
      \draw[dkante,black!23] (d1) -- (d1l) -- (d1r) ;

      \draw[dkante,black!23] (d2) -- (d2l) -- (d2r) ; 
    \end{pgfonlayer}  
    
\end{tikzpicture}
}


%% Das andere Kripke-Modell, das aus dem SAC1-Schaltkreis entsteht, die neueste Version
\newcommand{\ERistLOGCFLhartold}{%
\begin{tikzpicture}[vertex/.style={draw=black,ellipse,inner sep=0.4mm,fill=white}]
\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=38pt,inner sep=2pt,fill=white]

    \matrix[column sep=6mm,row sep=12mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node {layer $0$} ; \&
     \node (e1)[evertex] {\knoteninhalt{$s^r_1$}} ;
       \node[evertex,xshift=-11mm] (d1l) at (e1) {\knoteninhalt{$s_0$\\$s^l_1$\\$s^r_1$\\$t$}} ; 
       \node[evertex,minimum size=22pt,xshift=11mm] (d1r) at (e1) {\knoteninhalt{$s_0$\\$s^r_1$\\$t$\\$t_0$}} ;  \&
     \node (e2)[evertex] {\knoteninhalt{$s^r_1$}} ;
       \node[evertex,xshift=-11mm] (d2l) at (e2) {\knoteninhalt{$s_0$\\$s^l_1$\\$s^r_1$\\$t$}} ; 
       \node[evertex,minimum size=22pt,xshift=11mm] (d2r) at (e2) {\knoteninhalt{$s_0$\\$s^r_1$\\$t$\\$t_0$}} ;  \&
     \node (e3)[evertex] {\knoteninhalt{$s^r_1$}} ;
       \node[evertex,xshift=-11mm] (d3l) at (e3) {\knoteninhalt{$s_0$\\$s^l_1$\\$s^r_1$}} ; 
       \node[evertex,xshift=11mm] (d3r) at (e3) {\knoteninhalt{$s_0$\\$s^r_1$\\$t_0$}} ;  
     \& \node[evertex] (t4) { } ;\\

     \node {layer $1$} ; \&
     \node[evertex] (d1) {\knoteninhalt{$s^l_1$\\$s_2$\\$t_1$}}    ; \& 
     \node[evertex] (d2) {\knoteninhalt{$s^l_1$\\$s_2$\\$t_1$}} ;    \& 
     \node[evertex] (d3) {\knoteninhalt{$s^l_1$\\$s_2$\\$t_1$}} ; \& \\[2mm]
     
     \node {layer $2$} ; \&
     \node[evertex] (c1) {\knoteninhalt{$s^r_3$}} ;
       \node[evertex,xshift=-11mm] (b1l) at (c1) {\knoteninhalt{$s_2$\\$s^l_3$\\$s^r_3$}} ; 
       \node[evertex,xshift=11mm] (b1r) at (c1) {\knoteninhalt{$s_2$\\$s^r_3$\\$t_2$}} ;  \&
     \node[evertex] (c2) {\knoteninhalt{$s^r_3$}} ;
       \node[evertex,xshift=-11mm] (b2l) at (c2) {\knoteninhalt{$s_2$\\$s^l_3$\\$s^r_3$}} ; 
       \node[evertex,xshift=11mm] (b2r) at (c2) {\knoteninhalt{$s_2$\\$s^r_3$\\$t_2$}} ;  \&
     \node[evertex] (c3) {\knoteninhalt{$s^r_3$}} ;
       \node[evertex,xshift=-11mm] (b3l) at (c3) {\knoteninhalt{$s_2$\\$s^l_3$\\$s^r$}} ; 
       \node[evertex,xshift=11mm] (b3r) at (c3) {\knoteninhalt{$s_2$\\$s^r_3$\\$s_2$}} ;  
       \&  \\
     
     \node {layer $3$} ; \&
     \node[evertex] (b1) {\knoteninhalt{$s^l_3$\\$s_4$\\$t_3$}} ; \& 
     \node[evertex] (b2) {\knoteninhalt{$s^l_3$\\$s_4$\\$t_3$}} ; \& 
     \node[evertex] (b3) {\knoteninhalt{$s^l_3$\\$s_4$\\$t_3$}} ; \&  \\

     \node {layer $4$} ; \&   \& \node[evertex,label=below:{$out$}] (a1) {\knoteninhalt{$s_4$\\$s_5$\\$t_4$}} ; \& \& \\
    } ;

    % die horizontalen Kanten für die Und-Gatter-Simulation
    \foreach \von/\ueber/\zu in {{d1l/e1/d1r}, {d2l/e2/d2r}, {d3l/e3/d3r}}{
       \draw[edge,niceArrows] (\von) -- (\ueber) ;
       \draw[edge,niceArrows] (\ueber) -- (\zu) ;
     }


    \foreach \von/\ueber/\zu in {{b1l/c1/b1r}, {b2l/c2/b2r}, {b3l/c3/b3r}}{
       \draw[edge,niceArrows] (\von)   -- (\ueber) ;
       \draw[edge,niceArrows] (\ueber) -- (\zu) ;
     }  
     
    % die loops
    \foreach \knoten in {t4}
       \draw[edge,niceArrows] (\knoten) edge[loop right] (\knoten) ;
       
%    % die nach unten geschwungenen Kanten zu den t-Knoten
%    \foreach \von/\zu/\wie in {{b1/t1/21}, {b2/t1/18}, {b3/t1/15},
%                               {b1r/t2/25}, {b2r/t2/23}, {b3r/t2/20}}
%       \draw[edge,niceArrows] (\von) edge[bend right=\wie] (\zu) ;

    % die nach oben geschwungenen Kanten zu den t-Knoten
    \foreach \von/\zu/\wie in {{d1r/t4/25}, {d2r/t4/23}, {d3r/t4/20}}
       \draw[edge] (\von.north) edge[bend left=\wie,niceArrows] (\zu) ;
       
    \draw[revedge] (d1l) -- (d1) ;
%    \draw[revedge] (d1r) -- (d1) ;
    \draw[revedge] (d2l) -- (d2) ;
%    \draw[revedge] (d2r) -- (d2) ;
    \draw[revedge] (d3l) -- (d3) ;
%    \draw[revedge] (d3r) -- (d3) ;
    
    \draw[revedge] (d1) -- (b2l.north) ; 
    \draw[revedge] (d2) -- (b2l.north) ; 
    \draw[revedge] (d1) -- (b3l.north) ; 
    \draw[revedge] (d1) -- (b1l.north) ; 
    \draw[revedge] (d1) -- (b3r.north) ; 
    \draw[revedge] (d3) -- (b3r.north) ; 
    \draw[revedge] (d2) -- (b3l.north) ; 
%    \draw[revedge] (d2) -- (b1r) ; 
%    \draw[revedge] (d2) -- (b2r) ; 
    \draw[revedge] (d3) -- (b1l.north) ; 
    \draw[revedge] (d3) -- (b1r.north) ; 
    \draw[revedge] (d3) -- (b2r.north) ; 
    
    \draw[revedge] (b2l) -- (b2) ; 
    \draw[revedge] (b3l) -- (b3) ;
%    \draw[revedge] (b1r) -- (b1) ; 
%    \draw[revedge] (b3r) -- (b3) ; 
    \draw[revedge] (b1l) -- (b1) ; 
%    \draw[revedge] (b2r) -- (b2) ; 

     
     
    \draw[revedge] (b1) -- (a1) ; 
    \draw[revedge] (b2) -- (a1) ; 
    \draw[revedge] (b3) -- (a1) ; 


%    \node (KKK) at (0,-1) {Kripke model ${K}_{\ER,\lor}$} ;
    
    \begin{pgfonlayer}{background}
      \draw[dkante,black!23,densely dashed] (a1) -- (b3) ; 
%      \draw[dkante,black!23,densely dashed] (t1) edge[loopcover] (t1) ;
      
      \draw[dkante,black!35] (b3) -- (b3l) -- (b3r) ; 

      \draw[dkante,black!23,dashed] (b3r.north) -- (d1) ;
      \draw[dkante,black!23,dotted] (b3l.north) -- (d2) ; 
      
      \draw[dkante,black!23] (d1) -- (d1l) -- (d1r) ;

      \draw[dkante,black!23] (d2) -- (d2l) -- (d2r) ; 
    \end{pgfonlayer}  
    
\end{tikzpicture}
}

%% Das andere Kripke-Modell, das aus dem SAC1-Schaltkreis entsteht, die neueste Version
\newcommand{\ERistLOGCFLhart}{%
\begin{tikzpicture}[vertex/.style={draw=black,ellipse,inner sep=0.4mm,fill=white}]
\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=30pt,inner sep=2pt,fill=white]

    \matrix[column sep=6mm,row sep=2mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node {$V_5$:} ; \& \&
       \node[evertex,label=below:{$e$}] (ee) {} ;
     \\
     \node {$V_4\subseteq V_{\exists}$:} ; \&
     \node (e1) {} ;
       \node[evertex,xshift=-8mm] (d1l) at (e1) {\knoteninhalt{$s_4$\\$s^l_3$\\$t$}} ; 
       \node[evertex,xshift=8mm] (d1r) at (e1) {\knoteninhalt{$s_4$\\$s^r_3$\\$t$}} ;  \&
     \node (e2) {} ;
       \node[evertex,xshift=-8mm] (d2l) at (e2) {\knoteninhalt{$s_4$\\$s^l_3$}} ; 
       \node[evertex,xshift=8mm] (d2r) at (e2) {\knoteninhalt{$s_4$\\$s^r_3$\\$t$}} ;  \&
     \node (e3) {} ;
       \node[evertex,xshift=-8mm] (d3l) at (e3) {\knoteninhalt{$s_4$\\$s^l_3$\\$t$}} ; 
       \node[evertex,xshift=8mm] (d3r) at (e3) {\knoteninhalt{$s_4$\\$s^r_3$}} ;  
    \\

     \node {$V_3\subseteq V_{\forall}$:} ; \&
     \node[evertex] (d1) {\knoteninhalt{$s^l_3$\\$s^r_3$\\$s_2$}}    ; \& 
     \node[evertex] (d2) {\knoteninhalt{$s^l_3$\\$s^r_3$\\$s_2$}} ;    \& 
     \node[evertex] (d3) {\knoteninhalt{$s^l_3$\\$s^r_3$\\$s_2$}} ;  \\[6mm]
     
     \node {$V_2\subseteq V_{\exists}$:} ; \&
     \node (c1) {} ;
       \node[evertex,xshift=-8mm] (b1l) at (c1) {\knoteninhalt{$s_2$\\$s^l_1$}} ; 
       \node[evertex,xshift=8mm] (b1r) at (c1) {\knoteninhalt{$s_2$\\$s^r_1$}} ;  \&
     \node (c2) {} ;
       \node[evertex,xshift=-8mm] (b2l) at (c2) {\knoteninhalt{$s_2$\\$s^l_1$}} ; 
       \node[evertex,xshift=8mm] (b2r) at (c2) {\knoteninhalt{$s_2$\\$s^r_1$}} ;  \&
     \node (c3) {} ;
       \node[evertex,xshift=-8mm] (b3l) at (c3) {\knoteninhalt{$s_2$\\$s^l_1$}} ; 
       \node[evertex,xshift=8mm] (b3r) at (c3) {\knoteninhalt{$s_2$\\$s^r_1$}} ;  
     \\
     
     \node {$V_1\subseteq V_{\forall}$:} ; \&
     \node[evertex] (b1) {\knoteninhalt{$s^l_1$\\$s^r_1$\\$s_0$}} ; \& 
     \node[evertex] (b2) {\knoteninhalt{$s^l_1$\\$s^r_1$\\$s_0$}} ; \& 
     \node[evertex] (b3) {\knoteninhalt{$s^l_1$\\$s^r_1$\\$s_0$}} ; \&  \\[2mm]

     \node {$V_0\subseteq V_{\exists}$:} ; \&   \& \node[evertex,label=below:{$s$}] (a1) {\knoteninhalt{$s_0$}} ; \& \& \\
    } ;

    % von slice 3 nach slice 4
    \foreach \von/\nach in {d1/d1l, d1/d1r, d2/d2l, d2/d2r, d3/d3l, d3/d3r}{
       \draw[edge,niceArrows] (\von) -- (\nach.south) ;
     }

    % von slice 2 nach slice 3
    \foreach \von/\nach in {b1l/d1, b1l/d3, b1r/d3, b2l/d1, b2l/d2, b2r/d2, b2r/d3, b3l/d1, b3l/d2, b3r/d1, b3r/d3}{
       \draw[edge,niceArrows] (\von.north) -- (\nach.south) ;
     }

    % von slice 1 nach slice 2 und von 0 zu 1
    \foreach \von/\nach in {b1/b1l, b1/b1r, b2/b2l, b2/b2r, b3/b3l, b3/b3r, a1/b1, a1/b2, a1/b3}{
       \draw[edge,niceArrows] (\von) -- (\nach.south) ;
     }
     
    % die Kanten zum neuen Knoten e in V_5
    \draw[edge,niceArrows] (ee) edge[loop left] (ee) ;
    \foreach \knoten in {d1l, d1r, d2l, d2r, d3l, d3r}
       \draw[edge,niceArrows] (\knoten.north) -- (ee) ;
       
\end{tikzpicture}
}



%% Das Kripke-Modell mit den verschmolzenen Und- und Oder-Schichten
\newcommand{\ERistPhartneu}{%
\begin{tikzpicture}[vertex/.style={draw=black,ellipse,inner sep=0.4mm,fill=white}]
\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=38pt,inner sep=2pt,fill=white]

    \matrix[column sep=6mm,row sep=12mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node {layer $0$} ; \&
     \node (e1)[evertex] {\knoteninhalt{$s_2$\\$t$}} ; 
       \node[evertex,xshift=11mm] (e1r) at (e1) {\knoteninhalt{$t_0$\\$t$}} ;  \&
     \node (e2)[evertex] {\knoteninhalt{$s_2$\\$t$}} ; 
       \node[evertex,xshift=11mm] (e2r) at (e2) {\knoteninhalt{$t_0$\\$t$}} ;  \&
     \node (e3)[evertex]  {\knoteninhalt{$s_2$}} ; 
       \node[evertex,xshift=11mm] (e3r) at (e3) {\knoteninhalt{$t_0$}} ;  
     \& \node[evertex] (t4) { } ;\\

     \node {layer $1$} ; \&
%     \node (d1) {}    ; \& 
%     \node (d2) {} ;    \& 
%     \node (d3) {} ; \& 
\\[2mm]
     
     \node {layer $2$} ; \&
     \node[evertex] (c1) {\knoteninhalt{$s_2$\\$s_4$}} ; 
       \node[evertex,xshift=11mm] (c1r) at (c1) {\knoteninhalt{$s_2$\\$t_2$}} ;  \&
     \node[evertex] (c2) {\knoteninhalt{$s_2$\\$s_4$}} ; 
       \node[evertex,xshift=11mm] (c2r) at (c2) {\knoteninhalt{$s_2$\\$t_2$}} ;  \&
     \node[evertex] (c3) {\knoteninhalt{$s_2$\\$s_4$}} ; 
       \node[evertex,xshift=11mm] (c3r) at (c3) {\knoteninhalt{$s_2$}} ;  
       \node[evertex,xshift=11mm] (c3rr) at (c3r) {\knoteninhalt{$s_2$\\$t_2$}} ;      
       \&  \\
     
     \node {layer $3$} ; \&
%     \node[evertex] (b1) {\knoteninhalt{$s_3$\\$s_4$\\$t_3$}} ; \& 
%     \node[evertex] (b2) {\knoteninhalt{$s_3$\\$s_4$\\$t_3$}} ; \& 
%     \node[evertex] (b3) {\knoteninhalt{$s_3$\\$s_4$\\$t_3$}} ; \&  
\\

     \node {layer $4$} ; \&   \& \node[evertex,label=below:{$out$}] (a1) {\knoteninhalt{$s_4$\\$t_4$}} ; \& \& \\
    } ;

    % die horizontalen Kanten für die Und-Gatter-Simulation
    \foreach \von/\zu in {{e1/e1r}, {e2/e2r}, {e3/e3r}}{
       \draw[edge,niceArrows] (\von) -- (\zu) ;
     }


    \foreach \von/\zu in {{c1/c1r}, {c2/c2r}, {c3/c3r}, {c3r/c3rr}}{
       \draw[edge,niceArrows] (\von)   -- (\zu) ;
     }  
     
    % die loops
    \foreach \knoten in {t4}
       \draw[edge,niceArrows] (\knoten) edge[loop right] (\knoten) ;
       
%    % die nach unten geschwungenen Kanten zu den t-Knoten
%    \foreach \von/\zu/\wie in {{b1/t1/21}, {b2/t1/18}, {b3/t1/15},
%                               {b1r/t2/25}, {b2r/t2/23}, {b3r/t2/20}}
%       \draw[edge,->] (\von) edge[bend right=\wie] (\zu) ;

    % die nach oben geschwungenen Kanten zu den t-Knoten
    \foreach \von/\zu/\wie in {{e1r/t4/25}, {e2r/t4/23}, {e3r/t4/20}}
       \draw[edge] (\von.north) edge[bend left=\wie,niceArrows] (\zu) ;
       
    
    \draw[revedge] (e1) -- (c2.north) ; 
    \draw[revedge] (e2) -- (c2.north) ; 
    \draw[revedge] (e1) -- (c3.north) ; 
    \draw[revedge] (e1) -- (c1.north) ; 
    \draw[revedge] (e1) -- (c3r.north) ; 
    \draw[revedge] (e3) -- (c3r.north) ; 
    \draw[revedge] (e2) -- (c3.north) ; 
%    \draw[revedge] (d2) -- (b1r) ; 
%    \draw[revedge] (d2) -- (b2r) ; 
    \draw[revedge] (e3) -- (c1.north) ; 
    \draw[revedge] (e3) -- (c1r.north) ; 
    \draw[revedge] (e3) -- (c2r.north) ; 
    
    \draw[niceArrows,thick] (c3rr.north) -- (e2) ;
    \draw[niceArrows,thick] (c3rr.north) -- (e3) ;

%    \draw[revedge] (b2l) -- (b2) ; 
%    \draw[revedge] (b3l) -- (b3) ;
%%    \draw[revedge] (b1r) -- (b1) ; 
%%    \draw[revedge] (b3r) -- (b3) ; 
%    \draw[revedge] (b1l) -- (b1) ; 
%%    \draw[revedge] (b2r) -- (b2) ; 

     
     
    \draw[revedge] (c1) -- (a1) ; 
    \draw[revedge] (c2) -- (a1) ; 
    \draw[revedge] (c3) -- (a1) ; 


%    \node (KKK) at (0,-1) {Kripke model ${K}_{\ER,\lor}$} ;
    
    \begin{pgfonlayer}{background}
      \draw[dkante,black!23,densely dashed] (a1) -- (c3) ; 
%      \draw[dkante,black!23,densely dashed] (t1) edge[loopcover] (t1) ;
      
      \draw[dkante,black!35] (c3) -- (c3r) -- (c3rr) ; 

      \draw[dkante,black!23,dashed] (c3r.north) -- (e1) ;
      \draw[dkante,black!23,dotted] (c3.north) -- (e2) ; 
      \draw[dkante,black!23,dotted] (c3rr.north) -- (e2) ; 
      
      \draw[dkante,black!23] (e1) -- (e1r) ;

      \draw[dkante,black!23] (e2) -- (e2r)  ; 
    \end{pgfonlayer}  
    
\end{tikzpicture}
}



%% Das andere Kripke-Modell, das aus dem Schaltkreis entsteht, die neueste Version
\newcommand{\EUistPhart}{%
\begin{tikzpicture}[baseline=(KKK.base)] %,vertex/.style={draw=black,circle,inner sep=.7mm,fill=white}]

    \matrix[column sep=4mm,row sep=6mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node (e1)[vertex] {$r_0$} ;
     \node[vertex,xshift=-11mm] (d1l) at (e1) {$s_0,t$} ; \node[vertex,xshift=11mm] (d1r) at (e1) {$s_0,t$} ;  \&
     \node (e2)[vertex] {$r_0$} ;
     \node[vertex,xshift=-11mm] (d2l) at (e2) {$s_0,t$} ; \node[vertex,xshift=11mm] (d2r) at (e2) {$s_0,t$} ;  \&
     \node (e3)[vertex] {$r_0$} ;
     \node[vertex,xshift=-11mm] (d3l) at (e3) {$s_0$} ; \node[vertex,xshift=11mm] (d3r) at (e3) {$s_0$} ;  \&[12mm] \node[vertex] (t4) {$t_0$} ;\\
     
     \node[vertex] (d1) {$s_1$}    ; \& \node[vertex] (d2) {$s_1$} ; \& \node[vertex] (d3) {$s_1$} ; \& \node[vertex] (t3) {$t_1$} ;\\[2mm]
     \node[vertex] (c1) {$r_2$} ;
     \node[vertex,xshift=-11mm] (b1l) at (c1) {$s_2$} ; \node[vertex,xshift=11mm] (b1r) at (c1) {$s_2$} ;  \&
     \node[vertex] (c2) {$r_2$} ;
     \node[vertex,xshift=-11mm] (b2l) at (c2) {$s_2$} ; \node[vertex,xshift=11mm] (b2r) at (c2) {$s_2$} ;  \&
     \node[vertex] (c3) {$r_2$} ;
     \node[vertex,xshift=-11mm] (b3l) at (c3) {$s_2$} ; \node[vertex,xshift=11mm] (b3r) at (c3) {$s_2$} ;  \& \node[vertex] (t2) {$t_2$} ; \\
     \node[vertex] (b1) {$s_3$}    ; \& \node[vertex] (b2) {$s_3$} ; \& \node[vertex] (b3) {$s_3$} ; \& \node[vertex] (t1) {$t_3$} ; \\
      \& \node[vertex,label=below:{$out$}] (a1) {$s_4$} ; \& \& \node[vertex] (t0) {$t_4$} ; \\
    } ;

    % die horizontalen Kanten für die Und-Gatter-Simulation
    \foreach \von/\ueber/\zu in {{d1l/e1/d1r}, {d2l/e2/d2r}, {d3l/e3/d3r}}{
       \draw[edge,niceArrows] (\von) -- (\ueber) ;
       \draw[edge,niceArrows] (\ueber) -- (\zu) ;
     }


    \foreach \von/\ueber/\zu in {{b1l/c1/b1r}, {b2l/c2/b2r}, {b3l/c3/b3r}}{
       \draw[edge,niceArrows] (\von)   -- (\ueber) ;
       \draw[edge,niceArrows] (\ueber) -- (\zu) ;
     }  
     
    % die loops
    \foreach \knoten in {t0,t1,t2,t3,t4}
       \draw[edge,niceArrows] (\knoten) edge[loop right] (\knoten) ;
       
    % die nach unten geschwungenen Kanten zu den t-Knoten
    \foreach \von/\zu/\wie in {{b1/t1/21}, {b2/t1/18}, {b3/t1/15},
                               {b1r/t2/25}, {b2r/t2/23}, {b3r/t2/20}}
       \draw[edge,niceArrows] (\von) edge[bend right=\wie] (\zu) ;

    % die nach oben geschwungenen Kanten zu den t-Knoten
    \foreach \von/\zu/\wie in {{d1/t3/21}, {d2/t3/18}, {d3/t3/15},
                               {d1r/t4/25}, {d2r/t4/23}, {d3r/t4/20}}
       \draw[edge,niceArrows] (\von) edge[bend left=\wie] (\zu) ;
       
    \draw[revedge] (d1l) -- (d1) ;
%    \draw[revedge] (d1r) -- (d1) ;
    \draw[revedge] (d2l) -- (d2) ;
%    \draw[revedge] (d2r) -- (d2) ;
    \draw[revedge] (d3l) -- (d3) ;
%    \draw[revedge] (d3r) -- (d3) ;
    
    \draw[revedge] (d1) -- (b2l) ; 
    \draw[revedge] (d2) -- (b2l) ; 
    \draw[revedge] (d1) -- (b3l) ; 
    \draw[revedge] (d1) -- (b1l) ; 
    \draw[revedge] (d1) -- (b3r) ; 
    \draw[revedge] (d3) -- (b3r) ; 
    \draw[revedge] (d2) -- (b3l) ; 
%    \draw[revedge] (d2) -- (b1r) ; 
%    \draw[revedge] (d2) -- (b2r) ; 
    \draw[revedge] (d3) -- (b1l) ; 
    \draw[revedge] (d3) -- (b1r) ; 
    \draw[revedge] (d3) -- (b2r) ; 

    \draw[revedge] (b2l) -- (b2) ; 
    \draw[revedge] (b3l) -- (b3) ;
%    \draw[revedge] (b1r) -- (b1) ; 
%    \draw[revedge] (b3r) -- (b3) ; 
    \draw[revedge] (b1l) -- (b1) ; 
%    \draw[revedge] (b2r) -- (b2) ; 
     
    \draw[revedge] (b1) -- (a1) ; 
    \draw[revedge] (b2) -- (a1) ; 
    \draw[revedge] (b3) -- (a1) ; 

    \draw[edge,niceArrows,thick] (a1) -- (t0) ;

    \node (KKK) at (0,-1) {Kripke model $C_{\EU}$} ;
    
    \begin{pgfonlayer}{background}
      \draw[dkante,black!23,densely dashed] (a1) -- (b3) edge[bend right=15] (t1) ;
      \draw[dkante,black!23,densely dashed] (t1) edge[loopcover] (t1) ;
      
      \draw[dkante,black!35] (b3) -- (b3l) -- (b3r) edge[bend right=18] (t2) (t2) edge[loopcover] (t2) ;

      \draw[dkante,black!23,dashed] (b3r) -- (d1) edge[bend left=21] (t3) ;
      \draw[dkante,black!23,dotted] (b3l) -- (d2) edge[bend left=18] (t3) ;
      \draw[dkante,black!23,densely dotted] (t3) edge[loopcover] (t3) ;
      
      \draw[dkante,black!23] (d1) -- (d1l) -- (d1r) edge[bend left=25] (t4) ;
      \draw[dkante,black!35] (t4) edge[loopcover] (t4) ;

      \draw[dkante,black!23] (d2) -- (d2l) -- (d2r) edge[bend left=23] (t4) ;
      \draw[dkante,black!23] (t4) edge[loopcover] (t4) ;  
    \end{pgfonlayer}  
    
\end{tikzpicture}
}

%%%% ER ist P-hart
\newcommand{\ERistPhart}{%
\begin{tikzpicture}[baseline=(KKK.base)] %,vertex/.style={draw=black,circle,inner sep=.7mm,fill=white}]

    \matrix[column sep=4mm,row sep=6mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    {
     \node (e1) { } ;
     \node[vertex,xshift=-11mm] (d1l) at (e1) {$s_0,t$} ; \node[vertex,xshift=11mm] (d1r) at (e1) {$s_0,t_0,t$} ;  \&
     \node (e2) { } ;
     \node[vertex,xshift=-11mm] (d2l) at (e2) {$s_0,t$} ; \node[vertex,xshift=11mm] (d2r) at (e2) {$s_0,t_0,t$} ;  \&
     \node (e3) { } ;
     \node[vertex,xshift=-11mm] (d3l) at (e3) {$s_0$} ; \node[vertex,xshift=11mm] (d3r) at (e3) {$s_0,t_0$} ;  \\
     
     \node[vertex] (d1) {$s_1,t_1$}    ; \& \node[vertex] (d2) {$s_1,t_1$} ; \& \node[vertex] (d3) {$s_1,t_1$} ; \\[2mm]
     \node (c1) { } ;
     \node[vertex,xshift=-11mm] (b1l) at (c1) {$s_2$} ; \node[vertex,xshift=11mm] (b1r) at (c1) {$s_2,t_2$} ;  \&
     \node (c2) {} ;
     \node[vertex,xshift=-11mm] (b2l) at (c2) {$s_2$} ; \node[vertex,xshift=11mm] (b2r) at (c2) {$s_2,t_2$} ;  \&
     \node (c3) {} ;
     \node[vertex,xshift=-11mm] (b3l) at (c3) {$s_2$} ; \node[vertex,xshift=11mm] (b3r) at (c3) {$s_2,t_2$} ;   \\
     \node[vertex] (b1) {$s_3,t_3$}    ; \& \node[vertex] (b2) {$s_3,t_3$} ; \& \node[vertex] (b3) {$s_3,t_3$} ;  \\
      \& \node[vertex,label=below:{$out$}] (a1) {$s_4,t_4$} ; \& \&  \\
    } ;

    % die horizontalen Kanten für die Und-Gatter-Simulation
    \foreach \von/\zu in {{d1l/d1r}, {d2l/d2r}, {d3l/d3r}}{
       \draw[edge,niceArrows] (\von) -- (\zu) ;
     }


    \foreach \von/\zu in {{b1l/b1r}, {b2l/b2r}, {b3l/b3r}}{
       \draw[edge,niceArrows] (\von)   -- (\zu) ;
     }  
     
    % die loops
    \foreach \knoten in {d1r,d2r,d3r}
       \draw[edge,niceArrows] (\knoten) edge[loop above] (\knoten) ;
       
      
    \draw[revedge] (d1l) -- (d1) ;
%    \draw[revedge] (d1r) -- (d1) ;
    \draw[revedge] (d2l) -- (d2) ;
%    \draw[revedge] (d2r) -- (d2) ;
    \draw[revedge] (d3l) -- (d3) ;
%    \draw[revedge] (d3r) -- (d3) ;
    
    \draw[revedge] (d1) -- (b2l) ; 
    \draw[revedge] (d2) -- (b2l) ; 
    \draw[revedge] (d1) -- (b3l) ; 
    \draw[revedge] (d1) -- (b1l) ; 
    \draw[revedge] (d1) -- (b3r) ; 
    \draw[revedge] (d3) -- (b3r) ; 
    \draw[revedge] (d2) -- (b3l) ; 
%    \draw[revedge] (d2) -- (b1r) ; 
%    \draw[revedge] (d2) -- (b2r) ; 
    \draw[revedge] (d3) -- (b1l) ; 
    \draw[revedge] (d3) -- (b1r) ; 
    \draw[revedge] (d3) -- (b2r) ; 

    \draw[revedge] (b2l) -- (b2) ; 
    \draw[revedge] (b3l) -- (b3) ;
%    \draw[revedge] (b1r) -- (b1) ; 
%    \draw[revedge] (b3r) -- (b3) ; 
    \draw[revedge] (b1l) -- (b1) ; 
%    \draw[revedge] (b2r) -- (b2) ; 
     
    \draw[revedge] (b1) -- (a1) ; 
    \draw[revedge] (b2) -- (a1) ; 
    \draw[revedge] (b3) -- (a1) ; 

    \node (KKK) at (0,-1) {Kripke model $C_{\ER}$} ;
    
%    \begin{pgfonlayer}{background}
%      \draw[dkante,black!23,densely dashed] (a1) -- (b3) edge[bend right=15] (t1) ;
%      \draw[dkante,black!23,densely dashed] (t1) edge[loopcover] (t1) ;
%      
%      \draw[dkante,black!35] (b3) -- (b3l) -- (b3r) edge[bend right=18] (t2) (t2) edge[loopcover] (t2) ;
%
%      \draw[dkante,black!23,dashed] (b3r) -- (d1) edge[bend left=21] (t3) ;
%      \draw[dkante,black!23,dotted] (b3l) -- (d2) edge[bend left=18] (t3) ;
%      \draw[dkante,black!23,densely dotted] (t3) edge[loopcover] (t3) ;
%      
%      \draw[dkante,black!23] (d1) -- (d1l) -- (d1r) edge[bend left=25] (t4) ;
%      \draw[dkante,black!35] (t4) edge[loopcover] (t4) ;
%
%      \draw[dkante,black!23] (d2) -- (d2l) -- (d2r) edge[bend left=23] (t4) ;
%      \draw[dkante,black!23] (t4) edge[loopcover] (t4) ;  
%    \end{pgfonlayer}  
    
\end{tikzpicture}
}




%% LTL-MC: das Kripke-Modell für die Reduktion von 3SAT zu \F,\wedge
\newcommand{\ltlFwedge}{%
\tikzstyle{vertex}=[thick,draw=black,ellipse,minimum size=5.5mm,inner sep=0mm]
\begin{tikzpicture}

    \matrix[column sep=8mm,row sep=0mm,ampersand replacement=\&,matrix anchor=south] at (0,-0.4)
    { \& \node[vertex] (o1) {$c_1$} ; \& \node[vertex] (o2) { } ; \& 
             \node[vertex] (o3) {$c_2$} ; \& \node[vertex] (o4) {$c_3$} ; \& \\
    \node[vertex,label=below:{$w$}] (start) { } ; \&  \& \& \& \& \node[vertex] (ende) { } ; \\[-8mm]
    \& \node[vertex] (u1) {$c_2$} ; \& \node[vertex,label] (u2) {$c_1,c_3$} ; \& 
         \node[vertex] (u3) { } ; \& \node[vertex] (u4) {$c_1,c_2$} ; \& \\
    } ;
    
    \foreach \von/\nach in {{start/o1},{start/u1},{o4/ende},{u4/ende}}
      \draw[edge,thick,niceArrows] (\von) -- (\nach) ; 
    
    \foreach \von/\nach in {{1/2},{2/3},{3/4}}
    { \foreach \woher in {u,o} \foreach \wohin in {u,o}
           \draw[edge,thick,niceArrows] (\woher\von) -- (\wohin\nach) ;
    }
    
    \draw[edge,thick,niceArrows] (ende) edge[loop right] (ende) ;
    
    \foreach \wo/\was in {{1/a}, {2/b}, {3/d}, {4/e}}
    {
         \node[yshift=-10mm,anchor=base] at (u\wo) {$\neg \was$} ;
         \node[yshift=8mm,anchor=base] at (o\wo) {$\was$} ;
    }
\end{tikzpicture}
}

%% LTL-MC: das Kripke-Modell für die Reduktion von 3SAT zu G,X,\vee
\newcommand{\knoteninhalt}[1]{
\begin{minipage}{12pt}

\centering

#1

\end{minipage}
}

\newcommand{\ltlGXvee}{%
\begin{tikzpicture}[x=10mm,niceArrows]
\tikzstyle{vertex}=[circle,draw=black,thick,minimum size=5.5mm,inner sep=.5mm]
\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=40pt,inner sep=2pt]

% die drei Startknoten und der Endknoten
\node[vertex,label=below:{$w_1$}] (q1) at (0,2) {};
\node[vertex,label=below:{$w_2$}] (q2) at (1,2) {};
\node[vertex,label=below:{$w_3$}] (q3) at (2,2) {};
\node[vertex] (ende) at (12,2) {$s$} ;

\foreach \i/\la in {{1/a},{2/a},{3/a},{4/b},{5/b},{6/b},{7/d},{8/d},{9/d}}
{
  \node[evertex] (a\i) at (2+\i,3.5) {} ;
  \node[evertex] (b\i) at (2+\i,0.5) {} ;
}

\foreach \i/\la in {{1/a},{4/b},{7/d}}
{
  \node[yshift=10mm,anchor=base] at (a\i) {$\la$} ; 
  \node[yshift=-12mm,anchor=base] at (b\i) {$\neg \la$} ; 
}



\draw[edge,niceArrows,thick] (q1) -- (q2) ;
\draw[edge,niceArrows,thick] (q2) -- (q3) ;
\draw[edge,niceArrows,thick] (q3) -- (a1) ;
\draw[edge,niceArrows,thick] (q3) -- (b1) ;
\draw[edge,niceArrows,thick] (a9) -- (ende) ;
\draw[edge,niceArrows,thick] (b9) -- (ende) ;
\draw[edge,niceArrows,thick] (ende) edge[loop right] (ende) ;


\foreach \i [count=\j from 2] in {1,2,...,8}
{
  \draw[edge,niceArrows,thick] (a\i) -- (a\j) ;
  \draw[edge,niceArrows,thick] (b\i) -- (b\j) ;
}


\foreach \i  in {3,6}
{
  % berechne erstmal \j=\i+1
  \pgfmathparse{\i+1}  
  \pgfmathtruncatemacro\j\pgfmathresult
  
  \draw[edge,niceArrows,thick] (a\i) -- (b\j) ;
  \draw[edge,niceArrows,thick] (b\i) -- (a\j) ;
}

\node at (a1) {\knoteninhalt{$c_1$\\$s$}} ;
\node at (a4) {\knoteninhalt{$c_2$\\$s$}} ;
\node at (a7) {\knoteninhalt{$c_2$\\$c_3$\\$s$}} ;
\node at (b1) {\knoteninhalt{$c_2$\\$s$}} ;
\node at (b4) {\knoteninhalt{$c_1$\\$c_3$\\$s$}} ;
\node at (b7) {\knoteninhalt{$c_1$\\$s$}} ;

\foreach \i in {2,3,5,6,8,9}
{
  \node at (a\i) {\knoteninhalt{$s$}} ;
  \node at (b\i) {\knoteninhalt{$s$}} ;
}

\end{tikzpicture}
}

%------------------------------------------------------------------------

\newcommand{\ltlGXveeneu}{%
\begin{tikzpicture}[x=10mm,niceArrows]
\tikzstyle{vertex}=[circle,draw=black,thick,minimum size=5.5mm,inner sep=.5mm]
\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=40pt,inner sep=2pt]

% die drei Startknoten und der Endknoten
\node[vertex,label=below:{$w_1$}] (q1) at (0,2) {};
\node[vertex,label=below:{$w_2$}] (q2) at (1,2) {};
\node[vertex,label=below:{$w_3$}] (q3) at (2,2) {};
\node[vertex] (ende) at (12,2) {$s$} ;

\foreach \i/\la in {{1/a},{2/a},{3/a},{4/b},{5/b},{6/b},{7/d},{8/d},{9/d}}
{
  \node[evertex] (a\i) at (2+\i,3.5) {} ;
  \node[evertex] (b\i) at (2+\i,0.5) {} ;
}

\foreach \i/\la in {{1/a},{4/b},{7/d}}
{
  \node[yshift=10mm,anchor=base] at (a\i) {$\la$} ; 
  \node[yshift=-12mm,anchor=base] at (b\i) {$\neg \la$} ; 
}



\draw[edge,niceArrows,thick] (q1) -- (q2) ;
\draw[edge,niceArrows,thick] (q2) -- (q3) ;
\draw[edge,niceArrows,thick] (q3) -- (a1) ;
\draw[edge,niceArrows,thick] (q3) -- (b1) ;
\draw[edge,niceArrows,thick] (a9) -- (ende) ;
\draw[edge,niceArrows,thick] (b9) -- (ende) ;
\draw[edge,niceArrows,thick] (ende) edge[loop right] (ende) ;


\foreach \i [count=\j from 2] in {1,2,...,8}
{
  \draw[edge,niceArrows,thick] (a\i) -- (a\j) ;
  \draw[edge,niceArrows,thick] (b\i) -- (b\j) ;
}


\foreach \i  in {3,6}
{
  % berechne erstmal \j=\i+1
  \pgfmathparse{\i+1}  
  \pgfmathtruncatemacro\j\pgfmathresult
  
  \draw[edge,niceArrows,thick] (a\i) -- (b\j) ;
  \draw[edge,niceArrows,thick] (b\i) -- (a\j) ;
}

\node at (a1) {\knoteninhalt{$c_1$\\$s$}} ;
\node at (a4) {\knoteninhalt{$c_2$\\$s$}} ;
\node at (a7) {\knoteninhalt{$c_2$\\$c_3$\\$s$}} ;
\node at (b1) {\knoteninhalt{$c_2$\\$s$}} ;
\node at (b4) {\knoteninhalt{$c_1$\\$c_3$\\$s$}} ;
\node at (b7) {\knoteninhalt{$c_1$\\$s$}} ;

\foreach \i in {2,3,5,6,8,9}
{
  \node at (a\i) {\knoteninhalt{$s$}} ;
  \node at (b\i) {\knoteninhalt{$s$}} ;
}
\end{tikzpicture}
}
%----------------------------
\newcommand{\FXwedgeneu}{%
\begin{tikzpicture}[x=10mm,niceArrows]
\tikzstyle{vertex}=[circle,draw=black,thick,minimum size=5.5mm,inner sep=.5mm]
\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=40pt,inner sep=2pt]

\node[vertex,label=below:{$w_1$}] (ql1) at (0,2) {};
\node[vertex] (endel) at (12,2) { } ;

\foreach \i/\la in {{1/a},{4/b},{7/d}}
{
  \node[evertex] (al\i) at (2+\i,3.5) {} ;
  \node[evertex] (bl\i) at (2+\i,0.5) {} ;
}
\foreach \i/\la in {{1/a},{4/b},{7/d}}
{
  \node[yshift=10mm,anchor=base] at (al\i) {$\la$} ; 
  \node[yshift=-12mm,anchor=base] at (bl\i) {$\neg \la$} ; 
}
\node at (al1) {\knoteninhalt{$c_1$}} ;
\node at (al4) {\knoteninhalt{$c_2$}} ;
\node at (al7) {\knoteninhalt{$c_2$\\$c_3$}} ;
\node at (bl1) {\knoteninhalt{$c_2$}} ;
\node at (bl4) {\knoteninhalt{$c_1$\\$c_3$}} ;
\node at (bl7) {\knoteninhalt{$c_1$}} ;
\foreach \i [count=\j from 2] in {1,4}
{
  % berechne erstmal \j=\i+3
  \pgfmathparse{\i+3}  
  \pgfmathtruncatemacro\j\pgfmathresult
 
  \draw[edge,niceArrows,thick] (al\i) -- (al\j) ;
  \draw[edge,niceArrows,thick] (bl\i) -- (bl\j) ;
  \draw[edge,niceArrows,thick] (al\i) -- (bl\j) ;
  \draw[edge,niceArrows,thick] (bl\i) -- (al\j) ;
}

\draw[edge,niceArrows,thick] (ql1) -- (al1) ;
\draw[edge,niceArrows,thick] (ql1) -- (bl1) ;
\draw[edge,niceArrows,thick] (al7) -- (endel) ;
\draw[edge,niceArrows,thick] (bl7) -- (endel) ;
\draw[edge,niceArrows,thick] (endel) edge[loop right] (endel) ;

\end{tikzpicture}
}

% - - -- - - --  PSPACE-Härte von MDL

%----------------------------
\newcommand{\MDLa}{%
\begin{tikzpicture}[x=5mm,niceArrows]
\tikzstyle{vertex}=[circle,draw=black,thick,minimum size=5.5mm,inner sep=.5mm]
\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=40pt,inner sep=2pt]

\node[vertex,label=below:{$d^1_1$}] (ql1) at (0,2) {};

\foreach \i/\la in {{1/a}}
{
  \node[evertex] (al\i) at (2+\i,3.5) {} ;
  \node[evertex] (bl\i) at (2+\i,0.5) {} ;
}
\foreach \i/\la in {{1/a}}
{
  \node[yshift=10mm,anchor=base] at (al\i) {$\la^1$} ; 
  \node[yshift=-12mm,anchor=base] at (bl\i) {$\la^0$} ; 
}
\node at (al1) {\knoteninhalt{$a^1$\\$c_1$}} ;
\node at (bl1) {\knoteninhalt{$a^0$\\$c_2$}} ;

\draw[edge,niceArrows,thick] (ql1) -- (al1) ;
\draw[edge,niceArrows,thick] (ql1) -- (bl1) ;
\draw[edge,niceArrows,thick] (al1) edge[loop right] (al1) ;
\draw[edge,niceArrows,thick] (bl1) edge[loop right] (bl1) ;

\end{tikzpicture}
}

%----------------------------
\newcommand{\MDLb}{%
\begin{tikzpicture}[x=5mm,niceArrows]
\tikzstyle{vertex}=[circle,draw=black,thick,minimum size=5.5mm,inner sep=.5mm]
\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=40pt,inner sep=2pt]

\node[vertex,label=below:{$d^1_2$}] (ql1) at (0,2) {};
\node[vertex,label=below:{$d^2_2$}] (ql2) at (3,2) {};

\foreach \i/\la in {{4/b}}
{
  \node[evertex] (al\i) at (2+\i,3.5) {} ;
  \node[evertex] (bl\i) at (2+\i,0.5) {} ;
}
\foreach \i/\la in {{4/b}}
{
  \node[yshift=10mm,anchor=base] at (al\i) {$\la^1$} ; 
  \node[yshift=-12mm,anchor=base] at (bl\i) {$\la^0$} ; 
}
\node at (al4) {\knoteninhalt{$b^1$\\$c_2$}} ;
\node at (bl4) {\knoteninhalt{$b^0$\\$c_1$\\$c_3$}} ;


\draw[edge,niceArrows,thick] (ql1) -- (ql2) ;
\draw[edge,niceArrows,thick] (ql2) -- (al4) ;
\draw[edge,niceArrows,thick] (ql2) -- (bl4) ;
\draw[edge,niceArrows,thick] (al4) edge[loop right] (al4) ;
\draw[edge,niceArrows,thick] (bl4) edge[loop right] (bl4) ;

\end{tikzpicture}
}

%----------------------------
\newcommand{\MDLc}{%
\begin{tikzpicture}[x=5mm,niceArrows]
\tikzstyle{vertex}=[circle,draw=black,thick,minimum size=5.5mm,inner sep=.5mm]
\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=16pt,minimum height=40pt,inner sep=2pt]

\node[vertex,label=below:{$d^1_3$}] (ql1) at (0,2) {};
\node[vertex,label=below:{$d^2_3$}] (ql2) at (3,2) {};
\node[vertex,label=below:{$d^3_3$}] (ql3) at (6,2) {};

\foreach \i/\la in {{7/e}}
{
  \node[evertex] (al\i) at (2+\i,3.5) {} ;
  \node[evertex] (bl\i) at (2+\i,0.5) {} ;
}
\foreach \i/\la in {{7/e}}
{
  \node[yshift=10mm,anchor=base] at (al\i) {$\la^1$} ; 
  \node[yshift=-12mm,anchor=base] at (bl\i) {$\la^0$} ; 
}
\node at (al7) {\knoteninhalt{$e^1$\\$c_2$\\$c_3$}} ;
\node at (bl7) {\knoteninhalt{$e^0$\\$c_1$}} ;

\draw[edge,niceArrows,thick] (ql1) -- (ql2) ;
\draw[edge,niceArrows,thick] (ql2) -- (ql3) ;
\draw[edge,niceArrows,thick] (ql3) -- (al7) ;
\draw[edge,niceArrows,thick] (ql3) -- (bl7) ;
\draw[edge,niceArrows,thick] (al7) edge[loop right] (al7) ;
\draw[edge,niceArrows,thick] (bl7) edge[loop right] (bl7) ;

\end{tikzpicture}
}



%============= TILING ======================================================================
\definecolor{darkgrey}{gray}{0.4}

\definecolor{dyellow}{gray}{0.5}
\definecolor{dred}{gray}{0}
\definecolor{dblue}{gray}{1}

\tikzstyle{kvertex}=[circle,draw,minimum size=16pt,inner sep=0pt]

\tikzstyle{rvertex}= [rectangle, minimum width=30pt, minimum height=30pt]
\tikzstyle{smalltile}= [rectangle, minimum width=20pt, minimum height=20pt]

%% setze einen Domino-Stein an Position #1 mit Farben #2..#5
\newcommand{\tile}[5]{%

\node[rvertex]  at (#1) { };

\filldraw[fill=#2] (#1.north west) -- (#1.center) -- (#1.north east) -- cycle ;
\filldraw[fill=#3] (#1.north east) -- (#1.center) -- (#1.south east) -- cycle ;
\filldraw[fill=#4] (#1.south east) -- (#1.center) -- (#1.south west) -- cycle ;
\filldraw[fill=#5] (#1.south west) -- (#1.center) -- (#1.north west) -- cycle ;

}

% setze einen Domino-Stein vom Typ A an Position #1
\newcommand{\tilea}[1]{%
  \tile{#1}{dred}{dblue}{dyellow}{dblue} ;
}
% ... vom Typ B ...
\newcommand{\tileb}[1]{%
  \tile{#1}{dred}{dyellow}{dred}{dblue} ;
}
% ... Typ C ...
\newcommand{\tilec}[1]{%
  \tile{#1}{dyellow}{dblue}{dyellow}{dyellow} ;
}
% ... Typ D ...
\newcommand{\tiled}[1]{%
  \tile{#1}{dyellow}{dyellow}{dred}{dyellow} ;
}


% Beispiel für ein Kripke-Modell, das aus einem Tiling-Problem erzeugt wird
\newcommand{\kripketiling}{%
\begin{tikzpicture}[x=20mm,edge/.style={draw,thick,niceArrows}]

% die Senke
\node[kvertex,minimum width=9mm,thick,label=above:{$s$}] (ende) at (5,0) { } ;

% male die Domino-Knoten im Graph
\foreach \i in {1,2,3,4}{
\foreach \pos / \name / \tttt in {{(\i,0)/a1/\tilea}, {(\i,2)/a2/\tileb}, {(\i,4)/a3/\tilec}, {(\i,6)/a4/\tiled}}
{
   \node[smalltile] (\name\i) at \pos { } ;
   \tttt{\name\i} 
} 
}

% die Kanten zwischen den Domino-Steinen
\foreach \i [count=\j from 2] in {1,2,3}
{
  \path[edge] (a1\i.east) -- (a1\j.west) ;
  \path[edge] (a1\i.east) -- (a2\j.west) ;
  \path[edge] (a2\i.east) -- (a3\j.west) ;
  \path[edge] (a2\i.east) -- (a4\j.west) ;
  \path[edge] (a3\i.east) -- (a1\j.west) ;
  \path[edge] (a3\i.east) -- (a2\j.west) ;
  \path[edge] (a4\i.east) -- (a3\j.west) ;
  \path[edge] (a4\i.east) -- (a4\j.west) ;
}

% die Kanten zum Fehlerzustand
\path[edge] (a14.east) -- (ende) ;
\path[edge] (a24.east) -- (ende) ;
\path[edge] (ende) edge[loop right] (ende) ;

% die Kanten vom rechten Rand zurück zum Anfang
\path[edge,-] (0.5,0) -- (0.5,7.5) -- (4.5,7.7) -- (4.5,4) ;
\path[edge,-] (a34.east) -- (4.5,4) ;
\path[edge,-] (a44.east) -- (4.5,6) ;
\path[edge] (0.5,0) -- (a11.west) ;
\path[edge] (0.5,2) -- (a21.west) ;
\path[edge] (0.5,4) -- (a31.west) ;
\path[edge] (0.5,6) -- (a41.west) ;


\end{tikzpicture}
}

%%  -- Noch ein weiteres Beispiel

\newcommand{\tilecc}[1]{%
  \tile{#1}{dred}{dred}{dyellow}{dyellow} ;
}

\newcommand{\tileaa}[1]{%
  \tile{#1}{dyellow}{dred}{dblue}{dyellow} ;
}

\newcommand{\tilebb}[1]{%
  \tile{#1}{dblue}{dyellow}{dred}{dred} ;
}


\newcommand{\tilebild}{%
\begin{tikzpicture}

\node[rvertex] (a) at (0,0) { };

\tilea{a} ;

\end{tikzpicture}
}

\newcommand{\beispielinstanz}{%
\begin{tikzpicture}

\node ( ) at (-2,0) {Tiling instance:} ;
\node[rvertex] (a) at (2,0) { };
\node[rvertex] (b) at (4,0) { };
\node[rvertex] (c) at (6,0) { };
\node[rvertex] (d) at (6,0) {$1111$};

\tileaa{a} ;
\tilebb{b} ;
\tilecc{c} ;

\node[below=4mm of a,anchor=base] (d) {$r$} ;
\node[below=4mm of b,anchor=base] {$q$} ;
\end{tikzpicture}
}

\newcommand{\nocheinkripketiling}{%
\begin{tikzpicture}[x=20mm,edge/.style={draw,thick,niceArrows}]


\node[anchor=west] ( ) at (-1,8) {Tiling instance:} ;
\node[rvertex] (a) at (1,8) { };
\node[rvertex] (b) at (2,8) { };
\node[rvertex] (c) at (3,8) { };
\node[rvertex] (d) at (4,8) {${1111}$};

\tileaa{a} ;
\tilebb{b} ;
\tilecc{c} ;

\node[below=4mm of a,anchor=base] (d) {$r$} ;
\node[below=4mm of b,anchor=base] {$q$} ;


\node[anchor=west] ( ) at (-1,5) {Kripke model:} ;

% male die Domino-Knoten im Graph
\foreach \i in {1,2,3,4}{
\foreach \pos / \name / \tttt in {{(\i,0)/a1/\tileaa}, {(\i,2)/a2/\tilebb}, {(\i,4)/a3/\tilecc}}
{
   \node[smalltile] (\name\i) at \pos { } ;
   \tttt{\name\i} 
} 
}

% die Kanten zwischen den Domino-Steinen
\foreach \i [count=\j from 2] in {1,2,3}
{
  \path[edge] (a1\i.east) -- (a2\j.west) ;
  \path[edge] (a2\i.east) -- (a1\j.west) ;
  \path[edge] (a2\i.east) -- (a3\j.west) ;
  \path[edge] (a3\i.east) -- (a2\j.west) ;
}

% die Schleife am letzten Zustand
\node[kvertex,minimum width=9mm,thick] (ende) at (5,0) { } ;
\path[edge] (ende) edge[loop right,min distance=6mm] (ende);
\path[edge] (a14.east) -- (ende) ;

% die Kanten vom rechten Rand zurück zum Anfang
\path[edge,-] (0.5,0) -- (0.5,5.5) -- (4.5,5.5) -- (4.5,2) ;
\path[edge,-] (a34.east) -- (4.5,4) ;
\path[edge,-] (a24.east) -- (4.5,2) ;
\path[edge] (0.5,0) -- (a11.west) ;
\path[edge] (0.5,2) -- (a21.west) ;
\path[edge] (0.5,4) -- (a31.west) ;

\node[xshift=-2mm] () at (a21.south west) {$q^1$} ;

\end{tikzpicture}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\BooleanClones}{
% Die Struktur der Boolean Clones für Model Checking
\node (BF) at (4,4) {$\wedge,\oplus$} ;

\node (M) at (3,3) {$\wedge,\vee$} ;
\node (E) at (2.5,2) {$\wedge$} ;
\node (V) at (3.5,2) {$\vee$} ;

\node (L) at (5,3) {$\oplus$} ;
\node (N) at (5,2) {$\neg$} ;

\node (I) at (4,1) {\emph{id}} ;

% weitere Punkte, um später Abgrenzungslinien zu zeichnen

%\node (linksoben) at (1,3.5) {} ;
%\node (mitteoben) at (4,3.5) {} ;
%\node (rechtsoben) at (5.5,3.5) {} ;
%\node (linksmitte) at (1,2.5) {} ;
%\node (mittemitte) at (4,2.5) {} ;
%\node (rechtsmitte) at (5.5,2.5) {} ;
%\node (linksunten) at (1,1.5) {} ;
%\node (mitteunten) at (4,1.5) {} ;
%\node (rechtsunten) at (6,1.5) {} ;


\draw[edge] (M) -- (BF) 
            (L) -- (BF) 
            (V) -- (M) 
            (E) -- (M)
            (N) -- (L)
            (I) -- (E)
            (I) -- (V)
            (I) -- (N) ;
}

%--------------------------------------------
\newcommand{\ClonesBild}{
\begin{tikzpicture}[x=12mm,y=12mm,scale=0.85] 
\tikzstyle{edge}=[draw,thick,-]

\BooleanClones

\end{tikzpicture}
}
%---------------------------------------------
\newcommand{\MLResultate}{
\begin{tikzpicture}[x=12mm,y=12mm] 
\tikzstyle{edge}=[draw,thick,-]

% Die Struktur der Boolean Clones für Model Checking
\node (BF1) at (5,4.6) {$\wedge,\oplus$} ;

\node (M1) at (4,2.8) {$\wedge,\vee$} ;
\node (E1) at (3.5,2.2) {$\wedge$} ;
\node (V1) at (4.5,1.7) {$\vee$} ;

\node (L1) at (6,4.1) {$\oplus$} ;
\node (N1) at (6,3.5) {$\neg$} ;

\node (I1) at (5,1) {\emph{id}} ;
\node at (5,0.4) {$\Diamond$} ;


\foreach \x in {6.8}{ % \x dient zur einfachen Verschiebung nach rechts oder links

\node (BF2) at (2+\x,4.6) {$\wedge,\oplus$} ;

\node (M2) at (0.5+\x,2.8) {$\wedge,\vee$} ;
\node (E2) at (\x,1.7) {$\wedge$} ;
\node (V2) at (1+\x,2.2) {$\vee$} ;

\node (L2) at (2.5+\x,4.1) {$\oplus$} ;
\node (N2) at (2.5+\x,3.5) {$\neg$} ;

\node (I2) at (1.5+\x,1) {\emph{id}} ;
\node at (1.5+\x,0.4) {$\Box$} ;
}

\foreach \i in {1,2}
\draw[edge] (M\i) -- (BF\i) 
            (L\i) -- (BF\i) 
            (V\i) -- (M\i) 
            (E\i) -- (M\i)
            (N\i) -- (L\i)
            (I\i) -- (E\i)
            (I\i) -- (V\i)
            (I\i) -- (N\i) ;
            
            
\node (I3) at (11,3.5) {\emph{id}} ;
\node (BF3) at (11,4.6) {$\wedge,\oplus$} ;
\node at (11,0.4) {$\Diamond,\Box$} ;
\draw[thick,dotted] (I3) -- (BF3) ;

\draw[draw] (0.5,3.2) -- (11.5,3.2) ;

\draw[draw] (0.5,2) -- (11.5,2) ; 

\node[anchor=south west] at (0.5,3.2) {$\P$-complete} ;
\node[anchor=south west] at (0.5,2) {$\LOGCFL$-c.} ;
\node[anchor=south west] at (0.5,1.2) {$\NL$-complete} ;
\node[anchor=west] at (0.5,0.4) {with modal operator} ;

\end{tikzpicture}
}
%-----------------------------------------------
\newcommand{\CTLOperatorHierarchie}{
\begin{tikzpicture}[x=12mm,y=5mm,scale=0.7] 
\tikzstyle{edge}=[draw,thick,niceArrows]
\tikzstyle{vertex}=[rectangle,rounded corners,draw=black,thick,minimum size=16pt,inner sep=1pt]

\node[vertex] (EU) at (8,0) {$\EU$~$\AR$} ;

\node[vertex] (ER) at (6,0) {$\ER$~$\AU$} ;

\node[vertex] (EX) at (4,-2) {$\EX$} ;
\node[vertex] (AG) at (4,0) {$\AX$} ;
\node[vertex] (EG) at (4,2) {$\EG$~$\AF$} ;

\node[vertex] (EF) at (2,-2) {$\EF$} ;
\node[vertex] (AX) at (2,0) {$\AG$} ;

\draw[edge] (ER) -- (EU) ;
\draw[edge] (EX) -- (ER) ;
\draw[edge] (AG) -- (ER) ;
\draw[edge] (EG) -- (ER) ;
\draw[edge] (EF) -- (EX) ;
\draw[edge] (AX) -- (AG) ;

\end{tikzpicture}
}

%---------------------------------------------
\newcommand{\CTLResultate}{
\begin{tikzpicture}[x=10.4mm,y=11.8mm,scale=0.85,every node/.style={}] 
\tikzstyle{edge}=[draw,thick,-]


% -- EX
\foreach \x in {3.7}{
\node (BF3) at (\x,4.9) {$\wedge,\oplus$} ;

\node (M3) at (\x-0.4,2.7) {$\wedge,\vee$} ;
\node (E3) at (\x-0.9,2.1) {$\wedge$} ;
\node (V3) at (\x,1.6) {$\vee$} ;

\node (L3) at (\x+0.9,4.5) {$\oplus$} ;
\node (N3) at (\x+0.9,4.1) {$\neg$} ;

\node (I3) at (\x,1.1) {\emph{id}} ;
\node at (\x,0.5) {$\EX$} ;
}

% -- EG
\foreach \x in {6.2}{
\node (BF1) at (\x,4.9) {$\wedge,\oplus$} ;

\node (M1) at (\x-.5,4.1) {$\wedge,\vee$} ;
\node (E1) at (\x-1,1.7) {$\wedge$} ;
\node (V1) at (\x,1.7) {$\vee$} ;

\node (L1) at (\x+.8,4.1) {$\oplus$} ;
\node (N1) at (\x+.8,1.7) {$\neg$} ;

\node (I1) at (\x,1.1) {\emph{id}} ;
\node at (\x,0.5) {$\EG$} ;
}

% -- EU
\foreach \x in {8}{
\node (BF2) at (\x,4.9) {$\wedge,\oplus$} ;

\node (I2) at (\x,4.1) {\emph{id}} ;
\node at (\x,0.5) {$\EU$} ;
}

% -- EF
\foreach \x in {9.95}{
\node (BF4) at (\x,4.9) {$\wedge,\oplus$} ;

\node (M4) at (\x-.5,2.7) {$\wedge,\vee$} ;
\node (E4) at (\x-1,2.1) {$\wedge$} ;
\node (V4) at (\x,1.7) {$\vee$} ;

\node (L4) at (\x+1,3.7) {$\oplus$} ;
\node (N4) at (\x+1,1.7) {$\neg$} ;

\node (I4) at (\x,1.1) {\emph{id}} ;
\node at (\x,0.5) {$\EF$} ;
}


% -- ER
\foreach \x in {12.45}{
\node (BF5) at (\x,4.9) {$\wedge,\oplus$} ;

\node (M5) at (\x-.75,4.4) {$\wedge,\vee$} ;
\node (E5) at (\x-.75,3.15) {$\wedge$} ;
\node (V5) at (\x,4.1) {$\vee$} ;

\node (L5) at (\x+1,4.5) {$\oplus$} ;
\node (N5) at (\x+1,4.1) {$\neg$} ;

\node (I5) at (\x,2.5) {\emph{id}} ;
\node at (\x,0.5) {$\ER$} ;
}


% -- 

\foreach \i in {1,3,4,5}
\draw[edge] (M\i) -- (BF\i) 
            (L\i) -- (BF\i) 
            (V\i) -- (M\i) 
            (E\i) -- (M\i)
            (N\i) -- (L\i)
            (I\i) -- (E\i)
            (I\i) -- (V\i)
            (I\i) -- (N\i) ;
            
\draw[edge, dotted] (I2) -- (BF2);
%\draw[edge, dotted] (BF5) -- (N5);
%\draw[edge] (I5) -- (E5) (I5) -- (V5) (I5) -- (N5) (V5) -- (M5);
%\draw[edge] (E5) -- (M5) (M5) -- (BF5);


\draw[draw,dashed] (0.5,3.9) -- (13.8,3.9) ;
\draw[draw,dashed] (0.5,3.4) -- (13.8,3.4) ;
\draw[draw] (0.5,2.9) -- (13.8,2.9) ;
\draw[draw] (0.5,1.9) -- (13.8,1.9) ;


\node[anchor=south west] at (0.5,4.0) {$\P$-complete} ;
\node[anchor=south west] at (0.5,3.4) {$\AC1$-hard} ;
\node[anchor=south west] at (0.5,2.95) {$\LOGCFL$-hard} ;
\node[anchor=south west] at (0.5,2.2) {$\LOGCFL$-c.} ;
\node[anchor=south west] at (0.5,1.2) {$\NL$-complete} ;
\node[anchor=west] at (0.5,0.5) {\CTL operator} ;

\end{tikzpicture}
}

%---------------------------------------------------------------

\newcommand{\LTLUebersicht}{
\begin{tikzpicture}[x=10.8mm,y=11mm] 
\tikzstyle{edge}=[draw,thick,-]


% Die Struktur der Boolean Clones für FX
\node (BF1) at (4,4.5) {$\wedge,\oplus$} ;

\node (M1) at (3,2.4) {$\wedge,\vee$} ;
\node (E1) at (2.5,1.6) {$\wedge$} ;
\node (V1) at (3.5,0.9) {$\vee$} ;

\node (L1) at (5,3.1) {$\oplus$} ;
\node (N1) at (5,0.9) {$\neg$} ;

\node (I1) at (4,0) {\emph{id}} ;


% Die Struktur der Boolean Clones für GX
\node (BF2) at (7,4.5) {$\wedge,\oplus$} ;

\node (M2) at (6,3.9) {$\wedge,\vee$} ;
\node (E2) at (5.5,0.9) {$\wedge$} ;
\node (V2) at (6.5,3.1) {$\vee$} ;

\node (L2) at (8,3.1) {$\oplus$} ;
\node (N2) at (8,0.9) {$\neg$} ;

\node (I2) at (7,0) {\emph{id}} ;

% Die Struktur der Boolean Clones für FGX
\node (BF3) at (10,4.5) {$\wedge,\oplus$} ;

\node (M3) at (9,3.9) {$\wedge,\vee$} ;
\node (E3) at (8.5,3.1) {$\wedge$} ;
\node (V3) at (9.5,3.1) {$\vee$} ;

\node (L3) at (11,3.1) {$\oplus$} ;
\node (N3) at (11,0.9) {$\neg$} ;

\node (I3) at (10,0) {\emph{id}} ;

% Die Struktur der Boolean Clones für U
\node (BF4) at (12.5,4.5) {$\wedge,\oplus$} ;

\node (M4) at (11.5,3.9) {$\wedge,\vee$} ;
\node (E4) at (11.5,3.3) {$\wedge$} ;
\node (V4) at (12,3.3) {$\vee$} ;
%
\node (L4) at (13.2,3.3) {$\oplus$} ;
%\node (N3) at (12,0.9) {$\neg$} ;

\node (I4) at (12.5,2.9) {\emph{id}} ;


\foreach \i in {1,2,3} {
\draw[edge] (M\i) -- (BF\i) 
            (L\i) -- (BF\i) 
            (V\i) -- (M\i) 
            (E\i) -- (M\i)
            (N\i) -- (L\i)
            (I\i) -- (E\i)
            (I\i) -- (V\i)
            (I\i) -- (N\i) ;
}

\draw[edge] (M4) -- (BF4)
            (L4) -- (BF4)
            (I4) -- (E4)
            (I4) -- (V4)
            (E4) -- (M4)
            (V4) -- (M4) ;
\draw[edge,dotted] (I4) -- (L4) ;

\draw[draw] (1,3.5) -- (13.7,3.5) ;
\draw[draw,dashed] (1,2.75) -- (13.7,2.75) ;
\draw[draw] (1,1.25) -- (13.7,1.25) ;

\node[anchor=west] at (1,3.9) {$\PSPACE$-c.} ;
\node[anchor=west] at (1,3.1) {$\NP$-hard} ;
\node[anchor=west] at (1,2) {$\NP$-c.} ;
\node[anchor=west] at (1,0.5) {$\NL$-complete} ;
\node at (4,-1) {$\F,\X$} ;
\node at (7,-1) {$\G,\X$} ;
\node at (10,-1) {$\F,\G,\X$} ;
\node at (12.5,-1) {$\U$ resp. $\R$} ;

\end{tikzpicture}
}

%-----------------------------------------------------------
%------------Modal Dependence Logic-----Anfang--------------
\newcommand{\knoteninhaltii}[1]{
\begin{minipage}{30pt}

\centering

#1

\end{minipage}
}
\newcommand{\mtlpspacecomplete}{%
\begin{tikzpicture}
	\tikzstyle{world}=[thick,draw=black,circle,minimum size=5.5mm,inner sep=0.5mm]
	\tikzstyle{evertex}=[rectangle,draw=black,thick,minimum size=32pt,minimum height=40pt,inner sep=2pt]

	\node[world] (v)[label=below:{$d_1^1$}] at (0,0) {$\ast$};
	\node[evertex] (v11)[label=below:{$\neg{x}_1$}] at (1.5,-2) {\knoteninhaltii{$p_1^0$\\$p_2^0, p_2^1$\\$p_3^0, p_3^1$}} ; %{$p_1^0$};
	\node[evertex] (v12)[label=below:{$x_1$}] at (1.5,2) {\knoteninhaltii{$p_1^1$\\$p_2^0, p_2^1$\\$p_3^0, p_3^1$}} ; % {$p_1^1$};
%	\node[world] (v21)[label=below:{$\lANeg{v}_1^2$}] at (3,-2) {$p_1^0$};
%	\node[world] (v22)[label=below:{$v_1^2$}] at (3,2) {$p_1^1$};
%	\node[world] (v31)[label=below:{$\lANeg{v}_1^3$}] at (4.5,-2) {$p_1^0$};
%	\node[world] (v32)[label=below:{$v_1^3$}] at (4.5,2) {$p_1^1$};
	
	\node[world] (u)[label=below:{$d_2^1$}] at (6,0) {$\ast$};
	\node[world] (u1)[label=below:{$d_2^2$}] at (7.5,0) {$\ast$};
	\node[evertex] (u21)[label=below:{$\neg{x}_2$}] at (9,-2) {\knoteninhaltii{$p_1^0, p_1^1$\\$p_2^0$\\$p_3^0, p_3^1$}} ; % {$p_2^0$};
	\node[evertex] (u22)[label=below:{$x_2$}] at (9,2) {\knoteninhaltii{$p_1^0, p_1^1$\\$p_2^1$\\$p_3^0, p_3^1$}} ; %{$p_2^1$};
%	\node[world] (u31)[label=below:{$\lANeg{v}_2^2$}] at (10.5,-2) {$p_2^0$};
%	\node[world] (u32)[label=below:{$v_2^2$}] at (10.5,2) {$p_2^1$};
	
	\node[world] (t)[label=below:{$d_3^1$}] at (12,0) {$\ast$};
	\node[world] (t1)[label=below:{$d_3^2$}] at (13.5,0) {$\ast$};
	\node[world] (t2)[label=below:{$d_3^3$}] at (15,0) {$\ast$};
	\node[evertex] (t31)[label=below:{$\neg{x}_3$}] at (16.5,-2) {\knoteninhaltii{$p_1^0, p_1^1$\\$p_2^0,p_2^1$\\$p_3^0$}} ; % {$p_3^0$};
	\node[evertex] (t32)[label=below:{$x_3$}] at (16.5,2)  {\knoteninhaltii{$p_1^0, p_1^1$\\$p_2^0,p_2^1$\\$p_3^1$}} ; %{$p_3^1$};

{\tikzset{niceArrows}	
	\draw[niceArrows,thick] (v) -- (v11); 
	\draw[niceArrows,thick] (v) -- (v12);
	\draw[niceArrows,thick] (v11) edge[loop right] (v11);
	\draw[niceArrows,thick] (v12) edge[loop right] (v12);

	
%	\draw[->,thick] (v11) -- (v21);
%	\draw[->,thick] (v12) -- (v22);
%	\draw[->,thick] (v21) -- (v31);
%	\draw[niceArrows,thick] (v22) -- (v32);

	\draw[niceArrows,thick] (u) -- (u1);
	\draw[niceArrows,thick] (u1) -- (u21); 
	\draw[niceArrows,thick] (u1) -- (u22);
	\draw[niceArrows,thick] (u21) edge[loop right] (u21);
	\draw[niceArrows,thick] (u22) edge[loop right] (u22);


%	\draw[->,thick] (u21) -- (u31); 
%	\draw[->,thick] (u22) -- (u32);
	\draw[niceArrows,thick] (t) -- (t1);
	\draw[niceArrows,thick] (t1) -- (t2); 
	\draw[niceArrows,thick] (t2) -- (t31);
	\draw[niceArrows,thick] (t2) -- (t32);
	\draw[niceArrows,thick] (t31) edge[loop right] (t31);
	\draw[niceArrows,thick] (t32) edge[loop right] (t32);
}
\end{tikzpicture}
}

\newcommand{\mdlnpcomplete}{%
\begin{tikzpicture}[x=9mm]
	\tikzstyle{world}=[thick,draw=black,circle,minimum size=10mm,inner sep=0.5mm]
	
	\node[world,label=above:{$C_1$}] (c1) at (3,0) {};
	
	\node[world,label=above:{$C_2$}] (c2) at (5,0) { };
	
	\node[world,label=above:{$C_3$}] (c3) at (7,0) { };
	
	\node[world, label=below:{$x_1$}] (s11) at (0,-4) {$p_1,q$};
	\node[world, label=below:{$\neg x_1$}] (s10) at (2,-4) {$p_1$};
	
	\node[world, label=below:{$x_2$}] (s21) at (4,-4) {$p_2,q$};
	\node[world, label=below:{$\neg x_2$}] (s20) at (6,-4) {$p_2$};
	
	\node[world, label=below:{$x_3$}] (s31) at (8,-4) {$p_3,q$};
	\node[world, label=below:{$\neg x_3$}] (s30) at (10,-4) {$p_3$};

{\tikzset{niceArrows}
	\draw[niceArrows,thick] (c1) -- (s11); 
	\draw[niceArrows,thick] (c1) -- (s20); 
	\draw[niceArrows,thick] (c1) -- (s31); 
	\draw[niceArrows,thick] (c2) -- (s10); 
	\draw[niceArrows,thick] (c2) -- (s30); 
	\draw[niceArrows,thick] (c2) -- (s21);
	\draw[niceArrows,thick] (c3) -- (s21); 
	\draw[niceArrows,thick] (c3) -- (s11); 
	\draw[niceArrows,thick] (c3) -- (s30);
}
\end{tikzpicture}
}

\newcommand{\mdlMlExample}{%
	\begin{tikzpicture}
		\tikzstyle{world}=[thick,draw=black,ellipse,minimum size=5.5mm,inner sep=0mm]
		
		\node[world] (S1)[label=above:{$s_1$}] at (0,0)              {};
		\node[world] (S2)[label=left:{$s_2$}] at (-4,-2) {};
		\node[world] (S3)[label=left:{$s_3$}] at (0,-2) {};
		\node[world] (S4)[label=right:{$s_4$}] at (4,-2) {};
		\node[world, label=below:{$s_5$}] (S5) at (-5,-4)      {$p,r$};
		\node[world, label=below:{$s_6$}] (S6)  at (-3,-4)       {$p,q,r$};
		\node[world, label=below:{$s_7$}] (S7)  at (-1,-4)      {$q,r$};
		\node[world, label=below:{$s_8$}] (S8)  at (1,-4)     {$p$};
		\node[world, label=below:{$s_9$}] (S9)  at (3,-4)       {$q,r$};
		\node[world, label=below:{$s_{10}$}] (S10)  at (5,-4)       {$p,q$};

{\tikzset{niceArrows}
		\draw[niceArrows,thick] (S1) -- (S2);
		\draw[niceArrows,thick] (S1) -- (S3);
		\draw[niceArrows,thick] (S1) -- (S4);
		\draw[niceArrows,thick] (S2) -- (S5);
		\draw[niceArrows,thick] (S2) -- (S6);
		\draw[niceArrows,thick] (S3) -- (S7);
		\draw[niceArrows,thick] (S3) -- (S8);
		\draw[niceArrows,thick] (S4) -- (S9);
		\draw[niceArrows,thick] (S4) -- (S10);
}
	\end{tikzpicture}
}

\newcommand{\MDlTractable} {
\begin{tikzpicture}[x=10.8mm,y=11mm] 
	\tikzstyle{edge}=[draw,thick,-]


{\tikzset{xshift=-1.4cm}
	% Die Struktur der Boolean Clones für dep()
	\node (BF1) at (5.5,1.3) {$\wedge,\neg$} ;

	\node (M1) at (4.5,0.8) {$\wedge,\varovee$} ;
	\node (E1) at (4,0.3) {$\wedge$} ;
	\node (V1) at (5,0.3) {$\varovee$} ;

	\node (N1) at (6.1,0.3) {$\neg$} ;
	
	\node (I1) at (5.5,-0.3) {\emph{id}};
	
	\node (DEP) at (5.5,-0.8) {$\mdlDep(\cdot)$};
	
	\draw[edge] (I1) -- (E1)
				(I1) -- (N1)
				(I1) edge[shorten >=-1pt, shorten <=-1pt] node {} (V1)
				(V1) edge[shorten >=-1pt, shorten <=-1pt] node {} (M1)
				(E1) edge[shorten >=-1pt, shorten <=-1pt] node {} (M1)
				(M1) edge[shorten >=-1pt, shorten <=-1pt] node {} (BF1)
				(N1) edge[shorten >=-1pt, shorten <=-1pt] node {} (BF1);
				
}
{\tikzset{xshift=-2.75cm}
	% Die Struktur der Boolean Clones für dpe()
	\node (BF2) at (9,4.5) {$\wedge,\neg$} ;

	\node (M2) at (8,4.0) {$\wedge,\varovee$} ;
	\node (E2) at (8,2.4) {$\wedge$} ;
	\node (V2) at (9,3.4) {$\varovee$} ;

	\node (N2) at (10.1,2.4) {$\neg$} ;
	
	\node (I2) at (9,1.9) {\emph{id}};
	
	\node (DEPBOX) at (9,-0.8) {$\mdlDep(\cdot),\mtlAll$};
	
	\draw[edge] (I2) -- (E2)
				(I2) -- (N2)
				(I2) -- (V2)
				(V2) -- (M2)
				(E2) -- (M2)
				(M2) -- (BF2)
				(N2) -- (BF2);
}
	\draw[draw] (1,3.0) -- (13.7,3.0) ;
	%\draw[draw,dashed] (1,2.75) -- (13.7,2.75) ;
	\draw[draw] (1,1.6) -- (13.7,1.6) ;
	\node[anchor=west] at (1,3.4) {$\LOGCFL$-c.} ;
	%\node[anchor=west] at (1,3.1) {$\NL$-hard} ;
	\node[anchor=west] at (1,2) {$\NL$-c.} ;
	\node[anchor=west] at (1,0.5) {$\NC{1}$-c.} ;
	

% Trennstrich
	\draw[white, line width=.5cm] (8.25,5.25) -- (8.25,-1.5);
	\draw[black, solid] (8.25,5.25) -- (8.25,-1.5);

% intractable part
	% Die Struktur der Boolean Clones für dpe()
{\tikzset{xshift=2cm}
	\node (BF3) at (8.2,3.5) {$\wedge,\neg$} ;

	\node (M3) at (7.4,1.2) {$\wedge,\varovee$} ;
	\node (E3) at (7,0.5) {$\wedge$} ;
	\node (V3) at (7.8,0.5) {$\varovee$} ;

	\node (N3) at (9.1,2.4) {$\neg$} ;
	
	\node (I3) at (8.2,-0.2) {\emph{id}};
	
	\node (DEPBOX2) at (8,-0.8) {$\mdlDep(\cdot),\mtlDiamond $};
	\node (DEPBOX2) at (8,-1.2) {or $\mdlDep(\cdot),\mtlDiamond,\mtlAll $};
	
	\draw[edge] 
				(I3) edge node {} (E3)
				(I3) -- (N3)
				(I3) -- (V3)
				(V3) -- (M3)
				(E3) -- (M3)
				(M3) -- (BF3)
				(N3) -- (BF3);


	\node[anchor=east] at (11.9,3.4) {$\PSPACE$-c.} ;
	%\node[anchor=east] at (11.9,3.1) {$\P^{\NP[1]}$-hard} ;
	\node[anchor=east] at (11.9,2) {$\P^{\NP[1]}$-c.} ;
	\node[anchor=east] at (11.9,0.5) {$\NP$-c.} ;
}

\end{tikzpicture}
}

\newcommand{\MDLIntractable} {
\begin{tikzpicture}[x=10.8mm,y=11mm] 
	\tikzstyle{edge}=[draw,thick,-]
				
	% Die Struktur der Boolean Clones für dpe()
	\node (BF1) at (8.2,4) {$\wedge,\neg$} ;

	\node (M1) at (7.4,1.2) {$\wedge,\varovee$} ;
	\node (E1) at (7,0.5) {$\wedge$} ;
	\node (V1) at (7.8,0.5) {$\varovee$} ;

	\node (L1) at (9.1,3.3) {$\oplus$} ;
	\node (N1) at (9.1,2.4) {$\neg$} ;
	
	\node (I1) at (8.2,-0.2) {\emph{id}};
	
	\node (DEPBOX) at (8,-0.8) {$\mdlDep(\cdot),\mtlDiamond $};
	\node (DEPBOX) at (8,-1.2) {or $\mdlDep(\cdot),\mtlDiamond,\mtlAll $};
	
	\draw[edge] (I1) edge node {} (E1)
				(I1) -- (N1)
				(I1) -- (V1)
				(V1) -- (M1)
				(E1) -- (M1)
				(M1) -- (BF1)
				(L1) -- (BF1)
				(N1) -- (L1);
				
	\draw[draw] (1,3.5) -- (13.7,3.5) ;
	\draw[draw,dashed] (1,2.75) -- (13.7,2.75) ;
	\draw[draw] (1,1.6) -- (13.7,1.6) ;

	
	
	\node[anchor=west] at (1,3.9) {$\PSPACE$-c.} ;
	\node[anchor=west] at (1,3.1) {$\P^{\NP[1]}$-hard} ;
	\node[anchor=west] at (1,2) {$\P^{\NP[1]}$-complete} ;
	\node[anchor=west] at (1,0.5) {$\NP$-complete} ;
\end{tikzpicture}
}

\newcommand{\MDLResultate}{
\begin{tikzpicture}
		\tikzstyle{world}=[x=1cm,y=.5cm,ellipse,draw=black,thick,minimum size=5.5mm,inner sep=1mm]
		\tikzstyle{conn}=[niceArrows]
		
		\node[] (start) at (5.7,-2.5)  {};
		\node[world] (nc12) at (2,0)  {$\NC1$};
		\node[world] (nc14) at (0,0)  {$\NC1$};
		\node[world] (nc11) at (4,0)  {$\NC1$};
		
		\node[world] (nc13) at (6,0)  {$\NC1$};
		\node[world] (nc15) at (8,0)  {$\NC1$};
		
		\node[world] (nl1) at (4,3)  {$\NL$};
		\node[world] (nl2) at (2,3)  {$\NL$};
		
		\node[world] (logcfl) at (4,6)  {$\LOGCFL$};
		
		\node[world] (np1) at (4,9)  {$\NP$};
		\node[world] (np2) at (6,9)  {$\NP$};
		
		\node[world] (pnp) at (6,12)  {$\P^{\NP[1]}$};
		
		\node[world] (pspace) at (4,15)  {$\PSPACE$};
		
		\path[conn] (start) edge node[xshift=-0.6cm] {$\textnormal{dep()}$}(nc11);
		\path[conn] (nc11) edge node[yshift=-0.3cm] {$\wedge$}(nc12);	
		\path[conn] (nc11) edge node[yshift=-0.3cm] {$\varovee$} (nc13);		
		\path[conn] (nc12) edge node[yshift=-0.3cm] {$\varovee$} (nc14);
		\path[conn] (nc12) edge node[xshift=-0.3cm] {$\Box$} (nl2);
		\path[conn] (nc13) edge node[yshift=-0.3cm] {$\wedge$} (nc15);
		
		\path[conn] (nc11) edge[in=-90,out=35] node[yshift=-0.7cm,xshift=0.1cm] {$\Diamond$}(np2);
		
		\path[conn] (nc14) edge[in=180,out=90] node[xshift=-0.5cm] {$\Box$} (logcfl);
		
		\path[conn] (nc15) edge[in=0,out=90] node[xshift=0.5cm] {$\Box$} (logcfl);
		
		\path[conn] (nc11) edge node[xshift=-0.3cm] {$\Box$} (nl1);
		
		\path[conn] (nl1) edge node[yshift=-0.3cm] {$\wedge$} (nl2);
		
		\path[conn] (nl2) edge node[xshift=0.35cm] {$\varovee$} (logcfl);
		
		\path[conn] (logcfl) edge node[xshift=-0.5cm] {$\vee,\Diamond$} (np1);
		
		\path[conn] (np1) edge node[xshift=-0.3cm] {$\neg$} (pspace);
		
		\path[conn] (np2) edge node[xshift=0.3cm] {$\neg$} (pnp);
		
		\path[conn] (pnp) edge[loop right] node {$\Box$} (pnp);
		\path[conn] (pnp) edge[out=90,in=0] node[xshift=0.5cm] {$\wedge,\varovee$} (pspace);
	\end{tikzpicture}
}
%------------Modal Dependence Logic-----Ende----------------
%-----------------------------------------------------------


%--- Temporal Logic Operators ---
\newcommand{\ctloperators}{%
 \begin{tikzpicture}[dot/.style={circle,draw=black,fill=black,inner sep=0mm, minimum width=2mm},y=1cm]
	\node[anchor=east] at (-.5,0.2) {$\EX\phi$:};
	\node[dot,label={north:}] (x1) at (0,0) {};
	\node[dot,label={north:$\phi$}] (x2) at (1,0) {};
	\node[dot,label={north:}] (x3) at (2,0) {};
	\node[dot,label={north:}] (x4) at (3,0) {};
	\node[dot,label={north:}] (x5) at (4,0) {};
	\node[dot,label={north:}] (x6) at (5,0) {};
	\path[niceArrows] 	(x1) edge node {} (x2)
								(x2) edge node {} (x3)
								(x3) edge node {} (x4)
								(x4) edge node {} (x5)
								(x5) edge node {} (x6);

	\node[anchor=east] at (-.5,-.8) {$\EF\phi$:};
	\node[dot,label={north:}] (f1) at (0,-1) {};
	\node[dot,label={north:}] (f2) at (1,-1) {};
	\node[dot,label={north:$\phi$}] (f3) at (2,-1) {};
	\node[dot,label={north:}] (f4) at (3,-1) {};
	\node[dot,label={north:}] (f5) at (4,-1) {};
	\node[dot,label={north:}] (f6) at (5,-1) {};
	\path[niceArrows] 	(f1) edge node {} (f2)
								(f2) edge[thick,dotted] node {} (f3)
								(f3) edge node {} (f4)
								(f4) edge node {} (f5)
								(f5) edge node {} (f6);

	\node[anchor=east] at (-.5,-1.8) {$\EG\phi$:};
	\node[dot,label={north:$\phi$}] (g1) at (0,-2) {};
	\node[dot,label={north:$\phi$}] (g2) at (1,-2) {};
	\node[dot,label={north:$\phi$}] (g3) at (2,-2) {};
	\node[dot,label={north:$\phi$}] (g4) at (3,-2) {};
	\node[dot,label={north:$\phi$}] (g5) at (4,-2) {};
	\node[dot,label={north:$\phi$}] (g6) at (5,-2) {};
	\path[niceArrows] 	(g1) edge node {} (g2)
								(g2) edge node {} (g3)
								(g3) edge node {} (g4)
								(g4) edge node {} (g5)
								(g5) edge node {} (g6);

	\node[anchor=east] at (8.5,0.2) {$\psi\EU\varphi$:};
	\node[dot,label={north:$\psi$}] (u1) at (9,0) {};
	\node[dot,label={north:$\psi$}] (u2) at (10,0) {};
	\node[dot,label={north:$\psi$}] (u3) at (11,0) {};
	\node[dot,label={north:$\varphi$}] (u4) at (12,0) {};
	\node[dot,label={north:}] (u5) at (13,0) {};
	\node[dot,label={north:}] (u6) at (14,0) {};
	\path[niceArrows] 	(u1) edge[thick,dotted] node {} (u2)
								(u2) edge node {} (u3)
								(u3) edge node {} (u4)
								(u4) edge node {} (u5)
								(u5) edge node {} (u6);

	\node[anchor=east] at (8.5,-.8) {$\psi\ER\varphi$:};
	\node[dot,label={north:$\varphi$}] (r1) at (9,-1) {};
	\node[dot,label={north:$\varphi$}] (r2) at (10,-1) {};
	\node[dot,label={north:$\varphi$}] (r3) at (11,-1) {};
	\node[dot,label={north:$\varphi,\psi$}] (r4) at (12,-1) {};
	\node[dot,label={north:}] (r5) at (13,-1) {};
	\node[dot,label={north:}] (r6) at (14,-1) {};
	\path[niceArrows] 	(r1) edge[thick,dotted] node {} (r2)
								(r2) edge node {} (r3)
								(r3) edge node {} (r4)
								(r4) edge node {} (r5)
								(r5) edge node {} (r6);
	\node[anchor=east] at (8.5,-1.8) {or};
	\node[dot,label={north:$\varphi$}] (r1b) at (9,-2) {};
	\node[dot,label={north:$\varphi$}] (r2b) at (10,-2) {};
	\node[dot,label={north:$\varphi$}] (r3b) at (11,-2) {};
	\node[dot,label={north:$\varphi$}] (r4b) at (12,-2) {};
	\node[dot,label={north:$\varphi$}] (r5b) at (13,-2) {};
	\node[label={north:$\cdots$}] (r6b) at (14,-2) {};
	\path[niceArrows] 	(r1b) edge node {} (r2b)
								(r2b) edge node {} (r3b)
								(r3b) edge node {} (r4b)
								(r4b) edge node {} (r5b)
								(r5b) edge[thick,dotted] node {} (r6b);
 \end{tikzpicture}
}

%-----------------------------------------------------------------------------------------------------------------------
\newcommand{\kknoteninhalt}[1]{
\begin{minipage}{32pt}

\centering

#1

\end{minipage}
}

\newcommand{\Gxor}{%
\begin{tikzpicture}[x=9mm,y=15mm]

\tikzstyle{edge} = [draw,thick,niceArrows]
\tikzstyle{tinyloopabove} = [draw,niceArrows,thick,in=-15,out=15,min distance=3mm,looseness=8]
\tikzstyle{vertex}=[rectangle,draw=black,thick,minimum size=30pt,minimum height=38pt,inner sep=0pt,fill=white]

\node[vertex,label={below:$p_0$}] (start) at (0,3) {\kknoteninhalt{$y$}} ;

\node[vertex,label={below:$p_1$}] (p1) at (2,3) {\kknoteninhalt{$x_1~\barx_1$}} ;
\node[vertex,label={below:$p_2$}] (p2) at (4,3) {\kknoteninhalt{$x_1~\barx_1$\\$x_2~\barx_2$}} ;
\node[vertex,label={below:$p_3$}] (p3) at (6,3) {\kknoteninhalt{$x_1~\barx_1$\\$x_2~\barx_2$\\$x_3~\barx_3$}} ;

%\node[] (aa) at (-0.4,0) {} ;

\node[vertex,label={below:$\bara_1$}] (a10) at (1,1) {\kknoteninhalt{$\barx_1$\\$x_2~\barx_2$\\$x_3~\barx_3$}} ;
\node[vertex,label={below:$a_1$}] (a11) at (1,-1) {\kknoteninhalt{${x_1}$\\$x_2~\barx_2$\\$x_3~\barx_3$}} ;
\node[vertex,label={below:$\bara_2$}] (a20) at (3,1) {\kknoteninhalt{$x_1~\barx_1$\\$\barx_2$\\$x_3~\barx_3$}} ;
\node[vertex,label={below:$a_2$}] (a21) at (3,-1) {\kknoteninhalt{$x_1~\barx_1$\\${x_2}$\\$x_3~\barx_3$}} ;
\node[vertex,label={below:$\bara_3$}] (a30) at (5,1) {\kknoteninhalt{$x_1~\barx_1$\\$x_2~\barx_2$\\$\barx_3$}} ;
\node[vertex,label={below:$a_3$}] (a31) at (5,-1) {\kknoteninhalt{$x_1~\barx_1$\\$x_2~\barx_2$\\${x_3}$}} ;

\node[vertex,label={below:$L_{1,1}$}] (l11) at (9,1.5) {\kknoteninhalt{$x_1$\\$x_2~\barx_2$\\$x_3~\barx_3$}} ;
\node[vertex,label={below:$L_{1,2}$}] (l12) at (9,0) {\kknoteninhalt{$x_1~\barx_1$\\$x_2$\\$x_3~\barx_3$}} ;
\node[vertex,label={below:$L_{1,3}$}] (l13) at (9,-1.5) {\kknoteninhalt{$x_1~\barx_1$\\$x_2~\barx_2$\\$\barx_3$}} ;

\node[vertex,label={below:$L_{2,1}$}] (l21) at (11,1.5) {\kknoteninhalt{$\barx_1$\\$x_2~\barx_2$\\$x_3~\barx_3$}} ;
\node[vertex,label={below:$L_{2,2}$}] (l22) at (11,0) {\kknoteninhalt{$x_1~\barx_1$\\$x_2$\\$x_3~\barx_3$}} ;
\node[vertex,label={below:$L_{2,3}$}] (l23) at (11,-1.5) {\kknoteninhalt{$x_1~\barx_1$\\$x_2~\barx_2$\\$\barx_3$}} ;

\node[vertex,label={below:$L_{3,1}$}] (l31) at (13,1.5) {\kknoteninhalt{$x_1~\barx_1$\\$x_2$\\$x_3~\barx_3$}} ;
\node[vertex,label={below:$L_{3,2}$}] (l32) at (13,0) {\kknoteninhalt{$x_1~\barx_1$\\$x_2~\barx_2$\\$x_3$}} ;
\node[vertex,label={below:$L_{3,3}$}] (l33) at (13,-1.5) {\kknoteninhalt{$x_1~\barx_1$\\$x_2~\barx_2$\\$x_3$}} ;

%\path[edge] (rechts) edge [bend left=65] (links) ;

\foreach \von/\zu in {start/p1, p1/p2, p2/p3}
  \draw[edge] (\von) -- (\zu) ;
  
\foreach \von/\zu in {a1/a2,a2/a3}
{ \foreach \i in {0,1}
    \foreach \j in {0,1}
   \draw[edge] (\von\i.east) -- (\zu\j) ;
}

\foreach \von/\zu in {a3/l1}
{ \foreach \i in {0,1}
    \foreach \j in {1,2,3}
   \draw[edge] (\von\i.east) -- (\zu\j) ;
}

\foreach \von/\zu in {l1/l2,l2/l3}
{ \foreach \i in {1,2,3}
    \foreach \j in {1,2,3}
   \draw[edge] (\von\i) -- (\zu\j) ;
}

\coordinate (p4) at (7.5,3) ;
\coordinate (p5) at (7.5,2.2) ;

\coordinate (q1) at (14.5,2.2) ;
\coordinate (q2) at (-0.4,2.2) ;
\coordinate (aa) at (-0.4,0) ;

\draw[edge] (p3) -- (p4) -- (p5) ;
\draw[edge] (q1) -- (q2) -- (aa) ;

%\draw[edge] (p3) -- ++(right:12mm) -- ++(down:12mm) -- ++(left:70mm) -- (aa)  ;
\draw[edge] (aa) -- (a10) ;
\draw[edge] (aa) -- (a11) ;

\coordinate (h31) at (14.5,1.5)  ;
\coordinate (h32) at (14.5,0)  ;
\coordinate (h33) at (14.5,-1.5)  ;
\draw[edge] (l31) -- (h31) ;
\draw[edge] (l32) -- (h32) ;
\draw[edge] (l33) -- (h33) ;

\draw[edge] (h33) -- (q1) ;



\end{tikzpicture}
}



==> tikz-preambel.tex <==
%%% TikZ
\RequirePackage{tikz}
\usetikzlibrary{%
	arrows,%
	automata,%
	chains,%
	trees,%
	positioning,%
	scopes,%
	calc,%
	decorations.markings,%
	shadows,%
	shapes,%
	fadings,%
	decorations.pathreplacing%
}

% Other Nodes Styles
\tikzset{
stateCircle/.style={draw=black,
										circle,
										inner sep=0mm,
										minimum size=5mm,
%										general shadow={fill=schatten,
%																		shadow yshift=-1.5pt,
%																		shadow xshift=1.5pt},
										fill=white
										},
state/.style={	draw=black,
							rectangle,
%							general shadow={fill=schatten,
%															shadow yshift=-1.5pt,
%															shadow xshift=1.5pt},
							fill=white,
							inner sep=.5mm,
							minimum height=.4cm},
stateEllipse/.style={draw=black,
										ellipse,
										inner sep=1mm,
										minimum size=5mm,
%										general shadow={fill=schatten,
%																		shadow yshift=-1.5pt,
%																		shadow xshift=1.5pt},
										fill=white},
smallEllipse/.style={ellipse,draw=black,inner sep=0.0mm,fill=white},
legende/.style={minimum height=0.2cm,minimum width=0.2cm},
legendeRund/.style={draw=black,circle,minimum height=0.2cm,minimum width=0.2cm},
niceArrows/.style={->,>=stealth',black}
}

% Post's Lattice Clone-Node-Styles
\colorlet{schatten}{white}
\tikzset{
				clone/.style={circle,
											inner sep=0,
											minimum width=4.7mm,
%											general shadow={fill=schatten,
%																			shadow yshift=-1.1pt,
%																			shadow xshift=1.1pt},
											fill=white,
											font=\scriptsize,
											thick},
				x=0.7cm,y=0.55cm,
				edge/.style={draw=black,solid,-},
%				clonefill/.style={draw=black,circle,minimum width=4.8mm,inner sep=0,font=\scriptsize,thick}}
                clonefill/.style={draw=black,circle,minimum width=3.2mm,inner sep=0,font=\tiny,thick}}

\tikzset{
				clone/.style={circle,
											inner sep=0,
											minimum width=4.7mm,
%											general shadow={fill=schatten,
%																			shadow yshift=-1.1pt,
%																			shadow xshift=1.1pt},
											fill=white,
											font=\scriptsize,
											thick},
				x=0.7cm,y=0.55cm,
				edge/.style={draw=black,solid,-},
%				clonefill/.style={draw=black,circle,minimum width=4.8mm,inner sep=0,font=\scriptsize,thick}}
                mmclonefill/.style={draw=black,circle,minimum width=6mm,inner sep=0,font=\tiny,thick}}

% Complexityclass-Colors
\definecolor{2EXPTIME}{rgb}{0.74,0.26,0.86} 
\definecolor{EXPTIME}{rgb}{0.98,0.30,0.62}
\colorlet{EXPtriv}{EXPTIME!20}
\definecolor{PSPACE}{rgb}{0.9,0.27,0.27} 
\definecolor{DeltaP2}{rgb}{0.55,0.2,0.17}
\definecolor{coNP}{rgb}{0.91,0.65,0.31}
\definecolor{NP}{rgb}{0.88,0.9,0.54}
\definecolor{P}{rgb}{0.27,0.75,0.24}
\definecolor{LOGCFL}{rgb}{0.7,1,0.29}
\definecolor{NL}{rgb}{0.83,1,0.67}
\definecolor{L}{rgb}{0.6,0.99,1}
\definecolor{NC1}{rgb}{0.6,0.78,1}
\definecolor{TC0}{rgb}{0.66,0.61,1}

\definecolor{hellgrau}{gray}{0.8}

\tikzfading[name=fade EEXP, 
left color=2EXPTIME!0, 
right color=2EXPTIME!100] 


\tikzset{
	2EXPTIME/.style={fill=2EXPTIME},
	EXPTIME/.style={fill=EXPTIME},
	EXPTtriv/.style={fill=EXPtriv},
	PSPACE/.style={fill=PSPACE},
	DeltaP2/.style={fill=DeltaP2},
	coNP/.style={fill=coNP},
	NP/.style={fill=NP},
	P/.style={fill=P},
	LOGCFL/.style={fill=LOGCFL},
	NL/.style={fill=NL},
	L/.style={fill=L},
	NC1/.style={fill=NC1},
	TC0/.style={fill=TC0},
	trivial/.style={fill=white},
	open/.style={fill=gray}
}
